Provable Benefits of Task-Specific Prompts for In-context Learning

The in-context learning capabilities of modern language models have motivated a deeper mathematical understanding of sequence models. A line of recent work has shown that linear attention models can emulate projected gradient descent iterations to implicitly learn the task vector from the data provided in the context window. In this work, we consider a novel setting where the global task distribution can be partitioned into a union of conditional task distributions. We then examine the use of task-specific prompts and prediction heads for learning the prior information associated with the conditional task distribution using a one-layer attention model. Our results on loss landscape show that task-specific prompts facilitate a covariance-mean decoupling where prompt-tuning explains the conditional mean of the distribution whereas the variance is learned/explained through in-context learning. Incorporating task-specific head further aids this process by entirely decoupling estimation of mean and variance components. This covariance-mean perspective similarly explains how jointly training prompt and attention weights can provably help over fine-tuning after pretraining.

==> app/add_notations.tex <==
\section{Auxiliary Notations}

==> app/add_related.tex <==
\section{Extended Related Work}

Understanding the mechanisms underlying in-context learning (ICL) in large language models (LLMs) has become a crucial area of research~\citep{brown2020language,liu2023pre, rae2021scaling}, especially as LLMs continue to demonstrate impressive generalization capabilities across a wide range of applications~\citep{team2023gemini,gpt4_techreport,touvron2023_llama}. ICL allows models to leverage a few examples provided at inference time to adapt to new tasks without parameter updates, effectively functioning as meta-learners. This property has spurred efforts to uncover how LLMs utilize in-context information to make predictions.

A key line of research aims to provide theoretical interpretations of ICL. For instance, \citet{xie2022an} interpret ICL as a form of implicit Bayesian inference, suggesting that LLMs infer a shared latent concept from the provided examples and apply it to make predictions under certain assumptions about the data distribution. This Bayesian perspective posits that, during pre-training, the model learns to generalize in a way that allows it to infer latent structures among in-context examples during inference.

Complementing the Bayesian view, \citet{olsson2022context} propose that "induction heads" play a fundamental role in enabling ICL within Transformer architectures. These specialized attention mechanisms identify and propagate patterns found in the context, allowing the model to extend observed sequences to make predictions. This structural explanation ties the mechanism of ICL to specific architectural components of Transformers.

Moreover, several studies investigate how the statistical properties of training data influence the emergence of ICL capabilities. \citet{park2024can} focus on how different distributional characteristics, such as data variability and feature overlap, affect a model's ability to generalize through in-context examples. This line of work emphasizes that the distributional properties of pre-training data play a significant role in shaping the generalization behaviors observed during ICL.

The pioneering work by \citet{garg2022can} extends the theoretical analysis of ICL by exploring how Transformers can learn to perform ICL when the in-context examples are labeled by functions from a given class, such as linear models. This study reveals that Transformers, when exposed to such prompts, can learn to approximate a target function through the provided examples, essentially treating the in-context examples as a learning dataset. This work has led to subsequent research that further explores the conditions under which ICL emerges in Transformers.

Following this foundational study, several works have focused specifically on understanding the connection between ICL and gradient-based learning mechanisms. \citet{akyrek2023what} explore the ability of Transformers to emulate a single step of gradient descent (GD) based on in-context examples. They demonstrate that Transformers trained on prompts representing gradient-based learning can exhibit behaviors similar to those learned through explicit optimization algorithms. Similarly, \citet{von2023transformers} construct Transformer weights that mimic gradient descent steps for linear regression tasks, finding that their constructed networks resemble those learned from training on in-context prompts for similar problems. These studies suggest that ICL in Transformers may function by implicitly learning gradient-based updates within the attention mechanism.

Building on these primarily empirical insights, recent research has focused on developing a more rigorous theoretical understanding of how ICL manifests in simpler models, such as single-layer linear attention mechanisms. \citet{zhang2024trained}, \citet{mahankali2024one}, and \citet{ahn2024transformers} investigate how single-layer linear attention models can implement gradient descent-like behaviors when trained on in-context prompts. For example, \citet{mahankali2024one} and \citet{ahn2024transformers} show that models trained on isotropic Gaussian data learn to perform a single GD step during test-time inference. They further extend their analysis to anisotropic Gaussian features, showing that the learned models implement preconditioned gradient descent (PGD) steps when faced with non-isotropic conditions. These works provide a connection between ICL and classical optimization techniques, establishing a theoretical framework for understanding the behavior of linear attention models in simple regression tasks.

Furthermore, \citet{zhang2024trained} delve into the optimization dynamics of training single-layer linear attention models using gradient flow, focusing on convergence properties and robustness to distributional shifts. Despite the inherent non-convexity of the problem, they demonstrate convergence to the global minimum for in-context linear regression tasks and characterize how factors such as prompt length affect test-time performance. Their analysis also highlights potential vulnerabilities of linear attention models to certain types of distributional shifts, such as changes in covariate distributions between training and testing data.

These research efforts collectively offer valuable insights into the mechanisms behind ICL, particularly by connecting the observed behaviors of LLMs to well-known optimization principles like gradient descent. However, most of these studies focus on relatively idealized settings, such as zero-mean data distributions or single-task learning scenarios. In contrast, real-world applications often involve diverse tasks with non-zero means and complex data distributions, creating a gap between theoretical understanding and practical implementations of ICL.


Our research differs from these existing studies in several key aspects. While previous theoretical analyses focus on single-task ICL with zero-mean assumptions and predominantly study scenarios where models implicitly perform a single gradient descent step~\citep{zhang2024trained, mahankali2024one, ahn2024transformers}, our work expands the scope to multi-task ICL where tasks can have varying means and covariances. We propose and analyze training strategies for prompt-tuning in single-layer linear attention models, deriving closed-form solutions that generalize to settings with non-zero means and anisotropic covariances. Our introduction of the "covariance-mean decoupling" concept provides a novel framework for understanding how training strategies impact model performance across tasks, which has not been explored in prior work. Additionally, unlike \citet{von2023transformers} and \citet{akyrek2023what}, who focus on constructing models that emulate GD, we focus on analyzing the performance improvements achievable through different training strategies, offering insights into how attention models can be optimally designed and fine-tuned for better in-context learning performance. Our work thus represents a significant step toward understanding the dynamics of prompt-tuning and task-specific adaptation in more complex, real-world multi-task settings.



%

% {\color{blue}In a recent work,\asrnote{Not sure if we need this colored text.} motivated by the work on connecting ICL to implicit GD performed by Transformers, \citet{duraisamy2024finite} study non-asymptotic precise generalization error for in-context single step gradient-descent in a linear regression setting and contrasted it with the error realized by least square regression. Notably, they restrict themselves to in-context feature vectors distributed according to \textit{standard} normal distribution.}


% \citet{mahankali2024one}

% \citet{ahn2024transformers}

% Data distributional properties drive emergent in-context learning in transformers~\citep{chan2022data}

% Induction heads -- \citep{olsson2022context}



% Trained Transformers Learn Linear Models In-Context~\citep{zhang2024trained}

% Finite Sample Analysis and Bounds of Generalization Error of GD in In-Context Linear Regression~\citep{duraisamy2024finite}




% Hungary hungary hippos\citet{fu2023hungry}

% Is Mamba Capable of In-Context Learning?~\citep{grazzi2024mamba}

% Can Mamba Learn How to Learn? A Comparative Study on In-Context Learning Tasks~\cite{park2024can}




% Transformers as algorithms: Generalization and stability in in-context learning~\citet{li2023transformers}

% Transformers as statisticians: Provable in-context learning with in-context algorithm selection~\cite{bai2024transformers}

% A statistical perspective on retrieval-based models~\citet{basu2023statistical}

% Atlas: Few-shot learning with retrieval augmented language models~\citet{izacard2023atlas}

% Training data is more valuable than you think: A simple and effective method by retrieving from training data~\citet{wang2022training} -- REINA

% Webgpt: Browser-assisted question-answering with human feedback~\citet{nakano2021webgpt}

% Why Can {GPT} Learn In-Context? Language Models Secretly Perform GD as Meta-Optimizers~\cite{dai2023gpt}







% Transformers are RNN -- linear attention~\citep{katharopoulos2020transformers}

% Linear transformers are secretly fast weight programmers -- \citet{schlag2021linear}

==> app/proof_feature.tex <==
\section{Supporting results}
\noindent $\bullet$ \textbf{$2n$-th moment of normal distribution:} Let $u\sim\Nc(0,\sigma^2)$, then
\[
\E[u^{2n}] = \sigma^{2n}(2n-1)!!
\]

\noindent $\bullet$ \textbf{Forth moment: } Let $\ub\sim\Nc(0,\Iden_d)$, then for any $\W\in\R^{d\times d}$, 
\begin{align*}
\E\left[(\ub^\top\W\ub)^2\right]&=\E\left[\left(\sum_{i,j=1}^dW_{ij}u_iu_j\right)^2\right]\\
&=\E\left[\left(\sum_{i=1}^dW_{ii}u_i^2\right)^2\right]+\E\left[\left(\sum_{i\neq j}W_{ij}u_iu_j\right)^2\right]\\
&=\sum_{i=1}^dW_{ii}^2\E\left[u_i^4\right]+\sum_{i\neq j}W_{ii}W_{jj}\E[u_i^2]\E[u_j^2]+\sum_{i\neq j}W_{ij}^2\E[u_i^2]\E[u_j^2]+\sum_{i\neq j}W_{ij}W_{ji}\E[u_i^2]\E[u_j^2]\\
&=3\sum_{i=1}^dW_{ii}^2+\sum_{i\neq j}W_{ii}W_{jj}+\sum_{i\neq j}W_{ij}^2+\sum_{i\neq j}W_{ij}W_{ji}\\
&=\sum_{i,j=1}^dW_{ii}W_{jj}+\sum_{i,j=1}^dW_{ij}^2+\sum_{i,j=1}^dW_{ij}W_{ji}\\
&=\trace{\W}^2+\trace{\W\W^\top}+\trace{\W^2}
\end{align*}

\noindent $\bullet$ \textbf{Forth moment: } Let $\ub\sim\Nc(0,\Iden_d)$, then for any $\W,\W'\in\R^{d\times d}$, 
\begin{align*}
&\E\left[(\ub^\top\W\ub)(\ub^\top\W'\ub)\right]\\
&=\E\left[\left(\sum_{i,j=1}^dW_{ij}u_iu_j\right)\left(\sum_{i,j=1}^dW'_{ij}u_iu_j\right)\right]\\
&=\E\left[\left(\sum_{i=1}^dW_{ii}u_i^2\right)\left(\sum_{i=1}^dW'_{ii}u_i^2\right)\right]+\E\left[\left(\sum_{i\neq j}W_{ij}u_iu_j\right)\left(\sum_{i\neq j}W_{ij}'u_iu_j\right)\right]\\
&=\sum_{i=1}^dW_{ii}W'_{ii}\E\left[u_i^4\right]+\sum_{i\neq j}W_{ii}W'_{jj}\E[u_i^2]\E[u_j^2]+\sum_{i\neq j}W_{ij}W'_{ij}\E[u_i^2]\E[u_j^2]+\sum_{i\neq j}W_{ij}W'_{ji}\E[u_i^2]\E[u_j^2]\\
&=3\sum_{i=1}^dW_{ii}W'_{ii}+\sum_{i\neq j}W_{ii}W'_{jj}+\sum_{i\neq j}W_{ij}W'_{ij}+\sum_{i\neq j}W_{ij}W'_{ji}\\
&=\sum_{i,j=1}^dW_{ii}W'_{jj}+\sum_{i,j=1}^dW_{ij}W'_{ij}+\sum_{i,j=1}^dW_{ij}W'_{ji}\\
&=\trace{\W}\trace{\W'}+\trace{\W'\W^\top}+\trace{\W\W'}
\end{align*}

\noindent $\bullet$ \textbf{Forth moment (version 2): } Let $\ub,\vb\sim\Nc(0,\Iden_d)$, then for any $\W,\W'\in\R^{d\times d}$, 
\begin{align*}
&\E\left[(\ub^\top\W\vb\vb^\top\ub)^2\right]\\
&=\E\left[\left(\sum_{i,j=1}^dW_{ij}u_iv_j\right)^2\left(\sum_{i=1}^du_iv_i\right)^2\right]\\
&=\E\left[\left(\sum_{i,j=1}^dW_{ij}^2u_i^2v_j^2+\sum_{i\neq i'}W_{ij}W_{i'j}u_iu_{i'}v_j^2+\sum_{j\neq j'}W_{ij}W_{ij'}u_i^2v_jv_{j'}+\sum_{i'\neq i,j'\neq j}W_{ij}W_{i'j'}u_iu_{i'}v_jv_{j'}\right)\left(\sum_{i=1}^du_i^2v_i^2+\sum_{i\neq j}u_iu_jv_iv_j\right)\right]\\
&=\E\left[\left(\sum_{i,j=1}^dW_{ij}^2u_i^2v_j^2\right)\left(\sum_{i=1}^du_i^2v_i^2\right)+\left(\sum_{i\neq j}W_{ij}W_{ji}u_i^2u_j^2v_i^2v_j^2\right)\right]\\
&=\E\left[\left(\sum_{i=1}^dW_{ii}^2u_i^2v_i^2+\sum_{i\neq j}W_{ij}^2u_i^2v_j^2\right)\left(\sum_{i=1}^du_i^2v_i^2\right)\right]+\sum_{i\neq j}W_{ij}W_{ji}\\
&=\E\left[\left(\sum_{i=1}^dW_{ii}^2u_i^4v_i^4+\sum_{i\neq j}W_{ii}^2u_i^2v_i^2u_j^2v_j^2\right)\right]+\E\left[\left(\sum_{i\neq j}W_{ij}^2u_i^4v_j^2v_i^2+\sum_{i\neq j}W_{ij}^2u_i^2v_j^4u_j^2+\sum_{i\neq j\neq k}W_{ij}^2u_i^2v_j^2u_k^2v_k^2\right)\right]+\sum_{i\neq j}W_{ij}W_{ji}\\
&=9\sum_{i=1}^dW_{ii}^2+(d-1)\sum_{i=1}^dW_{ii}^2+6\sum_{i\neq j}W_{ij}^2+(d-2)\sum_{i \neq j}W_{ij}^2+\sum_{i\neq j}W_{ij}W_{ji}\\
&=3\sum_{i=1}^dW_{ii}^2+(d+4)\sum_{i,j=1}^dW_{ij}^2+\sum_{i,j=1}^dW_{ij}W_{ji}\\
&=3\tr{\La_{\W}^2}+(d+4)\tr{\W\W^\top}+\tr{\W^2}
\end{align*}

\noindent $\bullet$ \textbf{6th moment: } Let $\ub\sim\Nc(0,\Iden_d)$, then for any $\W,\W'\in\R^{d\times d}$, 
\begin{align*}
&\E\left[(\ub^\top\W\ub)(\ub^\top\W'\ub)\tn{\ub}^2\right]\\
&=\E\left[\left(\sum_{i,j=1}^dW_{ij}u_iu_j\right)\left(\sum_{i,j=1}^dW'_{ij}u_iu_j\right)\left(\sum_{i=1}^du_i^2\right)\right]\\
&=\E\left[\left(\sum_{i=1}^dW_{ii}u_i^2\right)\left(\sum_{i=1}^dW'_{ii}u_i^2\right)\left(\sum_{i=1}^du_i^2\right)\right]+\E\left[\left(\sum_{i\neq j}W_{ij}u_iu_j\right)\left(\sum_{i\neq j}W_{ij}'u_iu_j\right)\left(\sum_{i=1}^du_i^2\right)\right]\\
&=\sum_{i=1}^dW_{ii}W'_{ii}\E\left[u_i^4\left(\sum_{i'=1}^du_{i'}^2\right)\right]+\sum_{i\neq j}W_{ii}W'_{jj}\E\left[u_i^2u_j^2\left(\sum_{i'=1}^du_{i'}^2\right)\right]\\
&\quad+\sum_{i\neq j}W_{ij}W'_{ij}\E\left[u_i^2u_j^2\left(\sum_{i'=1}^du_{i'}^2\right)\right]+\sum_{i\neq j}W_{ij}W'_{ji}\E\left[u_i^2u_j^2\left(\sum_{i'=1}^du_{i'}^2\right)\right]\\
&=(d+4)\left(3\sum_{i=1}^dW_{ii}W'_{ii}+\sum_{i\neq j}W_{ii}W'_{jj}+\sum_{i\neq j}W_{ij}W'_{ij}+\sum_{i\neq j}W_{ij}W'_{ji}\right)\\
&=(d+4)\left(\sum_{i,j=1}^dW_{ii}W'_{jj}+\sum_{i,j=1}^dW_{ij}W'_{ij}+\sum_{i,j=1}^dW_{ij}W'_{ji}\right)\\
&=(d+4)\left(\trace{\W}\trace{\W'}+\trace{\W'\W^\top}+\trace{\W\W'}\right)
\end{align*}
\begin{align*}
    &\E\left[u_i^4\left(\sum_{i'=1}^du_{i'}^2\right)\right]=\E[u^6]+(d-1)\E[u^4]\E[u^2]=3(d+4)\\
    &\E\left[u_i^2u_j^2\left(\sum_{i'=1}^du_{i'}^2\right)\right]=2\E[u^4]\E[u^2]+(d-2)\E[u^2]\E[u^2]\E[u^2]=d+4
\end{align*}

\noindent $\bullet$ \textbf{6th moment (version 2): } Let $\ub\sim\Nc(0,\Iden_d)$, then for any $\W,\W'\in\R^{d\times d}$, 
\begin{align*}
&\E\left[(\ub^\top\W\ub)\tn{\ub}^4\right]\\
&=\E\left[\left(\sum_{i,j=1}^dW_{ij}u_iu_j\right)\left(\sum_{i,j=1}^du_i^2u_j^2\right)\right]\\
&=\E\left[\left(\sum_{i=1}^dW_{ii}u_i^2\right)\left(\sum_{i=1}^du_i^4+\sum_{i\neq j}u_i^2u_j^2\right)\right]+\E\left[\left(\sum_{i\neq j}W_{ij}u_iu_j\right)\left(\sum_{i=1}^du_i^4+\sum_{i\neq j}u_i^2u_j^2\right)\right]\\
&=\sum_{i=1}^dW_{ii}\E\left[u_i^2\left(\sum_{i'=1}^du_{i'}^4+\sum_{i'\neq j'}u_{i'}^2u_{j'}^2\right)\right]\\
&=(d+2)(d+4)\sum_{i=1}^dW_{ii}\\
&=(d+2)(d+4)\trace{\W}
\end{align*}
\begin{align*}
    &\E\left[u_i^2\left(\sum_{i'=1}^du_{i'}^4+\sum_{i'\neq j'}u_{i'}^2u_{j'}^2\right)\right]\\
    &=\E[u^6]+(d-1)\E[u^2]\E[u^4]+2(d-1)\E[u^4]\E[u^2]+(d-1)(d-2)\E[u^2]\E[u^2]\E[u^2]\\
    &=15+3(d-1)+6(d-1)+(d-1)(d-2)\\
    &=(d+2)(d+4)
\end{align*}

\noindent $\bullet$ \textbf{8th moment: } Let $\ub\sim\Nc(0,\Iden_d)$, then for any $\W,\W'\in\R^{d\times d}$, 
\begin{align*}
&\E\left[(\ub^\top\W\ub)(\ub^\top\W'\ub)\tn{\ub}^4\right]\\
&=\E\left[\left(\sum_{i,j=1}^dW_{ij}u_iu_j\right)\left(\sum_{i,j=1}^dW'_{ij}u_iu_j\right)\left(\sum_{i,j=1}^du_i^2u_j^2\right)\right]\\
&=\E\left[\left(\sum_{i=1}^dW_{ii}u_i^2\right)\left(\sum_{i=1}^dW'_{ii}u_i^2\right)\left(\sum_{i=1}^du_i^4+\sum_{i\neq j}u_i^2u_j^2\right)\right]+\E\left[\left(\sum_{i\neq j}W_{ij}u_iu_j\right)\left(\sum_{i\neq j}W_{ij}'u_iu_j\right)\left(\sum_{i=1}^du_i^4+\sum_{i\neq j}u_i^2u_j^2\right)\right]\\
&=\sum_{i=1}^dW_{ii}W'_{ii}\E\left[u_i^4\left(\sum_{i'=1}^du_{i'}^4+\sum_{i'\neq j'}u_{i'}^2u_{j'}^2\right)\right]+\sum_{i\neq j}W_{ii}W'_{jj}\E\left[u_i^2u_j^2\left(\sum_{i'=1}^du_{i'}^4+\sum_{i'\neq j'}u_{i'}^2u_{j'}^2\right)\right]\\
&\quad+\sum_{i\neq j}W_{ij}W'_{ij}\E\left[u_i^2u_j^2\left(\sum_{i'=1}^du_{i'}^4+\sum_{i'\neq j'}u_{i'}^2u_{j'}^2\right)\right]+\sum_{i\neq j}W_{ij}W'_{ji}\E\left[u_i^2u_j^2\left(\sum_{i'=1}^du_{i'}^4+\sum_{i'\neq j'}u_{i'}^2u_{j'}^2\right)\right]\\
&=(d+4)(d+6)\left(3\sum_{i=1}^dW_{ii}W'_{ii}+\sum_{i\neq j}W_{ii}W'_{jj}+\sum_{i\neq j}W_{ij}W'_{ij}+\sum_{i\neq j}W_{ij}W'_{ji}\right)\\
&=(d+4)(d+6)\left(\sum_{i,j=1}^dW_{ii}W'_{jj}+\sum_{i,j=1}^dW_{ij}W'_{ij}+\sum_{i,j=1}^dW_{ij}W'_{ji}\right)\\
&=(d+4)(d+6)\left(\trace{\W}\trace{\W'}+\trace{\W'\W^\top}+\trace{\W\W'}\right)
\end{align*}
\begin{align*}
    &\E\left[u_i^4\left(\sum_{i'=1}^du_{i'}^4+\sum_{i'\neq j'}u_{i'}^2u_{j'}^2\right)\right]\\
    &=\E[u^8]+(d-1)\E[u^4]\E[u^4]+2(d-1)\E[u^6]\E[u^2]+(d-1)(d-2)\E[u^4]\E[u^2]\E[u^2]\\
    &=105+9(d-1)+30(d-1)+3(d-1)(d-2)\\
    &=3(d+4)(d+6)\\
    &\E\left[u_i^2u_j^2\left(\sum_{i'=1}^du_{i'}^4+\sum_{i'\neq j'}u_{i'}^2u_{j'}^2\right)\right]\\
    &=2\E[u^6]\E[u^2]+(d-2)\E[u^4](\E[u^2])^2+2\E[u^4]\E[u^4]+4(d-2)\E[u^4](\E[u^2])^2+(d-2)(d-3)(\E[u^2])^4\\
    &=30+3(d-2)+18+12(d-2)+(d-2)(d-3)\\
    &=(d+4)(d+6)
\end{align*}
\section{Task-feature alignment}

In this section, we consider the task-feature alignment data model. In this model, we first draw task vector $\bt$ via
\[
\bt\sim\Nc(0,\Iden).
\]
Then we generate examples via
\[
\x_i\sim\Nn(\alpha\bt,\Iden),\quad\xi_i\sim\Nc(0,\sigma^2)\quad\text{and}\quad y_i=\x_i^\top \bt+\xi_i,
\]
and we can rewrite 
\[
\g_i\sim\Nc(0,\Iden),\quad\xi_i\sim\Nc(0,\sigma^2)\quad\text{and}\quad\x_i=\alpha\bt+\g_i,\quad y_i=(\alpha\bt+\g_i)^\top\bt+\xi_i=\g_i^\top\bt+\alpha\tn{\bt}^2+\xi_i.
\]
Then recap the loss function from \eqref{gd}, we obtain
\begin{align}
    \Lc(\W)&=\E\left[(y-g(\Z))^2\right]\nn\\
    &=\E\left[\left(\x^\top\bt+\xi-\x^\top\W\X^\top(\X\bt+\bxi)\right)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2+2(\x^\top\bt-\x^\top\W\X^\top\X\bt)(\xi-\x^\top\W\X^\top\bxi)+(\xi-\x^\top\W\X^\top\bxi)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+\E\left[(\x^\top\W\X^\top\bxi)^2\right]+\sigma^2\nn.
\end{align}
We first focus on 
\begin{align*}
    \E\left[(\x^\top\W\X^\top\bxi)^2\right]&=\E\left[\left((\alpha\bt+\g)^\top\W\sum_{i=1}^n\xi_i(\alpha\bt+\g_i)\right)^2\right]\\
    &=n\sigma^2\E\left[\left((\alpha\bt+\g)^\top\W(\alpha\bt+\g')\right)^2\right]\\
    &=n\sigma^2\left(\alpha^4\E\left[(\bt^\top\W\bt)^2\right]+2\alpha^2\E\left[(\bt^\top\W\g')^2\right]+\E\left[(\g^\top\W\g')^2\right]\right)\\
    &=n\sigma^2\left(\alpha^4\left(\trace{\W}^2+\trace{\W^2}+\trace{\W\W^\top}\right)+(2\alpha^2+1)\trace{\W\W^\top}\right)\\
    &=n\sigma^2\left(\alpha^4\trace{\W}^2+\alpha^4\trace{\W^2}+(\alpha^2+1)^2\trace{\W\W^\top}\right).
\end{align*}

Next, we focus on the following:
\begin{align*}
    \E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]&=\E\left[((\alpha\bt+\g)^\top(\bt-\W\X^\top\X\bt))^2\right]\\
    &=\E\left[\left(\alpha\bt^\top\bt-\alpha\bt^\top\W\X^\top\X\bt+\g^\top\bt-\g^\top\W\X^\top\X\bt\right)^2\right]\\
    &=\alpha^2\E[(\bt^\top\bt)^2]+\alpha^2\E[(\bt^\top\W\X^\top\X\bt)^2]+\E[(\g^\top\bt)^2]+\E[(\g^\top\W\X^\top\X\bt)^2]\\
    &\quad-2\alpha^2\E[\bt^\top\bt\bt^\top\W\X^\top\X\bt]-2\E[\bt^\top\g\g^\top\W\X^\top\X\bt]\\
    &=\alpha^2d(d+2)+\alpha^2\underset{(a)}{\underbrace{\E[(\bt^\top\W\X^\top\X\bt)^2]}}+d+\underset{(b)}{\underbrace{\E[(\g^\top\W\X^\top\X\bt)^2]}}\\
    &\quad-2\alpha^2\underset{(c)}{\underbrace{\E[\bt^\top\bt\bt^\top\W\X^\top\X\bt]}}-2\underset{(d)}{\underbrace{\E[\bt^\top\g\g^\top\W\X^\top\X\bt]}}.%\\
    % &=\alpha^2\E\left[(\bt^\top(\bt-\W\X^\top\X\bt))^2\right]+\E\left[\tn{\bt-\W\X^\top\X\bt}^2\right].
\end{align*}
We first obtain
\begin{align*}
    \X^\top\X\bt&=\sum_{i=1}^n\x_i\x_i^\top\bt\\
    &=\sum_{i=1}^n(\alpha\bt+\g_i)(\alpha\bt+\g_i)^\top\bt\\
    &=\sum_{i=1}^n\alpha^2\bt\bt^\top\bt+\alpha\bt\g_i^\top\bt+\alpha\g_i\bt^\top\bt+\g_i\g_i^\top\bt.
\end{align*}
\begin{align*}
    (a):\quad&\E[(\bt^\top\W\X^\top\X\bt)^2]=\E\left[\left(\sum_{i=1}^n\alpha^2\bt^\top\W\bt\bt^\top\bt+\alpha\bt^\top\W\bt\g_i^\top\bt+\alpha\bt^\top\W\g_i\bt^\top\bt+\bt^\top\W\g_i\g_i^\top\bt\right)^2\right]\\
    &=\alpha^4n^2\E\left[\left(\bt^\top\W\bt\bt^\top\bt\right)^2\right]+\alpha^2\E\left[\left(\sum_{i=1}^n\bt^\top\W\bt\g_i^\top\bt\right)^2\right]+\alpha^2\E\left[\left(\sum_{i=1}^n\bt^\top\W\g_i\bt^\top\bt\right)^2\right]+\E\left[\left(\sum_{i=1}^n\bt^\top\W\g_i\g_i^\top\bt\right)^2\right]\\
    &\quad+2\alpha^2n\E\left[\sum_{i=1}^n\bt^\top\W\bt\bt^\top\bt\bt^\top\W\g_i\g_i^\top\bt\right]+2\alpha^2\E\left[\sum_{i=1}^n\bt^\top\W\bt\g_i^\top\bt\bt^\top\W\g_i\bt^\top\bt\right]\\
    &=\alpha^4n^2\E\left[\left(\bt^\top\W\bt\bt^\top\bt\right)^2\right]+\alpha^2n\E\left[\left(\bt^\top\W\bt{\g'}^\top\bt\right)^2\right]+\alpha^2n\E\left[\left(\bt^\top\W{\g'}\bt^\top\bt\right)^2\right]+\E\left[\left(\sum_{i=1}^n\bt^\top\W\g_i\g_i^\top\bt\right)^2\right]\\
    &\quad+2\alpha^2n^2\E\left[\bt^\top\W\bt\bt^\top\bt\bt^\top\W\g'{\g'}^\top\bt\right]+2\alpha^2n\E\left[\bt^\top\W\bt\g_i^\top\bt\bt^\top\W\g_i\bt^\top\bt\right]\\
    &=\alpha^4n^2(d+4)(d+6)(M_1+M_2+M_3)+\alpha^2n(d+4)(M_1+M_2+M_3)+\alpha^2n(d+2)(d+4)M_2\\
    &\quad+3nM_4+(d+4)nM_2+nM_3+n(n-1)(M_1+M_2+M_3)\\
    &\quad+2\alpha^2n^2(d+4)(M_1+M_2+M_3)+2\alpha^2n(d+4)(M_1+M_2+M_3)\\
    &=A_1M_1+A_2M_2+A_3M_3+A_4M_4\\
    (b):\quad&\E\left[(\g^\top\W\X^\top\X\bt)^2\right]=\E\left[\left(\sum_{i=1}^n\alpha^2\g^\top\W\bt\bt^\top\bt+\alpha\g^\top\W\bt\g_i^\top\bt+\alpha\g^\top\W\g_i\bt^\top\bt+\g^\top\W\g_i\g_i^\top\bt\right)^2\right]\\        
    &=\alpha^4n^2\E\left[\left(\g^\top\W\bt\bt^\top\bt\right)^2\right]+\alpha^2\E\left[\left(\sum_{i=1}^n\g^\top\W\bt\g_i^\top\bt\right)^2\right]+\alpha^2\E\left[\left(\sum_{i=1}^n\g^\top\W\g_i\bt^\top\bt\right)^2\right]+\E\left[\left(\sum_{i=1}^n\g^\top\W\g_i\g_i^\top\bt\right)^2\right]\\
    &\quad+2\alpha^2n\E\left[\sum_{i=1}^n\g^\top\W\bt\bt^\top\bt\g^\top\W\g_i\g_i^\top\bt\right]+2\alpha^2\E\left[\sum_{i=1}^n\g^\top\W\bt\g_i^\top\bt\g^\top\W\g_i\bt^\top\bt\right]\\
    &=\alpha^4n^2\E\left[\left(\g^\top\W\bt\bt^\top\bt\right)^2\right]+\alpha^2n\E\left[\left(\g^\top\W\bt{\g'}^\top\bt\right)^2\right]+\alpha^2n\E\left[\left(\g^\top\W{\g'}\bt^\top\bt\right)^2\right]+\E\left[\left(\sum_{i=1}^n\g^\top\W\g_i\g_i^\top\bt\right)^2\right]\\
    &\quad+2\alpha^2n^2\E\left[\g^\top\W\bt\bt^\top\bt\g^\top\W\g'{\g'}^\top\bt\right]+2\alpha^2n\E\left[\g^\top\W\bt\g_i^\top\bt\g^\top\W\g_i\bt^\top\bt\right]\\
    &=\alpha^4n^2(d+2)(d+4)M_2+\alpha^2n(d+2)M_2+\alpha^2nd(d+2)M_2+n(d+2)M_2+n(n-1)M_2\\
    &\quad+2\alpha^2n^2(d+2)M_2+2\alpha^2n(d+2)M_2\\
    &=A_5M_2\\
    (c):\quad&\E\left[\bt^\top\bt\bt^\top\W\X^\top\X\bt\right]=n\E\left[\bt^\top\bt\bt^\top\W(\alpha\bt+\g')(\alpha\bt+\g')^\top\bt\right]\\
    &=\alpha^2n\E\left[\bt^\top\bt\bt^\top\W\bt\bt^\top\bt\right]+n\E\left[\bt^\top\bt\bt^\top\W{\g'}{\g'}^\top\bt\right]\\
    &=\alpha^2n(d+2)(d+4)\tr{\W}+n(d+2)\tr{\W}\\
    &=A_6\tr{\W}\\
    (d):\quad&\E\left[\bt^\top\g\g^\top\W\X^\top\X\bt\right]=n\E\left[\bt^\top\g\g^\top\W(\alpha\bt+\g')(\alpha\bt+\g')^\top\bt\right]\\
    &=\alpha^2n\E\left[\bt^\top\g\g^\top\W\bt\bt^\top\bt\right]+n\E\left[\bt^\top\g\g^\top\W\g'{\g'}^\top\bt\right]\\
    &=\alpha^2n(d+2)\tr{\W}+n\tr{\W}\\
    &=A_7\tr{\W}
\end{align*}
\begin{align*}
    \E\left[\left(\sum_{i=1}^n\bt^\top\W\g_i\g_i^\top\bt\right)^2\right]&=n\E\left[\left(\bt^\top\W\g'{\g'}^\top\bt\right)^2\right]+n(n-1)\E\left[\bt^\top\W\g'{\g'}^\top\bt\bt^\top\W\g''{\g''}^\top\bt\right]\\
    &=3nM_4+(d+4)nM_2+nM_3+n(n-1)(M_1+M_2+M_3)
\end{align*}
\begin{align*}
    \E\left[\left(\sum_{i=1}^n\g^\top\W\g_i\g_i^\top\bt\right)^2\right]&=n\E\left[\left(\g^\top\W\g'{\g'}^\top\bt\right)^2\right]+n(n-1)\E\left[\g^\top\W\g'{\g'}^\top\bt\g^\top\W\g''{\g''}^\top\bt\right]\\
    &=n(d+2)M_2+n(n-1)M_2
\end{align*}
\[
M_1 = \tr{\W}^2\qquad M_2=\tr{\W\W^\top}\qquad M_3=\tr{\W^2}\qquad M_4=\tr{\La_{\W}^2}
\]

If consider noiseless setting:
\begin{align*}
    \nabla\Lc(\W)=0\\
    \alpha^2\left(2A_1\tr{\W}\Iden+2A_2\W+2A_3\W^\top+2A_4\diag{\La_{\W}}\right)+2A_5\W-(2\alpha^2A_6+2A_7)\Iden=0\\
    (\alpha^2(dA_1+A_2+A_3+A_4)+A_5)\tr{\W}=(\alpha^2A_6+A_7)d\\
    \W = c\Iden\quad\text{where}\quad c = \frac{\alpha^2A_6+A_7}{\alpha^2(dA_1+A_2+A_3+A_4)+A_5}\\=\frac{\alpha^4n(d+2)(d+4)+2\alpha^2n(d+2)+n}{\alpha^6n^2(d+2)(d+4)(d+6)+\alpha^4n(d+2)(d+4)(3n+4)+\alpha^2n(3(d+4)+(d+2)(3n+d))+n(d+n+1)}\\
    =\frac{\alpha^4(d+2)(d+4)+2\alpha^2(d+2)+1}{\alpha^6n(d+2)(d+4)(d+6)+\alpha^4(d+2)(d+4)(3n+4)+\alpha^2(3(d+4)+(d+2)(3n+d))+(d+n+1)}
\end{align*}
\[
\Lc_\st=\alpha^2d(d+2)+d+\left(\alpha^2(dA_1+A_2+A_3+A_4)+A_5\right)c^2d-2\left(\alpha^2A_6+A_7\right)cd
\]

\[
\W\approx\frac{(\bar d+1)^2}{n\bar d^3+3n\bar d^2+(3n+d)\bar d+d+n}\Iden\qquad\Lc_\st\approx \bar d(d+2)+d-\frac{(\bar d+1)^4nd}{n\bar d^3+3n\bar d^2+(3n+d)\bar d+d+n}
\]
\[
\W\approx\frac{(\bar d+1)}{n(\bar d+1)^2+d}\Iden\qquad\Lc_\st\approx (\bar d+1)d-\frac{(\bar d+1)^3nd}{n(\bar d+1)^2+d}
\]
where $\bar d=\alpha^2(d+2)$.
Consider loss, we have 
\begin{align*}
        \alpha^2\left(2A_1\tr{\W}\Iden+2A_2\W+2A_3\W^\top+2A_4\diag{\La_{\W}}\right)+2A_5\W-(2\alpha^2A_6+2A_7)\Iden\\
        +n\sigma^2\left(2\alpha^4\tr{\W}\Iden+2\alpha^4\W+2(\alpha^2+1)^2\W\right)=0\\
    (\alpha^2(dA_1+A_2+A_3+A_4)+A_5+n\sigma^2(\alpha^4(d+1)+(\alpha^2+1)^2))\tr{\W}=(\alpha^2A_6+A_7)d\\
\end{align*}


% \section{Task-feature alignment}

% In this section, we consider the task-feature alignment model. In this model, we first draw task vector $\bt$ via
% \[
% \bt\sim\Nc(0,\Iden).
% \]
% Then we generate examples via
% \[
% \x_i\sim\Nn(\alpha\bt,\Iden),\quad\xi_i\sim\Nc(0,\sigma^2)\quad\text{and}\quad y_i=\x_i^\top \bt+\xi_i,
% \]
% and we can rewrite 
% \[
% \g_i\sim\Nc(0,\Iden),\quad\xi_i\sim\Nc(0,\sigma^2)\quad\text{and}\quad\x_i=\alpha\bt+\g_i,\quad y_i=(\alpha\bt+\g_i)^\top\bt+\xi_i=\g_i^\top\bt+\alpha\tn{\bt}^2+\xi_i.
% \]
% Then recap the loss function from \eqref{gd} and let $\bxi=[\xi_1~\cdots~\xi_n]^\top$, $\Gb=[\g_1~\cdots~\g_n]^\top$ where we have 
% \[
% \X=\alpha\onebb\bt^\top+\Gb\quad\text{and}\quad\y=\X\bt+\bxi=(\alpha\onebb\bt^\top+\Gb)\bt+\bxi=\alpha\tn{\bt}^2\onebb+\Gb\bt+\bxi.
% \]
% Then we obtain
% \begin{align}
%     \Lc(\W)&=\E\left[(y-g(\Z,\x))^2\right]\nn\\
%     &=\E\left[\left(\x^\top\bt+\xi-\x^\top\W\X^\top(\X\bt+\bxi)\right)^2\right]\nn\\
%     &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2+2(\x^\top\bt-\x^\top\W\X^\top\X\bt)(\xi-\x^\top\W\X^\top\bxi)+(\xi-\x^\top\W\X^\top\bxi)^2\right]\nn\\
%     &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+\E\left[(\x^\top\W\X^\top\bxi)^2\right]+\sigma^2\nn.
%     % &=\E\left[\tn{\x-(\x^\top\W\X^\top\X)^\top}^2\right]+\E\left[(\x^\top\W\X^\top\bxi)^2\right]+\sigma^2\nn.
%     % &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2,\nn\\
%     % &=\E\left[\tn{\bt-\W\X^\top\X\bt}^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2.\label{ind loss}
% \end{align}
% We first focus on 
% \begin{align*}
%     \E\left[(\x^\top\W\X^\top\bxi)^2\right]&=\E\left[((\alpha\bt+\g)^\top\W(\alpha\onebb\bt^\top+\Gb)^\top\bxi)^2\right]\\
%     &=\alpha^4\E\left[(\bt^\top\W\bt\onebb^\top\bxi)^2\right]+\alpha^2\E\left[(\bt^\top\W\Gb^\top\bxi)^2\right]+\alpha^2\E\left[(\g^\top\W\bt\onebb^\top\bxi)^2\right]+\E\left[(\g^\top\W\Gb^\top\bxi)^2\right]\\
%     &\approx n\alpha^4\sigma^2\trace{\W}^2+n\alpha^2\sigma^2\trace{\W\W^\top}+n\alpha^2\sigma^2\trace{\W\W^\top}+n\sigma^2\trace{\W\W^\top}\\
%     &=n\sigma^2\left(\alpha^4\trace{\W}^2+(2\alpha^2+1)\trace{\W\W^\top}\right)
% \end{align*}

% Next, we focus on the following:
% \begin{align*}
%     \E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]&=\E\left[((\alpha\bt+\g)^\top(\bt-\W\X^\top\X\bt))^2\right]\\
%     &=\alpha^2\E\left[(\bt^\top(\bt-\W\X^\top\X\bt))^2\right]+\E\left[\tn{\bt-\W\X^\top\X\bt}^2\right].
% \end{align*}
% We first obtain
% \begin{align*}
%     \X^\top\X\bt&=(\alpha\onebb\bt^\top+\Gb)^\top(\alpha\onebb\bt^\top+\Gb)\bt\\
%     &=\alpha^2n\tn{\bt}^2\bt+\alpha\bt\onebb^\top\Gb\bt+\alpha\tn{\bt}^2\Gb^\top\onebb+\Gb^\top\Gb\bt\\
%     &\approx \alpha^2nd\bt+\alpha\bt\onebb^\top\Gb\bt+\alpha d\Gb^\top\onebb+\Gb^\top\Gb\bt
% \end{align*}
% where we used $\tn{\bt}^2\approx d$. Here recall from \eqref{decomp XXB}, we have
% \[
% \frac{1}{n}\Gb^\top\Gb\bt\approx\bt+\sqrt{\frac{d}{n}}\hb,\quad\text{where}\quad\hb\sim\Nc(0,\Iden)
% \]
% and $\Gb^\top\onebb$ is distributed as $\Nc(0,n\Iden)$ and set $\Gb^\top\onebb=\sqrt{n}\tilde\g$. 
% We obtain
% \[
% \bt-\frac{1}{n}\W\X^\top\X\bt\approx\left(\Iden-(\alpha^2d+1)\W\right)\bt-\sqrt{\frac{d}{n}}\W\hb-\frac{\alpha d}{\sqrt{n}}\W\tilde\g-\frac{\alpha\tilde\g^\top\bt}{\sqrt{n}}\W\bt.
% \]
% and
% \[
% \E\left[\tn{\bt-\frac{1}{n}\W\X^\top\X\bt}^2\right]=
% \]
% Then 
% \begin{align*}
%     \x^\top\left(\bt-\frac{1}{n}\W\X^\top\X\bt\right)&\approx(\alpha\bt+\g)^\top\left(\Iden-(\alpha^2d+1)\W\right)\bt\\
%     &\quad-\sqrt{\frac{d}{n}}(\alpha\bt+\g)^\top\W\hb-\frac{\alpha d}{\sqrt{n}}(\alpha\bt+\g)^\top\W\tilde\g-\frac{\alpha\tilde\g^\top\bt}{\sqrt{n}}(\alpha\bt+\g)^\top\W\bt\\
%     % &\red{=\alpha\bt^\top\left(\bt-\frac{1}{n}\W\X^\top\X\bt\right)+\g^\top\left(\bt-\frac{1}{n}\W\X^\top\X\bt\right)}
% \end{align*}
% \red{Use the fact that $\g$ related products are easy to compute (your $\gamma_{\g,\dots}$ terms might be resulting in errors):}
% \begin{align}
% &\E[(\g^\top\left(\bt-\frac{1}{n}\W\X^\top\X\bt\right))^2]=\E[\tn{\bt-\frac{1}{n}\W\X^\top\X\bt}^2]\\
% &\E[\g^\top\left(\bt-\frac{1}{n}\W\X^\top\X\bt\right)\bt^\top\left(\bt-\frac{1}{n}\W\X^\top\X\bt\right))]=0.
% \end{align}
% Additionally, we approximate and set
% \begin{align*}
% &\bt^\top\W\bt\approx\trace{\W}\quad\text{and}\\
% &\g_1^\top\W\g_2:=\|\W\|_F\gamma_{\g_1,\g_2}\quad\text{where}\quad\E[\gamma_{\g_1,\g_2}]=0,~\E[\gamma_{\g_1,\g_2}^2]=1.
% \end{align*}
% Then
% \begin{align*}
% \x^\top\left(\bt-\frac{1}{n}\W\X^\top\X\bt\right)&\approx\alpha\cdot\trace{\Iden-(\alpha^2d+1+\alpha\tilde\g^\top\bt)\W}+\left\|\left(\Iden-(\alpha^2d+1+\alpha\tilde\g^\top\bt)\W\right)\right\|_F\gamma_{\g,\bt}\\
% &\quad-\|\W\|_F\cdot\left(\sqrt{\frac{d}{n}}(\alpha \gamma_{\bt,\hb}+\gamma_{\g,\hb})-\frac{\alpha d}{\sqrt{n}}(\alpha\gamma_{\bt,\tilde\g}+\gamma_{\g,\tilde\g})\right)\\
% &\approx\alpha\cdot\trace{\Iden-\alpha^2d\W}+\left\|\left(\Iden-\alpha^2d\W\right)\right\|_F\gamma_{\g,\bt}\\
% &\quad-\|\W\|_F\cdot\left(\sqrt{\frac{d}{n}}(\alpha \gamma_{\bt,\hb}+\gamma_{\g,\hb})-\frac{\alpha d}{\sqrt{n}}(\alpha\gamma_{\bt,\tilde\g}+\gamma_{\g,\tilde\g})\right).
% \end{align*}
% Therefore,
% \begin{align*}
%     \E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]&\approx \alpha^2\trace{\Iden-\alpha^2d\W)}^2+\|\Iden-\alpha^2d\W\|^2\\
%     % +\alpha^2\left((n\alpha^2d+n)^2+\alpha^2 nd\right)\trace{\W}^2\\
%     &\quad+\left(\alpha^4d^2n+\alpha^2dn+\alpha^2d^2n+nd)\right)\|\W\|_F^2\\
%     % &\quad-2\alpha^2d(n\alpha^2d+n)\trace{\W}\\
%     % &\quad+\trace{\left(\Iden-()}
%     &=\alpha^2\left(d^2+(n\alpha^2d+n)^2\trace{\W}^2-2(n\alpha^2d+n)\trace{\W}\right)\\
%     &\quad+d+(n\alpha^2d+n)^2\trace{\W\W^\top}-2(n\alpha^2d+n)\trace{\W}\\
%     &\quad+dn(\alpha^2+1)(d+1)\|\W\|_F^2
% \end{align*}

% --------------------------------

% Since $\tn{\bt}\approx\sqrt{d}$, consider the following
% \begin{align*}
%     \x^\top\bt-\x^\top\W\X^\top\X\bt&\approx(\alpha\bt+\g)^\top\bt-(\alpha\bt+\g)^\top\W(\alpha\onebb\bt^\top+\Gb)^\top(\alpha\onebb\bt^\top+\Gb)\bt\\
%     &=\alpha d+\g^\top\bt-(\alpha\bt+\g)^\top\W\left(n\alpha^2d\bt+\alpha\bt\onebb^\top\Gb\bt+\alpha d\Gb^\top\onebb+\Gb^\top\Gb\bt\right).
% \end{align*}
% Here recall from \eqref{decomp XXB}, we have
% \[
% \frac{1}{n}\Gb^\top\Gb\bt\approx\bt+\sqrt{\frac{d}{n}}\hb,\quad\text{where}\quad\hb\sim\Nc(0,\Iden)
% \]
% and $\Gb^\top\onebb$ is distributed as $\Nc(0,n\Iden)$ and let $\Gb^\top\onebb\approx\sqrt{n}\tilde\g$. Then we obtain
% \begin{align*}
%     \x^\top\bt-\x^\top\W\X^\top\X\bt&\approx\alpha \bt^\top\bt+\g^\top\bt-(\alpha\bt+\g)^\top\W\left(n\alpha^2d\bt+\alpha\sqrt{n}\bt\tilde\g^\top\bt+\alpha \sqrt{n}d\tilde\g+n\bt+\sqrt{dn}\hb\right)\\
%     &=\alpha \bt^\top\bt+\g^\top\bt-(\alpha\bt+\g)^\top\W\left((n\alpha^2d+n)\bt+\alpha\sqrt{n}(\bt\bt^\top+d\Iden)\tilde\g+\sqrt{dn}\hb\right).
% \end{align*}
% Additionally, let 
% \begin{align*}
% % &\bt^\top\W\bt\approx\trace{\W}\quad\text{and}\\
% &\g_1^\top\W\g_2\approx\|\W\|_F\gamma_{\g_1,\g_2}\quad\text{where}\quad\E[\gamma_{\g_1,\g_2}]=0,~\E[\gamma_{\g_1,\g_2}^2]=1.
% \end{align*}
% Then, 
% \begin{align*}
%     \x^\top\bt-\x^\top\W\X^\top\X\bt&\approx\alpha \bt^\top\left(\Iden-(n\alpha^2d+n)\W\right)\bt+\g^\top\left(\Iden-(n\alpha^2d+n)\W\right)\bt\\
%     % -\alpha(n\alpha^2d+n+\alpha\sqrt{n}\bt^\top\tilde\g)\trace{\W}\\
%     % &\quad-\Big(\alpha^2d\sqrt{n}\cdot\gamma_{\bt,\tilde\g}+\alpha\sqrt{dn}\cdot\gamma_{\bt,\hb}+(n\alpha^2d+n-\alpha\sqrt{n}\bt^\top\tilde\g)\cdot\gamma_{\g,\bt}\\
%     % &\quad+\alpha d\sqrt{n}\cdot\gamma_{\g,\tilde\g}+\sqrt{dn}\cdot\gamma_{\g,\hb}\Big)\|\W\|_F.
%     &\quad-\left(\alpha^2d\sqrt{n}\cdot\gamma_{\bt,\tilde\g}+\alpha\sqrt{dn}\cdot\gamma_{\bt,\hb}+\alpha \sqrt{n}d\cdot\gamma_{\g,\tilde\g}+\sqrt{dn}\cdot\gamma_{\g,\hb}\right)\|\W\|_F\\
%     % &\quad+(n\alpha^2d+n-\alpha\sqrt{n}\bt^\top\tilde\g)\g^\top\W\bt.
% \end{align*}
% Therefore,
% \begin{align*}
%     \E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]&\approx \alpha^2\trace{\Iden-(n\alpha^2d+n)\W)}^2+\trace{(\Iden-(n\alpha^2d+n)\W)(\Iden-(n\alpha^2d+n)\W)^\top}\\
%     % +\alpha^2\left((n\alpha^2d+n)^2+\alpha^2 nd\right)\trace{\W}^2\\
%     &\quad+\left(\alpha^4d^2n+\alpha^2dn+\alpha^2d^2n+nd)\right)\|\W\|_F^2\\
%     % &\quad-2\alpha^2d(n\alpha^2d+n)\trace{\W}\\
%     % &\quad+\trace{\left(\Iden-()}
%     &=\alpha^2\left(d^2+(n\alpha^2d+n)^2\trace{\W}^2-2(n\alpha^2d+n)\trace{\W}\right)\\
%     &\quad+d+(n\alpha^2d+n)^2\trace{\W\W^\top}-2(n\alpha^2d+n)\trace{\W}\\
%     &\quad+dn(\alpha^2+1)(d+1)\|\W\|_F^2
% \end{align*}
% % 
% Combing all together results in that 
% \begin{align*}
%     \frac{1}{2}\nabla_{\W}\Lc(\W)&\approx \left(\alpha^2(n\alpha^2d+n)^2+n\sigma^2\alpha^4\right)\trace{\W}\Iden\\
%     &\quad+\left((n\alpha^2d+n)^2+dn(\alpha^2+1)(d+1)+n\sigma^2(2\alpha^2+1)\right)\W\\
%     &\quad-(\alpha^2+1)(n\alpha^2d+n)\Iden.
% \end{align*}
% Let $\alpha=\sqrt{{c}/{d}}$. Then setting $\nabla_{\W}\Lc(\W)=0$, we obtain
% \begin{align*}
%     &\left(cn^2(c+1)^2+nc^2\sigma^2/d\right)\frac{\trace{\W}}{d}\Iden\\
%     &\quad+\left(n^2(c+1)^2+c^2n+cdn+nd+n\sigma^2(2c/d+1)\right)\W\\
%     &\quad-n(c/d+1)(c+1)\Iden=0\\
%     \Longrightarrow\W_\st&=\frac{(c/d+1)(c+1)}{n(c+1)^3+c^2+cd+d+\sigma^2(2c/d+1)+c^2\sigma^2/d}\\
%     % &=\frac{n(\alpha^2+1)(c+1)}{n(c+1)^3+2c^2+c+d(c+1)+\sigma^2(2c/d+1)+c^2\sigma^2/d}
%     &\approx\frac{(c+1)}{n(c+1)^3+cd+d+\sigma^2}=\frac{1}{n(c+1)^2+d+\sigma^2/(c+1)}
% \end{align*}

==> app/proof_iid.tex <==
\section{Proof of Theorem~\ref{thm:independent}}
\label{app:independent}
\begin{proof}
Consider a general  independent linear model similar as defined in \eqref{data ind} and suppose
\[
\x\sim\Nc(0,\bSi_{\x}),\quad\bt\sim\Nc(0,\bSi_{\bt}),\quad\xi\sim\Nc(0,\sigma^2),\quad\text{and}\quad y=\x^\top\bt+\xi.
\]
Let 
\[
\X=[\x_1~\cdots~\x_n]^\top,\quad\bxi=[\xi_1~\cdots~\xi_n]^\top,\quad\text{and}\quad \y=[y_1~\cdots~y_n]^\top=\X\bt+\bxi.
\]


To simplify, let $\xb=\bSi_{\x}^{-1/2}\x$, $\Xb=\X\bSi_{\x}^{-1/2}$,  $\btb=\bSi_{\x}^{1/2}\bt$ where we have $\xb\sim\Nc(0,\Iden)$, $\btb\sim\Nc(0,\bSi_{\x}^{1/2}\bSi_{\bt}\bSi_{\x}^{1/2})$ and
\[
y=\xb^\top\btb+\xi,\qquad\y=\Xb\btb+\bxi.
\]

Then recap the loss from \eqref{obj gd}, and we obtain
\begin{align}
    \Lc(\W)&=\E\left[(y-g(\Z))^2\right]\nn\\
    &=\E\left[\left(\x^\top\bt+\xi-\x^\top\W\X^\top(\X\bt+\bxi)\right)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2+2(\x^\top\bt-\x^\top\W\X^\top\X\bt)(\xi-\x^\top\W\X^\top\bxi)+(\xi-\x^\top\W\X^\top\bxi)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+\E\left[(\x^\top\W\X^\top\bxi)^2\right]+\sigma^2\nn.%\\
    % &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2,\nn\\
    % &=\E\left[\tn{\bt-\W\X^\top\X\bt}^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2.\label{ind loss}
\end{align}
where the last equality comes from the independence of label noise $\xi,\bxi$.

We first consider the following term
\begin{align*}
    \E\left[(\x^\top\W\X^\top\bxi)^2\right]=\E\left[(\xb^\top(\bSi_{\x}^{1/2}\W\bSi_{\x}^{1/2})\Xb^\top\bxi)^2\right]=n\sigma^2\cdot\trace{\Wb\Wb^\top}
\end{align*}
where we define $\Wb=\bSi_{\x}^{1/2}\W\bSi_{\x}^{1/2}$. 
Next, focus on the following
\begin{align*}
    \E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]&=\E\left[(\xb^\top\btb-\xb^\top\Wb\Xb^\top\Xb\btb)^2\right]\\
    &=\E\left[\left(\xb^\top\left(\Iden-\Wb\Xb^\top\Xb\right)\btb\right)^2\right]\\
    &=\trace{\E\left[\left(\Iden-\Wb\Xb^\top\Xb\right)\bSi\left(\Iden-\Wb\Xb^\top\Xb\right)^\top\right]}\\
    &=\trace{\bSi}-\tr{\bSi(\Wb+\Wb^\top)\E[\Xb^\top\Xb]}+\tr{\Wb^\top\Wb\E[\Xb^\top\Xb\bSi\Xb^\top\Xb]}\\
    &=\trace{\bSi}-2n\cdot\tr{\bSi\Wb}+\tr{\Wb^\top\Wb\E[\Xb^\top\Xb\bSi\Xb^\top\Xb]},
\end{align*}
where $\bSi:=\bSi_{\x}^{1/2}\bSi_{\bt}\bSi_{\x}^{1/2}$. 


Let $\xb_i\in\R^n$ be the $i$th column of $\Xb$ and $\bSi_{ij}$ be the $(i,j)$th entry of $\bSi$. Then the $(i,j)$ entry of matrix $\Xb^\top\Xb\bSi\Xb^\top\Xb$ is
\[
(\Xb^\top\Xb\bSi\Xb^\top\Xb)_{ij}=\sum_{k=1}^d\sum_{p=1}^d\bSi_{kp}\xb_i^\top\xb_k\xb_p^\top\xb_j.
\]
Then we get
\begin{align*}
    i\neq j:\quad\E\left[\left(\Xb^\top\Xb\bSi\Xb^\top\Xb\right)_{ij}\right]&=\bSi_{ij}\E[\xb_i^\top\xb_i\xb_j^\top\xb_j]+\bSi_{ji}\E[\xb_i^\top\xb_j\xb_i^\top\xb_j]=n^2\bSi_{ij}+n\bSi_{ji}\\
    i=j:\quad\E\left[\left(\Xb^\top\Xb\bSi\Xb^\top\Xb\right)_{ii}\right]&=\bSi_{ii}\E\left[\xb_i^\top\xb_i\xb_i^\top\xb_i\right]+\sum_{j\neq i}\bSi_{jj}\E\left[\xb_i^\top\xb_j\xb_j^\top\xb_i\right]\\
&=\bSi_{ii}\E\left[(x_{i1}^2+\cdots+x_{in}^2)^2\right]+n\sum_{j\neq i}\bSi_{jj}\\
&=\bSi_{ii}(3n+n(n-1))+n\sum_{j\neq i}\bSi_{jj}\\
&=n\left(\bSi_{ii}(n+1)+\sum_{j=1}^d\bSi_{jj}\right)\\
&=n\left(\bSi_{ii}(n+1)+\tr{\bSi}\right).
\end{align*}
Therefore 
\[
\E[\Xb^\top\Xb\bSi\Xb^\top\Xb]=n(n+1)\bSi+n\cdot\tr{\bSi}\Iden.
\]
Combining all together results in 
\begin{align}
\Lc(\W)=\tr{\bSi}-2n\tr{\bSi\Wb}+n(n+1)\tr{\bSi\Wb^\top\Wb}+n(\tr{\bSi}+\sigma^2)\tr{\Wb\Wb^\top}+\sigma^2.\label{loss}
\end{align}
Set $\nabla_{\Wb}\Lc(\W)=0$ returns
\[
-2n\cdot\bSi+2n(n+1)\cdot\bSi\Wb+2n(\tr{\bSi}+\sigma^2)\Wb=0\Longrightarrow\Wb_\st=\left((n+1)\Iden+(\tr{\bSi}+\sigma^2)\bSi^{-1}\right)^{-1}.
\]
Then we have 
\[
\W_\st=\bSi_{\x}^{-1/2}\left((n+1)\Iden+(\tr{\bSi}+\sigma^2)\bSi^{-1}\right)^{-1}\bSi_{\x}^{-1/2}
=\left((n+1)\bSi_{\x}+\left(\tr{\bSi_{\x}\bSi_{\bt}}+\sigma^2\right)\bSi_\bt^{-1}\right)^{-1}
\]
and 
$$\Lc^\st=\Lc(\W_\st)=\tr{\bSi}+\sigma^2-n\tr{((n+1)\bSi^{-1}+(\tr{\bSi}+\sigma^2)\bSi^{-2})^{-1}}.$$
% ------------------------------

% Let $\xb_i\in\R^n$ be the $i$th column of $\Xb$. Then the $(i,j)$ entry of matrix $\Xb^\top\Xb\Xb^\top\Xb$ is
% \[
% (\Xb^\top\Xb\Xb^\top\Xb)_{ij}=\xb_i^\top\left(\sum_{k=1}^d\xb_k\xb_k^\top\right)\xb_j,
% \]
% which gets $\E\left[\left(\Xb^\top\Xb\Xb^\top\Xb\right)_{ij}\right]=0$ for $i\neq j$, and for $i\in[d]$,
% \begin{align*}
% \E\left[\left(\Xb^\top\Xb\Xb^\top\Xb\right)_{ii}\right]&=\E\left[\xb_i^\top\xb_i\xb_i^\top\xb_i\right]+(d-1)\E\left[\xb_i^\top\xb_j\xb_j^\top\xb_i\right]\\
% &=\E\left[(x_{i1}^2+\cdots+x_{in}^2)^2\right]+(d-1)n\\
% &=3n+n(n-1)+(d-1)n\\
% &=n(n+d+1).
% \end{align*}
% Therefore $\E[\Xb^\top\Xb\Xb^\top\Xb]=n(n+d+1)\Iden$. 
% Combining all together results in 
% \[
% \Lc(\W)=\tr{\bSi}-2n\cdot\tr{\bSi\Wb}+n(n+d+1+\sigma^2)\cdot\tr{\bSi\Wb^\top\Wb}+\sigma^2.
% \]

% Set $\nabla_{\Wb}\Lc(\W)=0$ returns
% \[
% -2n\cdot\Iden+2n(n+d+1+\sigma^2)\cdot\Wb=0\Longrightarrow\Wb_\st=\frac{1}{n+d+1+\sigma^2}\Iden.
% \]
% Then we have 
% \[
% \Lc^\st=\left(1-\frac{n}{n+d+1+\sigma^2}\right)\tr{\bSi_{\x}\bSi_{\bt}}+\sigma^2\quad\text{and}\quad
% \W_\st=\frac{1}{n+d+1+\sigma^2}\bSi_{\x}^{-1}.
% \]

\begin{comment}
% where
% \begin{align*}
%     &\E\left[(\bt-\W\X^\top\X\bt)(\bt-\W\X^\top\X\bt)^\top\right]\\
%     &=\E\left[\bt\bt^\top-2\W\X^\top\X\bt\bt^\top+\W\X^\top\X\bt\bt^\top\X^\top\X\W^\top\right]\\
%     &=\bSi_{\bt}-2n\W\bSi_{\x}\bSi_{\bt}+ (n^2-n)\W\bSi_{\x}\bSi_{\bt}\bSi_{\x}\W^\top+n\W\E\left[\x\x^\top\bt\bt^\top\x\x^\top\right]\W^\top
% \end{align*}
% Additionally, let $\btb=\bt/\tn{\bt}$, $g=\x^\top\btb\in\Nc(0,\bSi_{\x})$, $\xb=\x-(\x^\top\btb)\btb=\x-g\btb$, and observe that $g,\xb$ are independent and $\xb,\bt$ are independent. We obtain
% \begin{align*}
%     \E\left[\x\x^\top\bt\bt^\top\x\x^\top\right]&=\E\left[g^2\tn{\bt}^2(\xb+g\btb)(\xb+g\btb)^\top\right]\\
%     &=\E\left[g^2\tn{\bt}^2\right]\E\left[\xb\xb^\top\right]+\E\left[g^3\tn{\bt}^2\bt\right]\E\left[\xb^\top\right]+\E\left[g^4\tn{\bt}^2\btb\btb^\top\right]\\
%     &=\trace{\bSi_{\x}\bSi_{\bt}}\cdot\left(\bSi_{\x}-2\bSi_{\x}+\right)
% \end{align*}
Consider the following orthogonal decomposition: Let $\btb=\bt/\tn{\bt}$, $\g=\X\btb$, $\Xb=\X-\X\btb\btb^\top=\X-\g\btb^\top$, and observe that $\g,\Xb$ are independent conditioned on $\btb$, $(\bt,\Xb)$ are orthogonal, and $\X=\Xb+\g\btb^\top$. We obtain
\begin{align*}
    \X^\top\X\bt=(\Xb+\g\btb^\top)^\top\g\tn{\bt}=\tn{\bt}\Xb^\top\g+\tn{\g}^2\bt.
\end{align*}
Note that $\g\sim\Nn(0,\Iden)$ conditioned on $\bt$. Additionally $\Xb$ is effectively a $n\times (d-1)$ standard normal as its rows lie over the $d-1$ dimensional subspace $\bPi=\Iden-\btb\btb^\top$.
%using $\tn{\bt}\approx\sqrt{d}$, the right hand side is approximately distributed as $\Nn(n\bt,nd\Iden_d)$. 

----------------------------------------------------

Consider independent linear data and suppose 
\[
\x\sim\Nc(0,\Iden),\quad\bt\sim\Nc(0,\bSi),\quad\xi\sim\Nc(0,\sigma^2),\quad\text{and}\quad y=\x^\top\bt+\xi.
\]
Then recap the loss from \eqref{gd} and let $\bxi=[\xi_1~\xi_2~\cdots~\xi_n]^\top$ where we have $\y=\X\bt+\bxi$. 
\begin{align}
    \Lc(\W)&=\E\left[(y-g(\Z,\x))^2\right]\nn\\
    &=\E\left[\left(\x^\top\bt+\xi-\x^\top\W\X^\top(\X\bt+\bxi)\right)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2+2(\x^\top\bt-\x^\top\W\X^\top\X\bt)(\xi-\x^\top\W\X^\top\bxi)+(\xi-\x^\top\W\X^\top\bxi)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+\E\left[(\x^\top\W\X^\top\bxi)^2\right]+\sigma^2\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2,\nn\\
    &=\E\left[\tn{\bt-\W\X^\top\X\bt}^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2.\label{ind loss}
\end{align}
% where
% \begin{align*}
%     &\E\left[(\bt-\W\X^\top\X\bt)(\bt-\W\X^\top\X\bt)^\top\right]\\
%     &=\E\left[\bt\bt^\top-2\W\X^\top\X\bt\bt^\top+\W\X^\top\X\bt\bt^\top\X^\top\X\W^\top\right]\\
%     &=\bSi_{\bt}-2n\W\bSi_{\x}\bSi_{\bt}+ (n^2-n)\W\bSi_{\x}\bSi_{\bt}\bSi_{\x}\W^\top+n\W\E\left[\x\x^\top\bt\bt^\top\x\x^\top\right]\W^\top
% \end{align*}
% Additionally, let $\btb=\bt/\tn{\bt}$, $g=\x^\top\btb\in\Nc(0,\bSi_{\x})$, $\xb=\x-(\x^\top\btb)\btb=\x-g\btb$, and observe that $g,\xb$ are independent and $\xb,\bt$ are independent. We obtain
% \begin{align*}
%     \E\left[\x\x^\top\bt\bt^\top\x\x^\top\right]&=\E\left[g^2\tn{\bt}^2(\xb+g\btb)(\xb+g\btb)^\top\right]\\
%     &=\E\left[g^2\tn{\bt}^2\right]\E\left[\xb\xb^\top\right]+\E\left[g^3\tn{\bt}^2\bt\right]\E\left[\xb^\top\right]+\E\left[g^4\tn{\bt}^2\btb\btb^\top\right]\\
%     &=\trace{\bSi_{\x}\bSi_{\bt}}\cdot\left(\bSi_{\x}-2\bSi_{\x}+\right)
% \end{align*}
Consider the following orthogonal decomposition: Let $\btb=\bt/\tn{\bt}$, $\g=\X\btb$, $\Xb=\X-\X\btb\btb^\top=\X-\g\btb^\top$, and observe that $\g,\Xb$ are independent conditioned on $\btb$, $(\bt,\Xb)$ are orthogonal, and $\X=\Xb+\g\btb^\top$. We obtain
\begin{align*}
    \X^\top\X\bt=(\Xb+\g\btb^\top)^\top\g\tn{\bt}=\tn{\bt}\Xb^\top\g+\tn{\g}^2\bt.
\end{align*}
Note that $\g\sim\Nn(0,\Iden)$ conditioned on $\bt$. Additionally $\Xb$ is effectively a $n\times (d-1)$ standard normal as its rows lie over the $d-1$ dimensional subspace $\bPi=\Iden-\btb\btb^\top$.
%using $\tn{\bt}\approx\sqrt{d}$, the right hand side is approximately distributed as $\Nn(n\bt,nd\Iden_d)$. 

{\color{red}
Define $\hb=\bar\X^\top\g/\tn{\g}\sim\Nn(0,\bPi)$ where $\bPi=\Iden-\btb\btb^\top$. We can decompose
\[
\X^\top\X\bt=\tn{\bt}\tn{\g}\hb+\tn{\g}^2\bt
\]
Key observation is that $\g,\hb$ are zero-mean gaussians and $(\tn{\g},\hb)$ are independent of each other conditioned on $\bt$. Let us take the expectations conditioned on $\bt$ first (i.e.~over $\X$ to take the expectations of $\hb,\g$ given $\bt$). Below we use $\E[\tn{\g}^4]=\sum_{i=1}^n \E[g_i^4]+\sum_{i\neq j}\E[g_i^2g_j^2]=n^2+2n$.
\begin{align*}
\E_{\X}[\tn{\bt-\W\X^\top\X\bt}^2]&=\E[\tn{\tn{\bt}\tn{\g}\W\hb+(\tn{\g}^2\W-\Iden)\bt}^2]\\
&=\E_{\X}[n\tn{\bt}^2\trace{\W\bPi\W^\top}+\tn{\bt}^2-2n\bt^\top\W\bt+(n^2+2n)\bt^\top\W\W^\top\bt].
%&=\E[nd\tn{\W\hb}^2]+\E[(\tn{(n\W-\Iden)\bt}^2]
\end{align*}
Note that $\E[\btb\btb^\top]=\Iden/d$ because $\btb$ is a random rank-1 projection matrix. Now taking expectation over $\bt$, using the independence of magnitude $\tn{\bt}$ and direction $\btb$ for gaussian vectors, and plugging in $\trace{\W\W^\top}=\tn{\W}^2$ we find $\E[\bPi]=(1-1/d)\Iden$, $\E[\tn{\bt}^2\bPi]=(d-1)\Iden$ and
\[ 
\E[\tn{\bt-\W\X^\top\X\bt}^2]=n(d-1)\tf{\W}^2+d-2n\cdot \trace{\W}+(n^2+2n)\tf{\W}^2.
\]
Differentiating, we find
\[ 
n(d-1)\W-n\Iden+(n^2+2n)\W=0\implies (d-1+n+2)\W=\Iden\implies \W=\frac{\Iden}{d+n+1}.
\]
%$\x_i = \hb-\X^T \g/\sqrt{n} = (1/\sqrt{n}-1/\|\g\|)\bar\X^T\g$
}




--------------------------------------------

% Define h=Xbar^T g/||g||. This way h is exactly h~N(0, Pi) where Pi=I-beta beta^T/||beta||^2.
% You can keep Pi in the analysis. It should change little because E[Pi]=(1-1/d)*I i.e. almost identity.
% Then you define xi = h-Xbar^T g/sqrt(n) = (1/sqrt(n)-1/||g||)*Xbar^T g. You similarly keep xi in the analysis and at the end say that terms involving xi are O(1/n) which is small compared to 1/sqrt(n).

Let $\hb\sim\Nn(0,\Iden_d)$, \red{and for some proper choice of $\hb$, we have $\tn{\hb-\Xb^\top\g/\sqrt{n}}=\order{1/\sqrt{nd}}$}. We can then write
% In other words, using $\tn{\bt}\approx\sqrt{d}$, for $\hb\sim\Nn(0,\Iden_d)$,
\begin{align}
\frac{1}{n}\X^\top\X\bt&= \bt+\sqrt{\frac{d}{n}}\hb+\left(\frac{\tn{\g}^2}{n}-1\right)\bt+\sqrt{\frac{d}{n}}\left(\frac{\tn{\bt}}{\sqrt{d}}\cdot\frac{\Xb^\top\g}{\sqrt{n}}-\hb\right)\nn\\
&=\bt+\sqrt{\frac{d}{n}}\hb+\beps.\label{decomp XXB}
% &=\bt+\sqrt{\frac{d}{n}}\hb+\order{\sqrt{\frac{d}{n}}\onebb}
\end{align} 
Thus,  
\begin{align*}
    \E\left[\tn{\bt-\W\X^\top\X\bt}^2\right]&=\E\left[\tn{\bt-n\W\left(\bt+\sqrt{\frac{d}{n}}\hb+\beps\right)}^2\right]\\
    &=\E\left[\tn{(\Iden-n\W)\bt-\sqrt{nd}\cdot\W\hb-n\W\beps}^2\right]\\
    &=\trace{(\Iden-n\W)\bSi(\Iden-n\W)^\top+nd\W\W^\top}+\order{1}\cdot\trace{\W\W^\top}.
\end{align*}
Combining with \eqref{ind loss}, we get
\begin{align*}
    \Lc(\W)&=\trace{(\Iden-n\W)\bSi(\Iden-n\W)^\top+nd\W\W^\top}+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2+\order{1}\cdot\trace{\W\W^\top}\\
    &=\trace{\bSi-2n\W\bSi+n^2\W\bSi\W^\top+n(d+\sigma^2)\W\W^\top}+\sigma^2+\order{1}\cdot\trace{\W\W^\top}.
\end{align*}
Next we obtain
\begin{align*}
\nabla_{\W}\Lc(\W)=-2n\bSi+2n^2\W\bSi+2(n(d+\sigma^2)+\order{1})\W
\end{align*}
and set $\nabla_{\W}\Lc(\W)=0$ returns
\[
\W=\bSi\left(n\bSi+(d+\sigma^2+\order{{1/n}})\Iden\right)^{-1}.
\]
Then if setting $\bSi=\Iden$, the optimal $\W$ is given by $\Ws\approx\frac{1}{n+d+\sigma^2}\Iden$.


    
\end{comment}

\end{proof}

==> app/proof_lora.tex <==
\section{Proof for LoRA -- \redp{Incomplete/Optional}}
\label{app:lora}

\begin{comment}
\begin{fact} Let $\bSi$ be a positive semidefinite matrix and let $\Ub,\Vb$ be matrices with orthonormal columns. We have that 
\[ 
2\cdot\trace{\Ub^\top\bSi\Vb}\leq \trace{\Ub^\top\bSi\Ub}+\trace{\Vb^\top\bSi\Vb}.
\]
\end{fact}
\begin{proof} Expanding $\tf{\sqrt{\bSi}(\Ub-\Vb)}^2$, we obtain
\[ 
0\leq \tf{\sqrt{\bSi}(\Ub-\Vb)}^2=\trace{\Ub^\top\bSi\Ub+\Vb^\top\bSi\Vb-2\Ub^\top\bSi\Vb}.
\] 
\end{proof}

\subsection{Low-Rank Attention without Symmetry}

\begin{proof} Recall the loss function from \eqref{loss}
\begin{align*}
\Lc(\W)&=\tr{\bSi}-2n\tr{\bSi\Wb}+n(n+1)\tr{\bSi\Wb^\top\Wb}+n(\tr{\bSi}+\sigma^2)\tr{\Wb\Wb^\top}+\sigma^2\\
&=\tr{\bSi}-2n\tr{\bSi\Wb^\top}+n(n+1)\tf{\bSi^{1/2}\Wb^\top}^2+n(\tr{\bSi}+\sigma^2)\tf{\Wb^\top}^2+\sigma^2
\end{align*}
where $\Wb=\bSi_{\x}^{1/2}\W\bSi_{\x}^{1/2}$ and $\bSi=\bSi_{\x}^{1/2}\bSi_{\bt}\bSi_{\x}^{1/2}$. 
For any $\Wb$, let us parameterize $\Wb^\top=\Ub\Db\Vb^\top$ where $\Vb,\Ub\in\R^{d\times r}$ denote the left/right singular vectors of $\Wb$ and $\Db\in\R^{r\times r}$. We will first treat $\Ub,\Vb$ as fixed and optimize $\Db$. We will then optimize $\Ub,\Vb$ and show that $\Ub=\Vb$. Fixing $\Ub,\Vb$, setting $\bSp=\Ub^\top\bSi\Vb$, $\bSb=\Ub^\top\bSi\Ub$ and let $M=\tr{\bSi}+\sigma^2$, we obtain
\begin{align*}
\Lc(\Db)&=M-2n\tr{\bSp^\top\Db}+n(n+1)\tf{\bSb^{1/2}\Db}^2+nM\tf{\Db}^2.
\end{align*}
Differentiating, we obtain 
\[
nM\Db+n(n+1)\bSb\Db=n\bSp\implies \Db=((n+1)\bSb+M\Iden)^{-1}\bSp.
\]
Now plugging in this optimal choice and using $\Vb^\top\Vb=\Iden$, we find 
\begin{align}
&\tr{\bSp^\top\Db}=\tr{\bSb((n+1)\bSb+M\Iden)^{-1}\bSb}=\tr{((n+1)\bSb+M\Iden)^{-1}\bSb^2}\\
&\tf{\bSb^{1/2}\Db}^2=\trace{((n+1)\bSb+M\Iden)^{-2}\A\bSb^2\A^\top\bSi}\\
&\tf{\Db}^2=\trace{((n+1)\bSb+M\Iden)^{-2}\A\bSb^2\A^\top}.
\end{align}
\newpage
Setting $\frac{\partial\Lc(\Db)}{\partial\Db_i}=0$ returns
\[
\Db_i^\st=\frac{\bSb_{ii}}{(n+1)\bSb_{ii}+M}.
\]
Plugging in this value, we obtain the optimal risk given by
\[ 
\Lc^\st:=\Lc^\st(\Ub)=M-n\sum_{i=1}^r \frac{\bSb_{ii}^2}{(n+1)\bSb_{ii}+M}=M-n\sum_{i=1}^r \frac{\bSb_{ii}}{(n+1)+M\bSb_{ii}^{-1}}.
\]
Now observe that, the right hand side is strictly decreasing function of the diagonal value $\bSb_{ii}$ of $\bSb=\Ub^\top\bSb\Ub$. Thus, to minimize $\Lc^\st(\Ub)$, we need to maximize $\sum_{i=1}^r\frac{n\bSb_{ii}}{M/\bSb_{ii}+n+1}$. It follows from Cauchy's interlace theorem that $\bSb_{ii}\leq \la_i$ where $\la_i$ is the $i$'th largest eigenvalue of $\Wb$ since $\bSb$ is an orthogonal projection of $\Wb$ on $\Ub$. Consequently, we find the desired bound where
\[
\Lc^\st=M-n\sum_{i=1}^r \frac{\la_{i}}{n+1+M\la_{i}^{-1}}.
\]
\end{proof}
\end{comment}

\subsection{Proof of Theorem~\ref{lora thm}}
\begin{theorem}\label{lora thm} 
Consider independent linear data as defined in \eqref{data ind}. Let $\W_0$ be the initial weight matrix. Define $\W=\Wlr+\W_0$. Recap the objective from \eqref{obj gd} and enforce $\rank{\Wlr}\leq r$ and $\Wlr=\Wlr^\top$. Let $\bSi=\bSi^{1/2}_{\x}\bSi_{\bt}\bSi_{\x}^{1/2}$ and $M=\tr{\bSi}+\sigma^2$. Assume $\W_0=\bSi_x^{-1/2}\Wb_0\bSi_x^{-1/2}$ and $(\Wb_0,\bSi)$ have identical eigenspaces i.e. $\Wb_0=\Ub\Eb\Ub^\top$ and $\bSi=\Ub\La\Ub^\top$ with $\la_i$ denoting the $i$'th largest eigenvalue of $\bSi$ and $d_i$ denotes the corresponding eigenvalue of $\W_0$. The LoRa solution obeys
\begin{align}
\red{\min_{\rank{\Wlr}\leq r,\Wlr=\Wlr^\top}\tilde\Lc(\W_{lora})= \dots}
%\leq\red{\min_{|\Ic|\leq r,\Ic\subset[d]}\left(\sum_{i\not\in\Ic}\frac{\lambda_i+M}{n+1+M/\la_i}+\sum_{i\in\Ic}\frac{\la^{new}_i+M}{n+1+M/\la^{new}_i}\right).} \label{formula lora2}
\end{align}
\end{theorem}
\begin{proof} We will carry out the analysis in the $\Wb=\bSi_x^{1/2}\W\bSi_x^{1/2}$ variable similar to Lemma \ref{low rank attn}. Thus, define $\Wbr=\bSi_x^{1/2}\Wlr \bSi_x^{1/2}$ and denote $\Wb=\Wb_0+\Wbr$. Recall $\bSi=\bSi_{\x}^{1/2}\bSi_{\bt}\bSi_{\x}^{1/2}$ and the loss function from \eqref{loss}
\begin{align*}
\Lc(\W)=\tr{\bSi}-2n\tr{\bSi\Wb}+n(n+1)\tr{\bSi\Wb^\top\Wb}+n(\tr{\bSi}+\sigma^2)\tr{\Wb\Wb^\top}+\sigma^2
\end{align*}
%where $\Wb=\bSi_{\x}^{1/2}\W\bSi_{\x}^{1/2}$ and . 
Let us parameterize $\Wbr=\A\Sb\A^\top$ where $\A\in\R^{d\times r}$ denotes the eigenvectors of $\Wbr$ and $\Sb\in\R^{r\times r}$ is the diagonal matrix of singular values. Now, setting $\Lb=\A^\top\Ub\in\R^{r\times d}$ and $\bSb=\A^\top\bSi\A$ observe that 
\begin{align*}
&\tr{\bSi\Wb}-\tr{\bSi\Wb_0}=\tr{\bSi\Wbr}=\tr{\Lb\La\Lb^\top \Sb}.\\
&\trace{\bSi\Wb^\top\Wb}-\trace{\bSi\Wb_0^\top\Wb_0}=\trace{\bSi\Wbr^2}+\trace{\bSi\Wb_0\Wbr}+\trace{\bSi\Wbr\Wb_0}\\
&\hspace{100pt}=\trace{\Lb\La\Lb^\top \Sb^2}+\trace{\Lb\La\Eb\Lb^\top \Sb}+\trace{\Lb\Eb\La\Lb^\top \Sb}\\
&\hspace{100pt}=\trace{\Lb\La\Lb^\top \Sb^2}+2\trace{\Lb\La\Eb\Lb^\top \Sb}.\\
&\trace{\Wb^\top\Wb}-\trace{\Wb_0^\top\Wb_0}=\trace{\Sb^2}+2\trace{\Lb\Eb\Lb^\top \Sb}.
%&=\trace{\Ub\La\Ub^\top\B \Sb^2\B^\top}=\trace{\Lb^\top\Ub^\top\bSi\Ub\Lb}.
\end{align*}
Aggregating these terms and setting $M=\tr{\bSi}+\sigma^2$ and setting $\Lcb(\Wlr)=\frac{\Lc(\W)-\Lc(\W_0)}{n}$, $\Bb=\Lb(\La-M\Eb-(n+1)\La\Eb)\Lb^\top$ and $\Cb=(M\Iden+(n+1)\Lb\La\Lb^\top)$, we obtain that
\begin{align}
\Lcb(\Wlr)&=M\cdot (\tr{\Sb^2}+2\tr{\Lb\Eb\Lb^\top\Sb})+(n+1)(\trace{\Lb\La\Lb^\top \Sb^2}+2\trace{\Lb\La\Eb\Lb^\top \Sb})-2\tr{\Lb\La\Lb^\top \Sb}\nonumber\\
&=\tr{\Cb\Sb^2}-2\tr{\Bb\Sb}.
\end{align}

Differentiation with respect to $\Sb$ %and setting $\nabla\Lcb=0$ returns
\[
\frac{1}{2}\nabla\Lcb(\Wlr)=(M\Iden+(n+1)\Lb\La\Lb^\top)\Sb-\Bb=\Cb\Sb-\Bb.
\]
Thus, we obtain that optimal $\Sb$ is given by
\begin{align}
\Sb^\st&=(M\Iden+(n+1)\Lb\La\Lb^\top)^{-1}\Bb\\
&=\Cb^{-1}\Bb%\Cb^{-1/2}\Bb\Cb^{-1/2}.
%&=\Lb(M\Iden+(n+1)\Lb\La\Lb^\top)\Lb^\top 
\end{align}
Set $\B=\La-M\Eb-(n+1)\La\Eb$. Using $\Lb^\top\Lb$ is a projection matrix, the objective is given by
\begin{align}
-\Lcb(\Wlr^\st)&=\tr{\Cb^{-1}\Bb^2}=\tr{(M\Iden+(n+1)\Lb\La\Lb^\top)^{-1}\Lb\B\Lb^\top\Lb\B\Lb^\top}\\
&=\tr{\B\Lb^\top(M\Iden+(n+1)\Lb\La\Lb^\top)^{-1}\Lb\B\Lb^\top\Lb}\\
&\leq \tr{\B\Lb^\top(M\Iden+(n+1)\Lb\La\Lb^\top)^{-1}\Lb\B}\\
&= \tr{(M\Iden+(n+1)\Lb\La\Lb^\top)^{-1}\Lb\B^2\Lb^\top}.
\end{align}
Applying matrix inversion lemma, we obtain
\[ 
(M\Iden+(n+1)\Lb\La\Lb^\top)^{-1}=M^{-1}\Iden-M^{-2}\Lb[(n+1)^{-1}\La^{-1}+M^{-1}\Lb^\top\Lb]^{-1}\Lb^\top.
\] 
Set $\bPi=\Lb^\top\Lb$. This yields
\begin{align} 
-M\Lcb(\Wlr^\st)&\leq \tr{\Lb\B^2\Lb^\top}-M^{-1}\tr{\Lb[(n+1)^{-1}\La^{-1}+M^{-1}\Lb^\top\Lb]^{-1}\Lb^\top\Lb\B^2\Lb^\top}\nonumber\\
&=\tr{\bPi\B^2}-M^{-1}\tr{[(n+1)^{-1}\La^{-1}+M^{-1}\bPi]^{-1}\bPi\B^2\bPi}\nonumber
\end{align}
\redp{Somehow we should conclude that optimal $\bPi/\Lb$ aligns with the eigenvectors of $\bSi$ and $\Wb_0$.}
\end{proof}




==> app/proof_low_rank.tex <==
\section{Proof of Lemma~\ref{low rank attn}}
\label{app:low-rank}

%\subsection{Proof of Lemma~\ref{low rank attn} -- revised}
{\color{red}
Let $\Wb=\Ub\Eb\Vb^\top$ and $\bSi=\B\La\B^\top$. Then
\begin{align*}
\Lc(\W)&=\tr{\bSi}-2n\tr{\bSi\Wb}+n(n+1)\tr{\bSi\Wb^\top\Wb}+n(\tr{\bSi}+\sigma^2)\tr{\Wb\Wb^\top}+\sigma^2\\
&=\tr{\La}-2n\tr{\B\La\B^\top\Ub\Eb\Vb^\top}+n(n+1)\tr{\B\La\B^\top\Vb\Eb^2\Vb^\top}+n(\tr{\La}+\sigma^2)\tr{\Vb\Eb^2\Vb^\top}+\sigma^2\\
% &=\tr{\La}-2n\tr{\La\Eb}+n(n+1)\tr{\La\Eb^2}+n(\tr{\La}+\sigma^2)\tr{\Eb^2}+\sigma^2
\end{align*}
}

\begin{proof}
Recall the loss function from \eqref{loss}
\begin{align*}
\Lc(\W)=\tr{\bSi}-2n\tr{\bSi\Wb}+n(n+1)\tr{\bSi\Wb^\top\Wb}+n(\tr{\bSi}+\sigma^2)\tr{\Wb\Wb^\top}+\sigma^2
\end{align*}
where $\Wb=\bSi_{\x}^{1/2}\W\bSi_{\x}^{1/2}$ and $\bSi=\bSi_{\x}^{1/2}\bSi_{\bt}\bSi_{\x}^{1/2}$. 
For any $\Wb$, let us parameterize $\Wb=\Ub\Eb\Ub^\top$ where $\Ub\in\R^{d\times r}$ denotes the eigenvectors of $\Wb$ and $\Eb\in\R^{r\times r}$ is a symmetric square matrix. We will first treat $\Ub$ as fixed and optimize $\Eb$. We will then optimize $\Ub$. Fixing $\Ub$, setting  $\bSb=\Ub^\top\bSi\Ub$ and let $M=\tr{\bSi}+\sigma^2$, we obtain
\begin{align*}
\Lc(\Eb)&=M-2n\tr{\bSb\Eb}+n(n+1)\tr{\bSb\Eb^2}+nM\tr{\Eb^2}.
\end{align*}
Differentiating, we obtain 
\[
0.5n^{-1}\nabla\Lc(\Eb)=-\bSb+(n+1)\bSb\Eb+M\Eb.
\]
Setting $\nabla\Lc(\Eb)=0$ returns
\begin{align}
\Eb^\st=(M\Iden+(n+1)\bSb)^{-1}\bSb.\label{ebst eq}
\end{align}
Let $\lab_i$ denote the $i$'th largest eigenvalue of $\bSb$. Plugging in this value, we obtain the optimal risk as a function of $\Ub$ is given by
\begin{align}
\Lc^\st(\Ub)&=M-n\cdot\tr{\bSb\Eb^\st}=M-n\cdot\tr{(M\Iden+(n+1)\bSb)^{-1}\bSb^2}\\
&=M-n\sum_{i=1}^r \frac{\lab_i^2}{(n+1)\lab_i+M}=M-n\sum_{i=1}^r \frac{\lab_i}{n+1+M\lab_i^{-1}}.
\end{align}
Now observe that, the right hand side is strictly decreasing function of the eigenvalues $\lab_i$ of $\bSb=\Ub^\top\bSi\Ub$. Thus, to minimize $\Lc^\st(\Ub)$, we need to maximize $\sum_{i=1}^r \frac{\lab_i}{n+1+M\lab_i^{-1}}$. It follows from Cauchy interlacing theorem that $\lab_j\leq \la_i$ where $\la_i$ is the $i$'th largest eigenvalue of $\bSi$ since $\bSb$ is an orthogonal projection of $\bSi$ on $\Ub$. Consequently, we find the desired bound where
\[
\Lc^\st=M-n\sum_{i=1}^r \frac{\la_{i}}{n+1+M\la_{i}^{-1}}.
\]
The equality holds by setting $\Ub$ to be the top-$r$ eigenvectors of $\bSi$ and $\Eb=\Eb^\st(\Ub)$ to be the diagonal matrix according to \eqref{ebst eq}.
\end{proof}

% \subsection{Analysis outline for general covariance}
% We can use the above strategy but we should whiten the covariances. \red{I believe the analysis below already generalizes the results of \url{https://arxiv.org/pdf/2307.03576} which assumes $\bSi=\B^{-1}$.} For instance, set $\X=\Xa\bSb$ where $\bSb=\sqrt{\bSi}$ and $\Xa$ is now $\Nn(0,1)$. Now set $\bta=\bSb\bt$ and $\btb=\bta/\tn{\bta}$. We have $\X\bt=\Xa\bSb\bt=\Xa\bta$ and set $\g=\Xa\btb\sim\Nn(0,\tn{\btb}^2\Iden)$. We similarly decompose 
% \[ 
% \Xa=\Xb+\g\btb^\top
% \] 
% where $\Xb,\g$ are independent. Set $\Sb=\bSb\B\bSb$. Noting $\E[\tn{\bt_0}^2]=\tr{\Sb}:=M$, we can then write
% \[
% \frac{1}{n}\X^\top\y=\frac{1}{n}\bSb\Xa^\top\Xa\bta\approx \bSb(\bt_0+\sqrt{\frac{M}{n}}\hb).
% \]
% The MSE error is given by (after accounting for $\x$'s covariance)
% \[ 
% \E[\tn{\bt_0-\frac{1}{n}\bSb\W\X^\top\y}^2]=\E[\tn{\bt_0-\bSb\W\bSb(\bt_0+\sqrt{\frac{M}{n}}\hb)}^2]
% \] 
% Now define the change-of-variable $\Wz=\bSb\W\bSb$. Recalling $M=\tr{\Sb}$, we can then write
% \begin{align}
% \E[\tn{\bt_0-\Wz(\bt_0+\sqrt{\frac{M}{n}}\hb)}^2]&=\E[\tn{(\Iden-\Wz)\bt_0}^2]+\frac{M}{n}\tr{\Wz\Wz^\top}\\
% &=M-2\tr{\Wz\Sb}+\tr{\Wz\Sb\Wz}+\frac{M}{n}\tr{\Wz\Wz^\top}.\label{loss function}
% \end{align}

% Differentiating, we basically obtain % and setting $\Sb=\sqrt{\Sb}$
% \[ 
% \Sb=\Sb\Wz+\frac{M}{n}\Wz\implies \Iden=(\Iden+\frac{M}{n}\Sb^{-1})\Wz\implies \Wz=(\Iden+\frac{M}{n}\Sb^{-1})^{-1}.
% \] 
% This then yields $\Ws=(\bSi+\frac{M}{n}\B^{-1})^{-1}$. This solution strictly generalizes and recovers the Identity covariance model. Crucially, through this, we can likely figure out what LoRa does. This is because performance is controlled by the combined covariance matrix $\Sb=\bSb\B\bSb$.

% \begin{lemma}[Optimizing Low-rank Attention Weights]\label{low rank attn} Suppose we use attention parameterization $\WQ,\WK\in\R^{d\times r}$ which enforces $\text{rank}(\W)\leq r$. Consider the population objective \eqref{loss}.
% % given by
% % \[ 
% % \Lc(\Wz)=\tr{\Sb}-2\tr{\Wz\Sb}+\tr{\Wz\Sb\Wz}+\frac{M}{n}\tr{\Wz\Wz^\top}.
% % \]
% Denoting $\la_i$ to be the $i$'th largest eigenvalue of $\bSi:=\bSi_{\x}^{1/2}\bSi_{\bt}\bSi_{\x}^{1/2}$, we have that 
% \[
% \min_{\text{rank}(\W)\leq r}\Lc(\W)=\tr{\bSi_{\x}\bSi_{\bt}}+\sigma^2-\sum_{i=1}^r\frac{n\la_i^2}{(n+1)\la_i+\tr{\bSi_{\x}\bSi_{\bt}}+\sigma^2}.
% \]
% % Noting $\tr{\bSi_{\x}\bSi_{\bt}}=\sum_{i=1}^d\la_i$ and removing the rank constraint, this reduces to the standard optimal risk
% % \[ 
% % \min_{\W}\Lc(\W)=\sum_{i=1}^d\frac{1}{n/M+1/\la_i}.
% % \]
% \end{lemma}
% \begin{proof}\redp{OLD PROOF: There are mistakes and typos such as applying interlacing to diagonal entries of $\Eb$ or calling $\la_i$ eigenvalue of $\Wb$.} Recall the loss function from \eqref{loss}
% \begin{align*}
% \Lc(\W)=\tr{\bSi}-2n\tr{\bSi\Wb}+n(n+1)\tr{\bSi\Wb^\top\Wb}+n(\tr{\bSi}+\sigma^2)\tr{\Wb\Wb^\top}+\sigma^2
% \end{align*}
% where $\Wb=\bSi_{\x}^{1/2}\W\bSi_{\x}^{1/2}$ and $\bSi=\bSi_{\x}^{1/2}\bSi_{\bt}\bSi_{\x}^{1/2}$. 
% For any $\Wb$, let us parameterize $\Wb=\Ub\Eb\Ub^\top$ where $\Ub\in\R^{d\times r}$ denotes the eigenvectors of $\Wb$ and $\Eb\in\R^{r\times r}$ is a diagonal matrix with non-increasing diagonal entries. We will first treat $\Ub$ as fixed and optimize $\Eb$. We will then optimize $\Ub$. Fixing $\Ub$, setting  $\bSb=\Ub^\top\bSi\Ub$ and let $M=\tr{\bSi}+\sigma^2$, we obtain
% \begin{align*}
% \Lc(\Eb)&=M-2n\tr{\bSb\Eb}+n(n+1)\tr{\bSb\Eb^2}+nM\tr{\Eb^2}\\
% &=M-2n\sum_{i=1}^r\Eb_{i}\bSb_{ii} +n(n+1)\sum_{i=1}^r\Eb_{i}^2\bSb_{ii}+nM\sum_{i=1}^r\Eb^2_i
% \end{align*}
% %     and setting $\Sbb=\Ub^\top\Sb\Ub$ and setting $\Lc'(\Eb)=\Lc(\Wz)-\tr{\Sb}$, we have that 
% % \begin{align}
% % \Lc'(\Eb)&=\tr{\Sbb\Eb^2}+\frac{M}{n}\tr{\Eb^2}-2\tr{\Eb\Sbb}.
% % \end{align}
% where $\bSb_{ii}$ and $\Eb_i$ are the $i$'th diagonal value of $\bSb$ and $\Eb$, respectively. Differentiating, we obtain 
% \[
% \frac{\partial\Lc(\Eb)}{\partial\Eb_i}=-2n\bSb_{ii}+2n(n+1)\bSb_{ii}\Eb_i+2nM\Eb_i.
% \]
% Setting $\frac{\partial\Lc(\Eb)}{\partial\Eb_i}=0$ returns
% \[
% \Eb_i^\st=\frac{\bSb_{ii}}{(n+1)\bSb_{ii}+M}.
% \]
% % $$\Eb_\st(\Ub)=\left((n+1)\Iden+(\tr{\bSi}+\sigma^2)\bSb^{-1}\right)^{-1}.$$
% % Let $\s_i$ denote the eigenvalues of $\Sbb$. 
% Plugging in this value, we obtain the optimal risk given by
% \[ 
% \Lc^\st:=\Lc^\st(\Ub)=M-n\sum_{i=1}^r \frac{\bSb_{ii}^2}{(n+1)\bSb_{ii}+M}=M-n\sum_{i=1}^r \frac{\bSb_{ii}}{(n+1)+M\bSb_{ii}^{-1}}.
% \]
% Now observe that, the right hand side is strictly decreasing function of the diagonal value $\bSb_{ii}$ of $\bSb=\Ub^\top\bSb\Ub$. Thus, to minimize $\Lc^\st(\Ub)$, we need to maximize $\sum_{i=1}^r\frac{n\bSb_{ii}}{M/\bSb_{ii}+n+1}$. It follows from Cauchy's interlace theorem that $\bSb_{ii}\leq \la_i$ where $\la_i$ is the $i$'th largest eigenvalue of $\Wb$ since $\bSb$ is an orthogonal projection of $\Wb$ on $\Ub$. Consequently, we find the desired bound where
% \[
% \Lc^\st=M-n\sum_{i=1}^r \frac{\la_{i}}{n+1+M\la_{i}^{-1}}.
% \]
% \end{proof}
% \begin{proof} 
% Let us parameterize $\Wz=\Ub\Eb\Ub^\top$ where $\Ub\in\R^{d\times r}$ is the eigenvectors of $\Wz$. We will first treat $\Ub$ as fixed and optimize $\Eb\in\R^{r\times r}$. We will then optimize $\Ub$. Fixing $\Ub$ and setting $\Sbb=\Ub^\top\Sb\Ub$ and setting $\Lc'(\Eb)=\Lc(\Wz)-\tr{\Sb}$, we have that 
% \begin{align}
% \Lc'(\Eb)&=\tr{\Sbb\Eb^2}+\frac{M}{n}\tr{\Eb^2}-2\tr{\Eb\Sbb}.
% \end{align}
% Differentiating, we obtain $\Eb^*=(\Iden+\frac{M}{n}\Sbb^{-1})^{-1}$. Let $\s_i$ denote the eigenvalues of $\Sbb$. Plugging in this value, we obtain the optimal risk given by
% \[ 
% \Lc^*:=\Lc^*(\Ub)=-\sum_{i=1}^r s_i (1+\frac{M}{ns_i})^{-1}=-\sum_{i=1}^r\frac{ns_i}{M/s_i+n}.
% \]
% Now observe that, the right hand side is strictly decreasing function of the eigenvalues $s_i$ of $\Ub^\top\Sb\Ub$. Thus, to minimize $\Lc^*(\Ub)$, we need to maximize $\sum_{i=1}^r\frac{ns_i}{M/s_i+n}$. It follows from Cauchy's interlace theorem that $s_i\leq \la_i$ where $\la_i$ is the $i$th largest eigenvalue of $\Sb$ since $\Sbb$ is an orthogonal projection of $\Sb$ on $\Ub$. Consequently, we find the desired bound.
% \end{proof}

\begin{comment}
\noindent\textbf{Impact of LoRA:} Suppose the model is well-pretrained over the $\bSi_{\x}$ and $\bSi_{\bt}$. Then we have obtained $\Wb_\st=\left((n+1)\Iden+(d+\sigma^2)\Iden\right)^{-1}:=\alpha\Iden$. Then consider a low-rank $\W_0$ with $\rank{\W_0}\leq  r$, we have
\begin{align*}
\Lc(\W+\W_0)&=M-2n\tr{\bSi(\W+\W_0)}\\
&\quad+n(n+1)\tr{\bSi(\W+\W_0)^\top(\W+\W_0)}+nM\tr{(\W+\W_0)(\W+\W_0)^\top}\\
&=\left(M-2n\tr{\bSi\W}+n(n+1)\tr{\bSi\W^\top\W}+nM\tr{\W\W^\top}\right)\\
&\quad+\left(-2n\tr{\bSi\W_0}+n(n+1)\tr{\bSi(2\W^\top\W_0+\W_0^\top\W_0)}+nM\tr{2\W^\top\W_0+\W^\top\W_0}\right)\\
&=\Lc(\W)+\left(-2n\tr{\bSi\W_0}+2n(n+1)\tr{\bSi\W^\top\W_0}+2nM\tr{\W^\top\W_0}\right)\\
&\quad+n(n+1)\tr{\bSi\W_0^\top\W_0}+nM\tr{\W^\top\W_0}\\
&=\Lc(\W)+\left(-2n\tr{\bSb\La}+2n(n+1)\tr{\bSb\Wb^\top\La}+2nM\tr{\Wb^\top\La}\right)\\
&\quad+n(n+1)\tr{\bSb\La^2}+nM\tr{\La^2}\\
&=\Lc(\W)+\left(-2n\tr{\bSb\La}+2\alpha n(n+1)\tr{\bSb\La}+2\alpha nM\tr{\La}\right)\\
&\quad+n(n+1)\tr{\bSb\La^2}+nM\tr{\La^2}
\end{align*}
Differentiating, we obtain 
\[
\La^\st=((n+1)\bSb+M\Iden)^{-1}\left(\bSb-(n+1)\bSb\Wb-M\Wb\right).
\]
Then
\[
\Lc(\La^\st)=\Lc(\W)-n\sum_{i=1}^r \frac{\left(\bSb-(n+1)\bSb\Wb-M\Wb\right)_{ii}^2}{(n+1)\bSb_{ii}+M}
\]

Suppose $\Wb=\alpha\Iden$. Then $\La^\st=((n+1)\bSb+M\Iden)^{-1}\left((1-\alpha(n+1))\bSb-\alpha M\Iden\right)$ and
\[
\Lc(\La^\st)=\Lc(\W)-n\sum_{i=1}^r \frac{\left(\bSb_{ii}-\alpha(n+1)\bSb_{ii}-\alpha M\right)^2}{(n+1)\bSb_{ii}+M}
\]
\[
\frac{d^2}{(n+d+1)^2(n+1)}\frac{\left(\bSb_{ii}- M/d\right)^2}{\bSb_{ii}+M/(n+1)}
\]

\[
\bSb_{ii}+M/(n+1)+\frac{\left( M/d+M/(n+1)\right)^2}{\bSb_{ii}+M/(n+1)}
\]
\[
\bSb_{ii}=M/d=\tr{\bSi}/d
\]
\end{comment}

% \noindent\textbf{Impact of LoRA:} Based on Lemma \ref{low rank attn}, under jointly-diagonalizable new and old eigenvalues of $\Sb,\Sb^{old}$ $(\la_i)_{i=1}^d,(\la_i^{old})_{i=1}^d$; LoRA obtains top $r$ eigenvalue indices $\Ic$ maximizing the function $\texttt{gain}_i=\frac{1}{n/M+1/\la^{old}_i}-\frac{1}{n/M+1/\la_i}$. That means, LoRA's risk is given by
% \[ 
% \Lc(\W_{lora})=\min_{|\Ic|\leq r,\Ic\subset[d]}\sum_{i\in\Ic}\frac{1}{n/M+1/\la_i}+\sum_{i\not\in\Ic}\frac{1}{n/M+1/\la^{old}_i}
% \]
% Note that, this only provides a lower bound as we have to prove that the optimal LoRA-updated model $\W_{lora}$ is also jointly diagonalizable with covariances $\Sb,\Sb^{old}$, and $\W^{old}$.


\begin{comment}
and letting $s_i=\Sbb_{ii}$, we have that
\begin{align}
\Lc'(\La)&=\tr{\Sbb\La^2}+\frac{M}{n}\tr{\La^2}-2\tr{\La\Sbb}\\
&=\sum_{i=1}^r \la_i^2(\frac{M}{n}+s_i)-2\la_is_i.
\end{align}
Differentiating, we obtain $\la^*_i=(1+\frac{M}{ns_i})^{-1}=s_i(s_i+\frac{M}{n})^{-1}$. Next, let us study the risk which is given by plugging the optimal $\La^*$
\[ 
\Lc^*=-\sum_{i=1}^d s_i (1+\frac{M}{ns_i})^{-1}=-\sum_{i=1}^d\frac{ns_i}{M/s_i+n}.%-\sum_{i=1}^d\frac{ns_i^2}{M+ns_i}=
\]
\noindent\red{\textbf{Basic LoRa analysis:}} Assume that new and old covariances are jointly diagonalizable (e.g.~$\bSi_{old},\bSi_{new}$). Write the loss function \eqref{loss function} in terms of a sum over eigenvalues. Then determine which $r$ eigenvalues of the old distribution's $\W_{\text{old}}$ should be updated and matched to new optimal $\W_{new}$ by LoRa.

Exact LoRa objective is: Suppose $\Wz$ is fixed
\begin{align}
\Lc(\Lb)=M-2\tr{(\Wz+\Lb)\Sb}+\tr{(\Wz+\Lb)\Sb(\Wz+\Lb)}+\frac{M}{n}\tr{(\Wz+\Lb)(\Wz+\Lb)^\top}.\label{loss function}
\end{align}
If $\Lb$ was full rank, solution is $\Lb_\st=(\Iden+\frac{M}{n}\Sb^{-1})^{-1}-\Wz$.
\end{comment}





==> app/proof_rag.tex <==
\section{Retrieval augmented generation with $\alpha$ correlation}
\label{app:rag}

In this section, we consider the retrieval augmented generation linear model. In this model, we draw the query vector $\x$ and task vector $\bt$ via
\[
\x\sim\Nc(0,\Iden)\quad\text{and}\quad\bt\sim\Nc(0,\Iden).
\]
We then draw data $(\x_i)_{i=1}^n$ to be used in-context according to the rule $\text{corr\_coef}(\x,\x_i)\geq \alpha>0$. Hence, we sample 
\[
\x_i\sim\Nn(\alpha\x,\gamma^2\Iden),\quad\xi_i\sim\Nc(0,\sigma^2)\quad\text{and}\quad y_i=\x_i^\top \bt+\xi_i,
\]
and we can rewrite 
\[
\g_i\sim\Nc(0,\Iden),\quad\xi_i\sim\Nc(0,\sigma^2)\quad\text{and}\quad\x_i=\alpha\x+\gamma\g_i,\quad y_i=(\alpha\x+\gamma\g_i)^\top\bt+\xi_i.
\]
% Then recap the loss function from \eqref{gd} and let $\bxi=[\xi_1~\cdots~\xi_n]^\top$, $\Gb=[\g_1~\cdots~\g_n]^\top$ where we have 
% \[
% \X=\alpha\onebb\x^\top+\Gb\quad\text{and}\quad\y=\X\bt+\bxi=(\alpha\onebb\x^\top+\Gb)\bt+\bxi.
% \]
Then we obtain
\begin{align}
    \Lc(\W)&=\E\left[(y-g(\Z))^2\right]\nn\\
    &=\E\left[\left(\x^\top\bt+\xi-\x^\top\W\X^\top(\X\bt+\bxi)\right)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2+2(\x^\top\bt-\x^\top\W\X^\top\X\bt)(\xi-\x^\top\W\X^\top\bxi)+(\xi-\x^\top\W\X^\top\bxi)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+\E\left[(\x^\top\W\X^\top\bxi)^2\right]+\sigma^2\nn.
    % &=\E\left[\tn{\x-(\x^\top\W\X^\top\X)^\top}^2\right]+\E\left[(\x^\top\W\X^\top\bxi)^2\right]+\sigma^2\nn.
    % &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2,\nn\\
    % &=\E\left[\tn{\bt-\W\X^\top\X\bt}^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2.\label{ind loss}
\end{align}
We first focus on 
\begin{align*}
    \E\left[(\x^\top\W\X^\top\bxi)^2\right]&=\E\left[\left(\sum_{i=1}^n{\xi_i}\x^\top\W(\alpha\x+\gamma\g_i)\right)^2\right]\\
    &=n\sigma^2\E\left[\x^\top\W(\alpha\x+\gamma\g)(\alpha\x+\gamma\g)^\top\W^\top\x\right]\\
    &=n\sigma^2\left(\alpha^2\E[\x^\top\W\x\x^\top\W^\top\x]+\gamma^2\E[\x^\top\W\g\g^\top\W^\top\x]\right)\\
    &=n\sigma^2\left(\alpha^2(M_1+M_2+M_3)+\gamma^2M_2\right).
\end{align*}
Next, consider the following
\begin{align*}
    \x^\top\W\X^\top\X\bt&=\x^\top\W(\alpha\onebb\x^\top+\Gb)^\top(\alpha\onebb\x^\top+\Gb)\bt\\
    &=\alpha^2n\x^\top\W\x\x^\top\bt+\alpha\x^\top\W(\x\onebb^\top\Gb+\Gb^\top\onebb\x^\top)\bt+\x^\top\W\Gb^\top\Gb\bt.
\end{align*}
Next, consider the following
\begin{align*}
    \E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]&=\underset{(a)}{\underbrace{\E\left[(\x^\top\bt)^2\right]}}+\underset{(b)}{\underbrace{\E\left[(\x^\top\W\X^\top\X\bt)^2\right]}}-2\underset{(c)}{\underbrace{\E\left[\x^\top\bt\x^\top\W\X^\top\X\bt\right]}}
\end{align*}
\begin{align*}
    (a):\quad&\E\left[(\x^\top\bt)^2\right]=d\\
    (b):\quad&\E\left[(\x^\top\W\X^\top\X\bt)^2\right]=\E\left[\left(\x^\top\W\sum_{i=1}^n(\alpha\x+\gamma\g_i)(\alpha\x+\gamma\g_i)^\top\bt\right)^2\right]\\
    &=\E\left[\left(\sum_{i=1}^n\x^\top\W(\alpha^2\x\x^\top+\gamma^2\g_i\g_i^\top+\alpha\gamma\x\g_i^\top+\alpha\gamma\g_i\x^\top)\bt\right)^2\right]\\
    &=\alpha^4n^2\E\left[(\x^\top\W\x\x^\top\bt)^2\right]+\gamma^4\E\left[\left(\sum_{i=1}^n\x^\top\W\g_i\g_i^\top\bt\right)^2\right]\\
    &\quad+\alpha^2\gamma^2\E\left[\left(\sum_{i=1}^n\x^\top\W\x\g_i^\top\bt\right)^2\right]+\alpha^2\gamma^2\E\left[\left(\sum_{i=1}^n\x^\top\W\g_i\x^\top\bt\right)^2\right]\\
    &\quad+2\alpha^2\gamma^2n^2\E\left[\x^\top\W\x\x^\top\bt\bt^\top\g\g^\top\W^\top\x\right]+2\alpha^2\gamma^2 n\E\left[\x^\top\W\x\g^\top\bt\x^\top\W\g\x^\top\bt\right]\\
    &=\alpha^4n^2(d+4)(M_1+M_2+M_3)+\gamma^4n(d+n+1)M_2\\
    &\quad+\alpha^2\gamma^2nd(M_1+M_2+M_3)+\alpha^2\gamma^2n(d+2)M_2\\
    &\quad+2\alpha^2\gamma^2n^2(M_1+M_2+M_3)+2\alpha^2\gamma^2n(M_1+M_2+M_3)\\
    &=A_1M_1+A_2M_2+A_3M_3\\
    (c):\quad&\E\left[\x^\top\bt\x^\top\W\X^\top\X\bt\right]=\E\left[\sum_{i=1}^n\x^\top\bt\x^\top\W(\alpha\x+\gamma\g_i)(\alpha\x+\gamma\g_i)^\top\bt\right]\\
    &=\E\left[\sum_{i=1}^n\x^\top\bt\x^\top\W(\alpha^2\x\x^\top+\gamma^2\g_i\g_i^\top+\alpha\gamma\x\g_i^\top+\alpha\gamma\g_i\x^\top)\bt\right]\\
    &=\alpha^2n\E\left[\x^\top\bt\x^\top\W\x\x^\top\bt\right]+\gamma^2n\E\left[\x^\top\bt\x^\top\W\g\g^\top\bt\right]\\
    &=\alpha^2n(d+2)\tr{\W}+\gamma^2n\tr{\W}\\
    &=A_4\tr{\W}
\end{align*}
\begin{align*}
    \nabla\Lc(\W)=0\\
    2A_1\tr{\W}\Iden+2A_2\W+2A_3\W^\top-2A_4\Iden+n\sigma^2\left(\alpha^2(2\tr{\W}\Iden+2\W+2\W^\top)+2\gamma^2\W\right)=0\\
    (dA_1+A_2+A_3+n\sigma^2(\alpha^2(d+2)+\gamma^2))\tr{\W}=A_4d\\
    \W_\st=c\Iden\Longrightarrow c=\frac{A_4}{dA_1+A_2+A_3+n\sigma^2(\alpha^2(d+2)+\gamma^2)}\\
    c=\frac{n(\alpha^2(d+2)+\gamma^2)}{\alpha^4n^2(d+2)(d+4)+\alpha^2\gamma^2n(d+2)(d+2n+3)+\gamma^4n(d+n+1)+n\sigma^2(\alpha^2(d+2)+\gamma^2)}\\
    c\approx\frac{\bar d+\gamma^2}{n\bar d^2+\bar d\gamma^2(d+2n+3)+\gamma^4(d+n+1)+\sigma^2(\bar d+\gamma^2)}
\end{align*}
\[
\Lc_\st = d+(dA_1+A_2+A_3)c^2d-2A_4cd
\]
 


% \section{Retrieval augmented generation with $\alpha$ correlation}
% \label{app:rag}

% In this section, we consider the retrieval augmented generation linear model. In this model, we draw the query vector $\x$ and task vector $\bt$ via
% \[
% \x\sim\Nc(0,\Iden)\quad\text{and}\quad\bt\sim\Nc(0,\Iden).
% \]
% We then draw data $(\x_i)_{i=1}^n$ to be used in-context according to the rule $\text{corr\_coef}(\x,\x_i)\geq \alpha>0$. Hence, we sample 
% \[
% \x_i\sim\Nn(\alpha\x,(1-\alpha^2)\Iden),\quad\xi_i\sim\Nc(0,\sigma^2)\quad\text{and}\quad y_i=\x_i^\top \bt+\xi_i,
% \]
% and we can rewrite 
% \[
% \g_i\sim\Nc(0,(1-\alpha^2)\Iden),\quad\xi_i\sim\Nc(0,\sigma^2)\quad\text{and}\quad\x_i=\alpha\x+\g_i,\quad y_i=(\alpha\x+\g_i)^\top\bt+\xi_i.
% \]
% Then recap the loss function from \eqref{gd} and let $\bxi=[\xi_1~\cdots~\xi_n]^\top$, $\Gb=[\g_1~\cdots~\g_n]^\top$ where we have 
% \[
% \X=\alpha\onebb\x^\top+\Gb\quad\text{and}\quad\y=\X\bt+\bxi=(\alpha\onebb\x^\top+\Gb)\bt+\bxi.
% \]
% Then we obtain
% \begin{align}
%     \Lc(\W)&=\E\left[(y-g(\Z,\x))^2\right]\nn\\
%     &=\E\left[\left(\x^\top\bt+\xi-\x^\top\W\X^\top(\X\bt+\bxi)\right)^2\right]\nn\\
%     &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2+2(\x^\top\bt-\x^\top\W\X^\top\X\bt)(\xi-\x^\top\W\X^\top\bxi)+(\xi-\x^\top\W\X^\top\bxi)^2\right]\nn\\
%     &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+\E\left[(\x^\top\W\X^\top\bxi)^2\right]+\sigma^2\nn.
%     % &=\E\left[\tn{\x-(\x^\top\W\X^\top\X)^\top}^2\right]+\E\left[(\x^\top\W\X^\top\bxi)^2\right]+\sigma^2\nn.
%     % &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2,\nn\\
%     % &=\E\left[\tn{\bt-\W\X^\top\X\bt}^2\right]+n\sigma^2\cdot\trace{\W\W^\top}+\sigma^2.\label{ind loss}
% \end{align}
% We first focus on 
% \begin{align*}
%     \E\left[(\x^\top\W\X^\top\bxi)^2\right]&=\E\left[(\x^\top\W(\alpha\onebb\x^\top+\Gb)^\top\bxi)^2\right]\\
%     &=\alpha^2\E\left[(\x^\top\W\x\onebb^\top\bxi)^2\right]+\E\left[(\x^\top\W\Gb^\top\bxi)^2\right]\\
%     &=n\alpha^2\sigma^2\trace{\W}^2+n\sigma^2(1-\alpha^2)\trace{\W\W^\top}.
% \end{align*}
% Next, consider the following
% \begin{align*}
%     \x^\top\W\X^\top\X\bt&=\x^\top\W(\alpha\onebb\x^\top+\Gb)^\top(\alpha\onebb\x^\top+\Gb)\bt\\
%     &=\alpha^2n\x^\top\W\x\x^\top\bt+\alpha\x^\top\W(\x\onebb^\top\Gb+\Gb^\top\onebb\x^\top)\bt+\x^\top\W\Gb^\top\Gb\bt.
% \end{align*}
% {\color{red}
% Next, consider the following
% \begin{align*}
%     \x^\top\W\X^\top\X\bt-\x^\top\bt&=\x^\top\W(\alpha\onebb\x^\top+\gamma\Gb)^\top(\alpha\onebb\x^\top+\gamma\Gb)\bt-\x^\top\bt\\
%     &=\alpha^2n\x^\top\W\x\x^\top\bt+\alpha\gamma\x^\top\W(\x\onebb^\top\Gb+\Gb^\top\onebb\x^\top)\bt+\x^\top(\gamma^2\W\Gb^\top\Gb-\Iden)\bt.
% \end{align*}
% \begin{align*}
%     &\E\left[({\x^\top\bt-\x^\top\W\X^\top\X\bt})^2\right]\\
%     &=\E\left[({\alpha^2n\x^\top\W\x\x^\top\bt+\alpha\gamma\x^\top\W(\x\onebb^\top\Gb+\Gb^\top\onebb\x^\top)\bt+\x^\top(\gamma^2\W\Gb^\top\Gb-\Iden)\bt})^2\right]\\
%     &=\alpha^4n^2\underset{(a)}{\underbrace{\E\left[({\x^\top\W\x\x^\top\bt})^2\right]}}+\alpha^2\gamma^2\underset{(b)}{\underbrace{\E\left[({\x^\top\W(\x\onebb^\top\Gb+\Gb^\top\onebb\x^\top)\bt})^2\right]}}+\underset{(c)}{\underbrace{\E\left[({\x^\top(\gamma^2\W\Gb^\top\Gb-\Iden)\bt})^2\right]}}\\&\quad+2\alpha^2n\underset{(d)}{\underbrace{\E\left[(\x^\top\W\x\x^\top\bt)^\top(\x^\top(\gamma^2\W\Gb^\top\Gb-\Iden)\bt)\right]}}
% \end{align*}
% \begin{align*}
%     &\E\left[({\x^\top\W\x\x^\top\bt})^2\right]\\
%     &=\E\left[{\x^\top\W\x\x^\top}\x\x^\top\W^\top\x\right]\\
%     &=\E\left[\left(\sum_{i=1}^dx_i^2\right)\left(\sum_{i,j=1}^dx_ix_j w_{ij}\right)^2\right]\\
%     &=\E\left[\left(\sum_{i=1}^dx_i^2\right)\left(\sum_{i=1}^dx_i^4 w_{ii}^2+\sum_{i\neq j}x_i^2x_j^2(w_{ii}w_{jj}+w_{ij}w_{ij}+w_{ij}w_{ji})\right)\right]\\
%     &=\E\left[\left(\sum_{i=1}^dx_i^2\right)\left(\sum_{i=1}^dx_i^4 w_{ii}^2\right)\right]+\E\left[\left(\sum_{i=1}^dx_i^2\right)\left(\sum_{i\neq j}x_i^2x_j^2(w_{ii}w_{jj}+w_{ij}w_{ij}+w_{ij}w_{ji})\right)\right]\\
%     &=(d+4)\left(\tr{\W}^2+\tr{\W\W^\top}+\tr{\W^2}\right)
% \end{align*}
% \begin{align*}
%     &\E\left[\left(\sum_{i=1}^dx_i^2\right)\left(\sum_{i=1}^dx_i^4 w_{ii}^2\right)\right]=\E\left[\sum_{i=1}^dx_i^6w_{ii}^2+\sum_{i\neq j}x_i^4x_j^2w_{ii}^2\right]\\
%     &=\sum_{i=1}^d(15+3(d-1))w_{ii}^2\\
%     &=3(d+4)\sum_{i=1}^dw_{ii}^2
% \end{align*}
% \begin{align*}
%     &\E\left[\left(\sum_{i=1}^dx_i^2\right)\left(\sum_{i\neq j}x_i^2x_j^2(w_{ii}w_{jj}+w_{ij}w_{ij}+w_{ij}w_{ji})\right)\right]\\
%     &=\E\left[\sum_{i\neq j}(x_i^4x_j^2+x_{i}^2x_j^4+\sum_{k\neq i,j}x_i^2x_j^2x_k^2)(w_{ii}w_{jj}+w_{ij}w_{ij}+w_{ij}w_{ji})\right]\\
%     &=(d+4)\sum_{i\neq j}(w_{ii}w_{jj}+w_{ij}w_{ij}+w_{ij}w_{ji})
% \end{align*}
% \begin{align*}
%     &\E\left[({\x^\top\W(\x\onebb^\top\Gb+\Gb^\top\onebb\x^\top)\bt})^2\right]\\
%     &=\E\left[\x^\top\W(\x\onebb^\top\Gb+\Gb^\top\onebb\x^\top)(\x\onebb^\top\Gb+\Gb^\top\onebb\x^\top)\W^\top\x\right]\\
%     &=\E\left[\x^\top\W\x\onebb^\top\Gb\x\onebb^\top\Gb\W^\top\x\right]+\E\left[\x^\top\W\x\onebb^\top\Gb\Gb^\top\onebb\x^\top\W^\top\x\right]\\
%     &\quad+\E\left[\x^\top\W\Gb^\top\onebb\x^\top\x\onebb^\top\Gb\W^\top\x\right]+\E\left[\x^\top\W\Gb^\top\onebb\x^\top\Gb^\top\onebb\x^\top\W^\top\x\right]\\
%     &=3n\gamma^2\E\left[\x^\top\W\x\x^\top\W^\top\x\right]+n\gamma^2\E\left[(\x^\top\x)\x^\top\W\W^\top\x\right]\\
%     &=3n\gamma^2\E\left[\left(\sum_{i,j=1}^dx_ix_jw_{ij}\right)^2\right]+n\gamma^2\E\left[\left(\sum_{i=1}^dx_i^2\right)\sum_{i,j=1}^dx_ix_j\bar w_{ij}\right]\\
%     &=3n\gamma^2\E\left[\left(\sum_{i=1}^dx_i^4 w_{ii}^2+\sum_{i\neq j}x_i^2x_j^2(w_{ii}w_{jj}+w_{ij}w_{ij}+w_{ij}w_{ji})\right)\right]+n\gamma^2\E\left[\left(\sum_{i=1}^dx_i^2\right)\left(\sum_{i=1}^dx_i^2\bar w_{ii}\right)\right]\\
%     &=3n\gamma^2\E\left[\left(\sum_{i=1}^dx_i^4 w_{ii}^2+\sum_{i\neq j}x_i^2x_j^2(w_{ii}w_{jj}+w_{ij}w_{ij}+w_{ij}w_{ji})\right)\right]+n\gamma^2\E\left[\left(\sum_{i=1}^dx_i^4\bar w_{ii}+\sum_{i\neq j}x_i^2x_j^2\bar w_{ii}\right)\right]\\
%     &=3n\gamma^2\left(3\sum_{i=1}^dw_{ii}^2+\sum_{i\neq j}(w_{ii}w_{jj}+w_{ij}w_{ij}+w_{ij}w_{ji})\right)+n\gamma^2\left(3\sum_{i=1}^d\bar w_{ii}+(d-1)\sum_{i=1}^d\bar w_{ii}\right)\\
%     &=3n\gamma^2\left(\tr{\W}^2+\tr{\W\W^\top}+\tr{\W^2}\right)+n\gamma^2(d+2)\tr{\W\W^\top}
% \end{align*}
% \begin{align*}
%     \E\left[({\x^\top(\W\Gb^\top\Gb-\Iden)\bt})^2\right]&=\tr{\E\left[(\W\Gb^\top\Gb-\Iden)(\W\Gb^\top\Gb-\Iden)^\top\right]}\\
%     &=n\gamma^2(3\gamma^2+n+d-2)\tr{\W\W^\top}-2n\gamma^2\tr{\W}+d
% \end{align*}
% \begin{align*}
%     &\E\left[(\x^\top\W\x\x^\top\bt)^\top(\x^\top(\W\Gb^\top\Gb-\Iden)\bt)\right]\\
%     &=\tr{\E\left[\x\x^\top\W^\top\x\x^\top(\W\Gb^\top\Gb-\Iden)\right]}\\
%     &=n\gamma^2\tr{\E\left[\x\x^\top\W^\top\x\x^\top\W\right]}-\tr{\E\left[\x\x^\top\W^\top\x\x^\top\right]}\\
%     &=n\gamma^2\left(\tr{\W}^2+\tr{\W\W^\top}+\tr{\W}\right)+n(d+2)\tr{\W}
% \end{align*}
% Combining all results in 
% \begin{align*}
%     &\E\left[({\x^\top\bt-\x^\top\W\X^\top\X\bt})^2\right]\\
%     &=\alpha^2n^2(d+4)\left(\tr{\W}^2+\tr{\W\W^\top}+\tr{\W^2}\right)\\
%     &\quad+\alpha\left(3n\gamma^2\left(\tr{\W}^2+\tr{\W\W^\top}+\tr{\W^2}\right)+n\gamma^2(d+2)\tr{\W\W^\top}\right)\\
%     &\quad +n\gamma^2(3\gamma^2+n+d-2)\tr{\W\W^\top}-2n\gamma^2\tr{\W}+d\\
%     &\quad+2\alpha^2\left(n\gamma^2\left(\tr{\W}^2+\tr{\W\W^\top}+\tr{\W}\right)+n(d+2)\tr{\W}\right)\\
%     &=(\alpha^2n^2(d+4)+3\alpha n\gamma^2+2\alpha^2n\gamma^2)\tr{\W}^2
% \end{align*}
% }

% Consider the following orthogonal decomposition: Let $\btb=\bt/\tn{\bt}$, $\g'=\Gb\btb$, $\Gbb=\Gb-\Gb\btb\btb^\top=\Gb-\g'\btb^\top$, and observe that $\g',\Gbb$ are independent conditioned on $\btb$, $(\bt,\Gbb)$ are orthogonal, and $\Gb=\Gbb+\g'\btb^\top$. We obtain
% \begin{align*}
%     \Gb^\top\Gb\bt=(\Gbb+\g'\btb^\top)^\top\g'\tn{\bt}=\tn{\bt}\Gbb^\top\g'+\tn{\g'}^2\bt.
% \end{align*}
% Note that $\g'\sim\Nn(0,(1-\alpha^2)\Iden)$ conditioned on $\bt$. Additionally $\Gbb$ is effectively a $n\times (d-1)$ standard normal as its rows lie over the $d-1$ dimensional subspace $\bPi=\Iden-\btb\btb^\top$.
% %using $\tn{\bt}\approx\sqrt{d}$, the right hand side is approximately distributed as $\Nn(n\bt,nd\Iden_d)$. 


% % Here recall from \eqref{decomp XXB}, 
% Therefore, we have
% \[
% \frac{1}{n(1-\alpha^2)}\Gb^\top\Gb\bt\approx\bt+\sqrt{\frac{d}{n}}\hb,\quad\text{where}\quad\hb\sim\Nc(0,\Iden)
% \]
% and $\Gb^\top\onebb$ is distributed as $\Nc(0,n\Iden)$ and let $\Gb^\top\onebb\approx\sqrt{n}\tilde\g$. Additionally, we approximate the $\W$-weighted inner-products of $\x,\bar{\g}$ as a constant and independent noise scalar $\gamma$ as follows
% \begin{align*}
% &\x^\top\W\x\approx\trace{\W}\quad\text{and}\\
% &\x^\top\W\tilde\g\approx\|\W\|_F\gamma\quad\text{where}\quad\E[\gamma]=0,~\E[\gamma^2]=1.
% \end{align*}
% Then, 
% \begin{align*}
%     \frac{1}{n}\x^\top\W\X^\top\X\bt&\approx\alpha^2\x^\top\W\x\x^\top\bt+\frac{\alpha}{\sqrt{n}}\x^\top\W\x\tilde\g^\top\bt+\frac{\alpha}{\sqrt{n}}\x^\top\W\tilde\g\x^\top\bt+(1-\alpha^2)\x^\top\W\left(\bt+\sqrt{\frac{d}{n}}\hb\right)\\
%     &\approx\alpha^2\trace{\W}\x^\top\bt+\frac{\alpha}{\sqrt{n}}\trace{\W}\tilde\g^\top\bt+\frac{\alpha}{\sqrt{n}}\|{\W}\|_F\gamma\x^\top\bt+(1-\alpha^2)\x^\top\W\left(\bt+\sqrt{\frac{d}{n}}\hb\right)\\
%     &\approx \x^\top\left(\alpha^2\trace{\W}+(1-\alpha^2)\W\right)\bt+(1-\alpha^2)\sqrt{\frac{d}{n}}\x^\top\W\hb+\frac{\alpha\cdot\trace{\W}}{\sqrt{n}}\tilde \g^\top\bt+\frac{\alpha\|\W\|_F\gamma}{\sqrt{n}}\x^\top\bt
% \end{align*}
% Therefore,
% \begin{align*}
%     &\E\left[(\x^\top\bt-\frac{1}{n}\x^\top\W\X^\top\X\bt)^2\right]\\
%     &\approx\trace{\left(\left(1-\alpha^2\cdot\trace{\W}\right)\Iden-(1-\alpha^2)\W\right)\left(\left(1-\alpha^2\cdot\trace{\W}\right)\Iden-(1-\alpha^2)\W\right)^\top}\\
%     &\quad+(1-\alpha^2)^2\frac{d}{n}\trace{\W\W^\top}+\frac{\alpha^2d\cdot\trace{\W}^2}{n}+\frac{\alpha^2d\cdot\|\W\|_F^2}{n}\\
%     &=\left(\alpha^4d+2\alpha^2(1-\alpha^2)+\frac{\alpha^2d}{n}\right)\trace{\W}^2+\left((1-\alpha^2)^2(1+\frac{d}{n})+\frac{\alpha^2d}{n}\right)\trace{\W\W^\top}-2(\alpha^2d+1-\alpha^2)\trace{\W}+d.
%     % \\
%     % &\approx\alpha^2(2+(d-2)\alpha^2+\frac{d}{n})\trace{\W}^2+(1-\alpha^2)^2\left(1+\frac{d}{n}\right)\trace{\W\W^\top}+\\
%     % &\approx n^2(1-\alpha^2)^2\trace{\W\W^\top}+n^2\alpha^4\cdot\trace{\W}^2-2n^2\alpha^2(1-\alpha^2)\trace{\W}^2+(1-\alpha^2)^2dn\cdot\trace{\W\W^\top}\\
%     % &\approx n(n+d)(1-\alpha^2)^2\trace{\W\W^\top}+(n^2\alpha^4-2n^2\alpha^2(1-\alpha^2))\cdot\trace{\W}^2.
% \end{align*}
% % 
% Combing all together results in that 
% \begin{align*}
%     \Lc(\W)&\approx \left(\alpha^4d+2\alpha^2(1-\alpha^2)+\frac{\alpha^2d}{n}+\frac{\alpha^2\sigma^2}{n}\right)\trace{\W}^2\\
%     &\quad+\left((1-\alpha^2)^2(1+\frac{d}{n})+\frac{\alpha^2d}{n}+\frac{\sigma^2(1-\alpha^2)}{n}\right)\trace{\W\W^\top}-2(\alpha^2d+1-\alpha^2)\trace{\W}+d+\sigma^2
% \end{align*}
% Let $\alpha=\sqrt{{c}/{d}}$. Then setting $\nabla_{\W}\Lc(\W)=0$,
% \begin{align*}
%     \left(c^2+2c(1-\alpha^2)+\frac{cd}{n}+\frac{c\sigma^2}{n}\right)&\frac{\trace{\W}}{d}\Iden+\left((1-\alpha^2)^2(1+\frac{d}{n})+\frac{c}{n}+\frac{\sigma^2(1-\alpha^2)}{n}\right)\W-(\alpha^2d+1-\alpha^2)\Iden=0\\
%     \Longrightarrow\W_{\st}&=\frac{1}{c^2+2c(1-\alpha^2)+\frac{cd}{n}+\frac{c\sigma^2}{n}+(1-\alpha^2)^2(1+\frac{d}{n})+\frac{c}{n}+\frac{\sigma^2(1-\alpha^2)}{n}}\Iden\\
%     &=\frac{c+1-\alpha^2}{(c+(1-\alpha^2))^2+(c+(1-\alpha^2))\frac{d}{n}+\frac{c}{n}+\frac{\sigma^2(c+(1-\alpha^2))}{n}}\Iden\\
%     &=\frac{1}{c+1+\frac{d}{n}+\frac{\sigma^2}{n}}\Iden\\
%     &=\frac{n}{(c+1)n+d+\sigma^2}\Iden.
% \end{align*}
% Plugging this $\W_\st$ results in 
% \[
% \Lc(\W_\st)\approx d+\sigma^2-\frac{(c+1-\alpha^2)nd}{(c+1)n+d+\sigma^2}.
% \]

==> app/reduction.tex <==
\begin{align*}
\Wb^\star_{\pt}&=\left((n+1)\Iden+(\tr{\bSbmu}+d)(\Iden+\bSbmu)^{-1}\right)^{-1},\\
&=(\Iden+\bSbmu)\left((n+1)(\Iden+\bSbmu)+(\tr{\bSbmu}+d)\Iden\right)^{-1}\\
&=\left((n+1+d+\tr{\bSbmu})\Iden+(n+1)\bSbmu\right)^{-1}+\bSbmu\left((n+1+d+\tr{\bSbmu})\Iden+(n+1)\bSbmu\right)^{-1}
\end{align*}
\[
\Wb^\star_{\jt} =
\Big( (n+1+d+\tr{\bSbmu}) \Iden + \bSbmu\Big)^{-1},
\]
\section{Reduction}
\subsection{Observation - joint training}
Consider a preconditioned GD problem with weight $\W$ and prompt $\begin{bmatrix}
    \p_1\\p
\end{bmatrix}$. Let $\y=\x^\top\bt^\st=\x^\top\btb+\x^\top\bmu$ where $\E[\btb]=\zerbb$ and $\bar\p=\p_1p$. Then it returns prediction
\begin{align*}
g_{\gd}(\X,\y;\x)&=\x^\top\W\begin{bmatrix}
    \p_1&\X^\top
\end{bmatrix}\begin{bmatrix}
    p\\\y
\end{bmatrix}\\
&=\x^\top\W\X^\top\y+\x^\top\W\bar\p\\
&=\x^\top\W\X^\top(\X\btb+\X\bmu)+\x^\top\W\bar\p\\
\Longrightarrow g_{\gd}(\X,\y;\x)-\x^\top\bmu&=\x^\top\W\X^\top(\X\btb+\X\bmu)+\x^\top(\W\bar\p-\bmu).
\end{align*}
Suppose $\x\sim \Nc(0,\bSi_x), \btb\sim \Nc(0,\bSi_\beta)$.

\begin{align*}
\Lc(\W,\bar\p)&=\E\left[\left(g_{\gd}(\X,\y;\x)-y\right)^2\right]\\
&=\E\left[\left(\x^\top\W\X^\top(\X\btb+\X\bmu)+\x^\top(\W\bar\p-\bmu)-\x^\top\btb-\xi\right)^2\right]\\
&=\E\left[\left(\x^\top\W\X^\top\X(\btb+\bmu)+\x^\top(\W\bar\p-\bmu)-\x^\top\btb\right)^2\right]+\sigma^2\\
\end{align*}
Then
\begin{align*}
    \frac{\partial\Lc(\W,\bar\p)}{\partial\bar\p}&=2\W^\top\bSi_x\left(\E\left[(\W\X^\top\X-\Iden)(\btb+\bmu)\right]+\W\bar\p\right)\\
    &=2\W^\top\bSi_x\left((n\W\bSi_x-\Iden)\bmu+\W\bar\p\right)\\
    \frac{\partial\Lc(\W,\bar\p)}{\partial\bar\p}=0&\Longrightarrow\bar\pb^\st=\W^{-1}(\Iden-n\W\bSi_x)\bmu=(\W^{-1}-n\bSi_x)\bmu
\end{align*}
Next we get
\begin{align*}
    \Lc(\W,\bar\p^\st)&=\E\left[\left(\x^\top\W\X^\top\X(\btb+\bmu)+\x^\top((\Iden-n\W\bSi_x)-\bmu)-\x^\top\btb\right)^2\right]+\sigma^2\\
    &=\tr{\W^\top\bSi_x\W\E\left[\left(\X^\top\X(\btb+\bmu)-n\bSi_x\bmu\right)\left(\X^\top\X(\btb+\bmu)-n\bSi_x\bmu\right)^\top\right]}\\
    &-2\E\left[\x^\top\W\left(\X^\top\X(\btb+\bmu)-n\bSi_x\bmu\right)\x^\top\btb \right]\\
    &+\tr{\bSi_\beta\bSi_x}+\sigma^2
\end{align*}


\chang{------from here do some derivation----}


{\color{red}{Part A. }}For \(\text{tr} \left( W^\top \Sigma_x W \mathbb{E} \left[ \left( X^\top X(\bar{\beta} + \mu) - n \Sigma_x \mu \right) \left( X^\top X(\bar{\beta} + \mu) - n \Sigma_x \mu \right)^\top \right] \right)\)

\textbf{1. Identifying the Components in the Expression}

Firstly, define:
\[
\vb = \X^\top \X (\btb + \bmu) - n \bSi_x \bmu
\]
Thus, the expression becomes:
\[
\tr{\W^\top \bSi_x \W \E \left[ \vb \vb^\top \right]}
\]

Compute:
\[
\mathbb{E}[v v^\top] = \mathbb{E}\left[ \left( X^\top X (\bar{\beta} + \mu) - n \Sigma_x \mu \right) \left( X^\top X (\bar{\beta} + \mu) - n \Sigma_x \mu \right)^\top \right]
\]

Expansion of \(v v^\top\)

First, expand \(v v^\top\):
\[
v v^\top = \left( X^\top X (\bar{\beta} + \mu) - n \Sigma_x \mu \right) \left( X^\top X (\bar{\beta} + \mu) - n \Sigma_x \mu \right)^\top
\]
Expanding the product:
\[
v v^\top = X^\top X (\bar{\beta} + \mu)(\bar{\beta} + \mu)^\top X^\top X - n X^\top X (\bar{\beta} + \mu) (\Sigma_x \mu)^\top - n \Sigma_x \mu (\bar{\beta} + \mu)^\top X^\top X + n^2 \Sigma_x \mu \mu^\top \Sigma_x
\]

\textbf{2. Computation of \(\mathbb{E}[v v^\top]\)}

Assuming \(X\) and \(\bar{\beta}\) are independent, and \(\bar{\beta} \sim \mathcal{N}(0, \Sigma_\beta)\), we compute the expectation of each term separately.

First Term: \(\mathbb{E}[X^\top X (\bar{\beta} + \mu)(\bar{\beta} + \mu)^\top X^\top X]\)

Let \(S = X^\top X\), which follows a Wishart distribution \(S \sim \mathcal{W}(n, \Sigma_x)\). Then:
\[
\mathbb{E}[S (\bar{\beta} + \mu)(\bar{\beta} + \mu)^\top S] = \mathbb{E}[S A S]
\]
where
\[
A = \mathbb{E}[(\bar{\beta} + \mu)(\bar{\beta} + \mu)^\top] = \Sigma_\beta + \mu \mu^\top
\]
For a Wishart-distributed matrix \(S \sim \mathcal{W}(n, \Sigma_x)\), the following property holds:
\[
\mathbb{E}[S A S] = n \, \text{tr}(A \Sigma_x) \Sigma_x + n(n + 1) \Sigma_x A \Sigma_x
\]
Substituting \(A = \Sigma_\beta + \mu \mu^\top\):
\[
\mathbb{E}[S (\Sigma_\beta + \mu \mu^\top) S] = n \left( \text{tr}(\Sigma_\beta \Sigma_x) + \mu^\top \Sigma_x \mu \right) \Sigma_x + n(n + 1) \Sigma_x (\Sigma_\beta + \mu \mu^\top) \Sigma_x
\]

Second and Third Terms: \(\mathbb{E}[X^\top X (\bar{\beta} + \mu) (\Sigma_x \mu)^\top]\) and \(\mathbb{E}[\Sigma_x \mu (\bar{\beta} + \mu)^\top X^\top X]\)

Since \(X\) and \(\bar{\beta}\) are independent, and \(\mathbb{E}[\bar{\beta}] = 0\):
\[
\mathbb{E}[X^\top X (\bar{\beta} + \mu)] = \mathbb{E}[X^\top X] \mathbb{E}[\bar{\beta} + \mu] = \mathbb{E}[X^\top X] \mu = n \Sigma_x \mu
\]
Thus,
\[
\mathbb{E}[X^\top X (\bar{\beta} + \mu) (\Sigma_x \mu)^\top] = n \Sigma_x \mu (\Sigma_x \mu)^\top = n \Sigma_x \mu \mu^\top \Sigma_x
\]
Similarly,
\[
\mathbb{E}[\Sigma_x \mu (\bar{\beta} + \mu)^\top X^\top X] = n \Sigma_x \mu \mu^\top \Sigma_x
\]

Fourth Term: \(\mathbb{E}[n^2 \Sigma_x \mu \mu^\top \Sigma_x] = n^2 \Sigma_x \mu \mu^\top \Sigma_x\)

This term is deterministic and remains unchanged:
\[
\mathbb{E}[n^2 \Sigma_x \mu \mu^\top \Sigma_x] = n^2 \Sigma_x \mu \mu^\top \Sigma_x
\]

\textbf{3. Combining All Terms}

Combining all the expectations:
\[
\mathbb{E}[v v^\top] = \mathbb{E}[S (\bar{\beta} + \mu)(\bar{\beta} + \mu)^\top S] - n \mathbb{E}[S (\bar{\beta} + \mu) (\Sigma_x \mu)^\top] - n \mathbb{E}[\Sigma_x \mu (\bar{\beta} + \mu)^\top S] + n^2 \Sigma_x \mu \mu^\top \Sigma_x
\]
Substituting the computed expectations:
\[
\mathbb{E}[v v^\top] = n \left( \text{tr}(\Sigma_\beta \Sigma_x) + \mu^\top \Sigma_x \mu \right) \Sigma_x + n(n + 1) \Sigma_x \Sigma_\beta \Sigma_x + n(n + 1) \Sigma_x \mu \mu^\top \Sigma_x - 2n^2 \Sigma_x \mu \mu^\top \Sigma_x + n^2 \Sigma_x \mu \mu^\top \Sigma_x
\]
Simplifying the coefficients:
\[
n(n + 1) - 2n^2 + n^2 = n^2 + n - 2n^2 + n^2 = n
\]
Thus, the final simplified form is:
\[
\mathbb{E}[v v^\top] = n \, \text{tr}(\Sigma_\beta \Sigma_x) \Sigma_x + n (\mu^\top \Sigma_x \mu) \Sigma_x + n(n + 1) \Sigma_x \Sigma_\beta \Sigma_x + n \Sigma_x \mu \mu^\top \Sigma_x
\]

\[
\text{tr} \left( W^\top \Sigma_x W \mathbb{E} \left[ v v^\top \right] \right) = n  \left(\text{tr}(\Sigma_\beta \Sigma_x)  +  \mu^\top \Sigma_x \mu \right) \text{tr}(W^\top \Sigma_x W \Sigma_x) + n(n + 1) \, \text{tr}(W^\top \Sigma_x W \Sigma_x \Sigma_\beta \Sigma_x) + n \, \text{tr}(W^\top \Sigma_x W \Sigma_x \mu \mu^\top \Sigma_x)
\]


{\color{red}{Part B. }}
For
\[
-2 \mathbb{E}\left[ x^\top W v \cdot x^\top \beta \right]
\]

where:

- \( x \sim \mathcal{N}(0, \Sigma_x) \), independent of \( X \) and \( \beta \),

- \( \beta \sim \mathcal{N}(0, \Sigma_\beta) \), independent of \( X \) and \( x \),

- \( v = X^\top X (\beta + \mu) - n \Sigma_x \mu \).


1. Expanding the Third Term

We need to calculate:

\[
-2 \mathbb{E}\left[ x^\top W v \cdot x^\top \beta \right] = -2 \mathbb{E}_{x, X, \beta}\left[ x^\top W v \cdot x^\top \beta \right]
\]

Since \( x \) is independent of \( X \) and \( \beta \), we can decompose the expectation as:

\[
-2 \mathbb{E}_x\left[ x^\top W \cdot \mathbb{E}_{X, \beta}\left[ v \cdot x^\top \beta \right] \right]
\]

However, \( x^\top \beta \) depends on both \( x \) and \( \beta \), though \( x \) and \( \beta \) are independent.

2. Computing \( \mathbb{E}_{X, \beta}\left[ v \cdot x^\top \beta \right] \)

Given that \( x \) is independent of \( X \) and \( \beta \), we can factor out \( x^\top \beta \) from the expectation:

\[
\mathbb{E}_{X, \beta}\left[ v \cdot x^\top \beta \right] = \mathbb{E}_{X, \beta}\left[ v \beta^\top \right] x
\]

Thus, we need to compute:

\[
\mathbb{E}_{X, \beta}\left[ v \beta^\top \right] x
\]

3. Computing \( \mathbb{E}_{X, \beta}\left[ v \beta^\top \right] \)

Now, expand \( v \beta^\top \):

\[
v \beta^\top = \left( X^\top X (\beta + \mu) - n \Sigma_x \mu \right) \beta^\top
\]

This expands as:

\[
v \beta^\top = X^\top X (\beta + \mu) \beta^\top - n \Sigma_x \mu \beta^\top
\]

(a) First Term: \( \mathbb{E}_{X, \beta}\left[ X^\top X (\beta + \mu) \beta^\top \right] \)

Since \( X \) and \( \beta \) are independent, and \( \mathbb{E}[\beta] = 0 \), we compute:

\[
\mathbb{E}_{X, \beta}\left[ X^\top X \beta \beta^\top \right] + \mathbb{E}_{X, \beta}\left[ X^\top X \mu \beta^\top \right]
\]

- For \( \mathbb{E}_{X, \beta}\left[ X^\top X \beta \beta^\top \right] \), because \( \beta \) is independent of \( X \):

  \[
  \mathbb{E}_{X, \beta}\left[ X^\top X \beta \beta^\top \right] = \mathbb{E}_X\left[ X^\top X \right] \mathbb{E}_{\beta}\left[ \beta \beta^\top \right] = n \Sigma_x \Sigma_\beta
  \]

- For \( \mathbb{E}_{X, \beta}\left[ X^\top X \mu \beta^\top \right] \), because \( \mathbb{E}[\beta] = 0 \):

  \[
  \mathbb{E}_{X, \beta}\left[ X^\top X \mu \beta^\top \right] = 0
  \]

Thus, the first term's expectation is:

\[
\mathbb{E}_{X, \beta}\left[ X^\top X (\beta + \mu) \beta^\top \right] = n \Sigma_x \Sigma_\beta
\]

(b) Second Term: \( \mathbb{E}_{X, \beta}\left[ -n \Sigma_x \mu \beta^\top \right] \)

Again, because \( \mathbb{E}[\beta] = 0 \):

\[
\mathbb{E}_{X, \beta}\left[ -n \Sigma_x \mu \beta^\top \right] = 0
\]

Therefore, we have:

\[
\mathbb{E}_{X, \beta}\left[ v \beta^\top \right] = n \Sigma_x \Sigma_\beta
\]

4. Returning to the Term

Now, the term becomes:

\[
-2 \mathbb{E}\left[ x^\top W v \cdot x^\top \beta \right] = -2 \mathbb{E}_x\left[ x^\top W \left( n \Sigma_x \Sigma_\beta \right) x \right] = -2 n \mathbb{E}_x\left[ x^\top W \Sigma_x \Sigma_\beta x \right]
\]

5. Computing \( \mathbb{E}_x\left[ x^\top W \Sigma_x \Sigma_\beta x \right] \)

Using the matrix trace property for quadratic forms:

\[
\mathbb{E}_x\left[ x^\top A x \right] = \operatorname{tr}(A \Sigma_x)
\]

where \( A = W \Sigma_x \Sigma_\beta \). Therefore, we have:

\[
\mathbb{E}_x\left[ x^\top W \Sigma_x \Sigma_\beta x \right] = \operatorname{tr}(W \Sigma_x \Sigma_\beta \Sigma_x)
\]



{\color{red}{Part C. }}

The derivative of the loss function \(\mathcal{L}(W)\) with respect to \(W\) is given by:

\[
\frac{\partial \mathcal{L}(W)}{\partial W} = 2 \Sigma_x W \mathbb{E} \left[ \left( X^\top X (\bar{\beta} + \mu) - n \Sigma_x \mu \right) \left( X^\top X (\bar{\beta} + \mu) - n \Sigma_x \mu \right)^\top \right] 
\]
\[
- 2 \Sigma_x \Sigma_\beta \Sigma_x
\]
\[
=2 \Sigma_x W \mathbb{E}[v v^\top] - 2 \Sigma_x\Sigma_\beta \Sigma_x
\]
\[
=2 \Sigma_x W \left(n \, \text{tr}(\Sigma_\beta \Sigma_x) \Sigma_x + n (\mu^\top \Sigma_x \mu) \Sigma_x + n(n + 1) \Sigma_x \Sigma_\beta \Sigma_x + n \Sigma_x \mu \mu^\top \Sigma_x\right) - 2n \Sigma_x\Sigma_\beta \Sigma_x
\]







\textbf{Final Solution}

The optimal \( W^* \) is given by:
\[
\boxed{
W^* =  \Sigma_\beta \left( \left(\text{tr}(\Sigma_\beta \Sigma_x)  + \mu^\top \Sigma_x \mu\right)I  +  (n + 1) \Sigma_x\Sigma_\beta+  \Sigma_x\mu \mu^\top \right)^{-1} .
}
\]
\chang{----------end of derivation------------}


% where
% \[
% \tr{\W^\top\W\E\left[\left(\X^\top\X(\btb+\bmu)-n\bSi_x\bmu\right)\left(\X^\top\X(\btb+\bmu)-n\bSi_x\bmu\right)^\top\right]}=(d+\tn{\bmu}^2+n+1)n\tr{\W^\top\W}+2n\tr{\W^\top\W\bmu\bmu^\top}-n\tn{\bmu}^2
% \]
% and
% \[
% \tr{\W\E\left[\left(\X^\top\X(\btb+\bmu)-n\bmu\right)\btb^\top\right]}=n\tr{\W}
% \]
which returns
\begin{align*}
    \frac{\partial\Lc(\W,\bar\p^\st)}{\partial\W}&=2(d+\tn{\bmu}^2+n+1)n\W+4n\bmu\bmu^\top\W-2n\Iden\\
    \frac{\partial\Lc(\W,\bar\p^\st)}{\partial\W}&=0\Longrightarrow\W^\st=\left((d+\tn{\bmu}^2+n+1)\Iden+2\bmu\bmu^\top\right)^{-1}.
\end{align*}
Therefore, the optimal loss returns 
\[
\Lc^\st=\Lc(\W^\st,\bar\p^\st)=
\]


\subsection{Observation - Pretraining and finetuning}

\chang{Proof sketch: \\
1. Pretraining stage: Solve the PGD minimization problem on the mixture dataset, and obtian a pretrained $W$. In the first step, no prompts are involved.}

Consider a preconditioned GD problem with weight $\W$ and prompt $\begin{bmatrix}
    \p_1\\p
\end{bmatrix}$. Let $\y=\x^\top\bt^\st=\x^\top\btb+\x^\top\bmu$ where $\E[\btb]=\zerbb$ and $\bar\p=\p_1p$. Then it returns prediction
\begin{align*}
g_{\gd}(\X,\y;\x)&=\x^\top\W\begin{bmatrix}
    \p_1&\X^\top
\end{bmatrix}\begin{bmatrix}
    p\\\y
\end{bmatrix}\\
&=\x^\top\W\X^\top\y+\x^\top\W\bar\p\\
&=\x^\top\W\X^\top(\X\btb+\X\bmu)+\x^\top\W\bar\p\\
\Longrightarrow g_{\gd}(\X,\y;\x)-\x^\top\bmu&=\x^\top\W\X^\top(\X\btb+\X\bmu)+\x^\top(\W\bar\p-\bmu).
\end{align*}
Suppose $\x\sim \Nc(0,\bSi_x), \btb\sim \Nc(0,\bSi_\beta)$.


{\color{red}
\begin{align*}
\Lc(\W,\bar\p)|_{\bar\p=0}&=\E\left[\left(g_{\gd}(\X,\y;\x)-y\right)^2\right]\\
&=\sum_{k=1}^K\pi_k\E\left[\left(\x^\top\W\X^\top(\X\btb_k+\X\bmu_k)+\x^\top(-\bmu_k)-\x^\top\btb_k-\xi\right)^2\right]
\end{align*}}

We aim to compute and simplify the expression:

\[
\sum_{k=1}^{K} \pi_k \mathbb{E} \left[ \left( x^\top \left( W X^\top X - I \right) \left( \bar{\beta}_k + \mu_k \right) - \xi \right)^2 \right],
\]
where:
\begin{itemize}
    \item \( x \sim \mathcal{N}(0, \Sigma_x) \in \mathbb{R}^d \),
    \item \( X = [x_1, \dots, x_n]^\top \in \mathbb{R}^{n \times d} \) with each \( x_i \sim \mathcal{N}(0, \Sigma_x) \),
    \item \( \bar{\beta}_k \sim \mathcal{N}(0, \Sigma_{\beta_k}) \in \mathbb{R}^d \),
    \item \( \xi \sim \mathcal{N}(0, \sigma^2) \).
\end{itemize}

\textbf{Step 1: Expand the Square}
The expression inside the expectation is:
\[
\left( x^\top \left( W X^\top X - I \right) \left( \bar{\beta}_k + \mu_k \right) - \xi \right)^2.
\]
Expanding the square:
\[
\begin{aligned}
\left( x^\top \left( W X^\top X - I \right) \left( \bar{\beta}_k + \mu_k \right) - \xi \right)^2 &= \left( x^\top \left( W X^\top X - I \right) \left( \bar{\beta}_k + \mu_k \right) \right)^2 \\
&\quad - 2 \xi x^\top \left( W X^\top X - I \right) \left( \bar{\beta}_k + \mu_k \right) + \xi^2.
\end{aligned}
\]

\textbf{Step 2: Compute Expectation over \(\xi\)}
Since \( \xi \) is independent of \( x \), \( X \), and \( \bar{\beta}_k \), and \( \mathbb{E}[\xi] = 0 \):
\[
\mathbb{E}[-2 \xi x^\top (\dots)] = 0,
\]
\[
\mathbb{E}[\xi^2] = \sigma^2.
\]
Thus, the expectation simplifies to:
\[
\mathbb{E} \left[ \left( x^\top \left( W X^\top X - I \right) \left( \bar{\beta}_k + \mu_k \right) \right)^2 \right] + \sigma^2.
\]

\textbf{Step 3: First Term Expansion}
We need to compute:
\[
\mathbb{E} \left[ \left( x^\top \left( W X^\top X - I \right) \left( \bar{\beta}_k + \mu_k \right) \right)^2 \right].
\]
This expands as:
\[
\mathbb{E} \left[ \operatorname{tr} \left( \left( W X^\top X - I \right)^\top \Sigma_x \left( W X^\top X - I \right) \left( \Sigma_{\beta_k} + \mu_k \mu_k^\top \right) \right) \right].
\]

\textbf{Step 4: Expectation over \( X \)}
We need to compute:
\[
\mathbb{E} \left[ \left( W X^\top X - I \right)^\top \Sigma_x \left( W X^\top X - I \right) \right].
\]
Expanding \( \left( W X^\top X - I \right) \):
\[
\left( W X^\top X - I \right) = W X^\top X - I,
\]
and its transpose:
\[
\left( W X^\top X - I \right)^\top = X^\top X W^\top - I.
\]
Now, expand the product:
\[
\left( X^\top X W^\top - I \right) \Sigma_x \left( W X^\top X - I \right) = X^\top X W^\top \Sigma_x W X^\top X - X^\top X W^\top \Sigma_x - \Sigma_x W X^\top X + \Sigma_x.
\]

\textbf{Step 5: Expectation of Each Term}
We compute the expectations:
\[
\mathbb{E}[ X^\top X W^\top \Sigma_x W X^\top X ],
\]
\[
\mathbb{E}[ X^\top X W^\top \Sigma_x ],
\]
\[
\mathbb{E}[ \Sigma_x W X^\top X ].
\]
Using properties of Wishart-distributed matrices:
\[
\mathbb{E}[ X^\top X ] = n \Sigma_x,
\]
\[
\mathbb{E}[ X^\top X A X^\top X ] = n \operatorname{tr}( A \Sigma_x ) \Sigma_x + n(n+1) \Sigma_x A \Sigma_x.
\]
Let \( A = W^\top \Sigma_x W \). Then:
\[
\mathbb{E}[ X^\top X W^\top \Sigma_x W X^\top X ] = n \operatorname{tr}( W^\top \Sigma_x W \Sigma_x ) \Sigma_x + n(n+1) \Sigma_x W^\top \Sigma_x W \Sigma_x.
\]
We also have:
\[
\mathbb{E}[ X^\top X W^\top \Sigma_x ] = n \Sigma_x W^\top \Sigma_x,
\]
\[
\mathbb{E}[ \Sigma_x W X^\top X ] = n \Sigma_x W \Sigma_x.
\]

\textbf{Step 6: Combine All Terms}
Thus, the final expectation is:
\[
\mathbb{E} \left[ \left( W X^\top X - I \right)^\top \Sigma_x \left( W X^\top X - I \right) \right] = n \operatorname{tr}( W^\top \Sigma_x W \Sigma_x ) \Sigma_x + n(n+1) \Sigma_x W^\top \Sigma_x W \Sigma_x - n \Sigma_x W^\top \Sigma_x - n \Sigma_x W \Sigma_x + \Sigma_x.
\]

\textbf{Step 7: Final Simplified Expression}
The final expression is:
\[
n(n+1) \operatorname{tr} \left( \Sigma_x W^\top \Sigma_x W \Sigma_x M \right) + n \operatorname{tr} \left( W^\top \Sigma_x W \Sigma_x \right ) \operatorname{tr} \left( \Sigma_x M \right ) - 2 n \operatorname{tr} \left( \Sigma_x W \Sigma_x M \right ) + \operatorname{tr} \left( \Sigma_x M \right ) + \sigma^2,
\]
where \( M = \sum_{k=1}^{K} \pi_k \left( \Sigma_{\beta_k} + \mu_k \mu_k^\top \right) \).


We are given the function:
\[
\mathcal{L}(W) = n(n+1) \operatorname{tr} \left( \Sigma_x W^\top \Sigma_x W \Sigma_x M \right) + n \operatorname{tr} \left( W^\top \Sigma_x W \Sigma_x \right ) \operatorname{tr} \left( \Sigma_x M \right ) - 2 n \operatorname{tr} \left( \Sigma_x W \Sigma_x M \right ) + \operatorname{tr} \left( \Sigma_x M \right ) + \sigma^2,
\]
where:
\[
M = \sum_{k=1}^{K} \pi_k \left( \Sigma_{\beta_k} + \mu_k \mu_k^\top \right).
\]

Our goal is to compute the derivative of \( \mathcal{L}(W) \) with respect to \( W \), find the minimizer \( W^* \), and compute the minimal value of \( \mathcal{L}(W) \).

\textbf{Derivation}

\textbf{Step 1: Compute the Gradient \( \frac{\partial \mathcal{L}(W)}{\partial W} \)}

We will compute the gradient by differentiating each term of \( \mathcal{L}(W) \) with respect to \( W \).

\textbf{Term 1: \( L_1 = n(n+1) \operatorname{tr} \left( \Sigma_x W^\top \Sigma_x W \Sigma_x M \right) \)}

First, note that \( \Sigma_x \) and \( M \) are symmetric matrices. We can use the matrix derivative formula:
\[
\frac{\partial}{\partial W} \operatorname{tr}(W^\top A W B) = 2 A W B,
\]
when \( A \) and \( B \) are constants.

Thus, the derivative of \( L_1 \) is:
\[
\frac{\partial L_1}{\partial W} = 2 n(n+1) \Sigma_x W \Sigma_x \Sigma_x M.
\]

\textbf{Term 2: \( L_2 = n \operatorname{tr} \left( W^\top \Sigma_x W \Sigma_x \right ) \operatorname{tr} \left( \Sigma_x M \right ) \)}

Let \( t = \operatorname{tr} \left( W^\top \Sigma_x W \Sigma_x \right ) \). Then:
\[
\frac{\partial t}{\partial W} = 2 \Sigma_x W \Sigma_x.
\]
Therefore, the derivative of \( L_2 \) is:
\[
\frac{\partial L_2}{\partial W} = n \left( 2 \Sigma_x W \Sigma_x \right ) \operatorname{tr} \left( \Sigma_x M \right ) = 2 n \Sigma_x W \Sigma_x \operatorname{tr} \left( \Sigma_x M \right ).
\]

\textbf{Term 3: \( L_3 = -2 n \operatorname{tr} \left( \Sigma_x W \Sigma_x M \right ) \)}

The derivative is:
\[
\frac{\partial L_3}{\partial W} = -2 n \Sigma_x M \Sigma_x.
\]

\textbf{Term 4 and 5}

Terms \( L_4 = \operatorname{tr} \left( \Sigma_x M \right ) \) and \( L_5 = \sigma^2 \) are constants with respect to \( W \), so their derivatives are zero:
\[
\frac{\partial L_4}{\partial W} = 0, \quad \frac{\partial L_5}{\partial W} = 0.
\]

\textbf{Total Gradient}

Combining the derivatives:
\[
\frac{\partial \mathcal{L}(W)}{\partial W} = \frac{\partial L_1}{\partial W} + \frac{\partial L_2}{\partial W} + \frac{\partial L_3}{\partial W} = 2 n(n+1) \Sigma_x W \Sigma_x \Sigma_x M + 2 n \Sigma_x W \Sigma_x \operatorname{tr} \left( \Sigma_x M \right ) - 2 n \Sigma_x M \Sigma_x.
\]

\textbf{Step 2: Set the Gradient to Zero and Solve for \( W^* \)}

We set the gradient to zero to find the minimizer \( W^* \):
\[
0 = 2 n(n+1) \Sigma_x W^* \Sigma_x \Sigma_x M + 2 n \Sigma_x W^* \Sigma_x \operatorname{tr} \left( \Sigma_x M \right ) - 2 n \Sigma_x M \Sigma_x.
\]


Thus, the minimizer \( W^* \) is:
\[
W^* = M \left( (n+1) \Sigma_x M + \operatorname{tr} \left( \Sigma_x M \right ) I \right )^{-1}.
\]


\textbf{Minimal Value}

Given the complexity and without further simplifications, we can denote the minimal value as:
\[
\mathcal{L}_{\text{min}} = \mathcal{L}(W^*) = \operatorname{tr} \left( \Sigma_x M \right ) + \sigma^2 - n \operatorname{tr} \left( \Sigma_x M W^* \Sigma_x \right ).
\]

Since \( W^* \) satisfies:
\[
W^* = M \left( (n+1) \Sigma_x M + \operatorname{tr} \left( \Sigma_x M \right ) I \right )^{-1},
\]
we can, in principle, compute \( \operatorname{tr} \left( \Sigma_x M W^* \Sigma_x \right ) \) and thus find \( \mathcal{L}_{\text{min}} \).


\textbf{Conclusion}

The minimizer \( W^* \) of \( \mathcal{L}(W) \) is given by: (define \(\boxed{M = \sum_{k=1}^{K} \pi_k \left( \Sigma_{\beta_k} + \mu_k \mu_k^\top \right)}.\))
\[
\boxed{ W^* = M \left( (n+1) \Sigma_x M + \operatorname{tr} \left( \Sigma_x M \right ) I \right )^{-1} }.
\]

The minimal value of \( \mathcal{L}(W) \) is:
\[
\boxed{ \mathcal{L}(W^*) = \operatorname{tr} \left( \Sigma_x M \right ) + \sigma^2 - n \operatorname{tr} \left( \Sigma_x M W^* \Sigma_x \right ) }.
\]
\chang{Proof sketch: \\
2. Fine-tuning stage: Take the optimal \(\W^*\) into the original expression, and solve for the optimal \(\bar\p\)}
\[
\mathcal{L}(W, \bar{p}) = \mathbb{E} \left[ \left( g_{\text{GD}}(X, y; x) - y \right)^2 \right] \\
= \mathbb{E} \left[ \left( x^\top W X^\top (X \beta + X \mu) + x^\top (W \bar{p} - \mu) - x^\top \beta - \xi \right)^2 \right] 
\]
\[
= \mathbb{E} \left[ \left( x^\top W X^\top X (\beta + \mu) + x^\top (W \bar{p} - \mu) - x^\top \beta \right)^2 \right] + \sigma^2
\]
Define the following:
\begin{itemize}
    \item \( M = \sum_{k=1}^{K} \pi_k \left( \Sigma_{\beta_k} + \mu_k \mu_k^\top \right) \).
    \item \( W^* = M \left( (n+1) \Sigma_x M + \operatorname{tr} \left( \Sigma_x M \right ) I \right )^{-1} \).
    \item \( \beta_i \) is the \( i \)-th random variable with mean zero and covariance \( \Sigma_{\beta_i} \).
    \item \( \mu_i \) is the \( i \)-th mean vector.
    \item \( \bar{p} \) is a deterministic vector.
    \item \( x \sim \mathcal{N}(0, \Sigma_x) \).
\end{itemize}




\textbf{Step 1: Simplify the Expression}

Combine terms:
\[
\begin{aligned}
S &= x^\top \left( W^* X^\top X (\beta_i + \mu_i) + W^* \bar{p} - (\beta_i + \mu_i) \right ) \\
&= x^\top \left( \left( W^* X^\top X - I \right ) (\beta_i + \mu_i) + W^* \bar{p} \right ).
\end{aligned}
\]

\textbf{Step 2: Compute \( \mathbb{E}[S^2] \)}

Expand the square:
\[
\begin{aligned}
\mathbb{E}[S^2] &= \mathbb{E} \left[ \left( x^\top \left( W^* X^\top X - I \right ) (\beta_i + \mu_i) \right )^2 \right ] + 2 \mathbb{E} \left[ x^\top \left( W^* X^\top X - I \right ) (\beta_i + \mu_i) x^\top W^* \bar{p} \right ] \\
&\quad + \mathbb{E} \left[ \left( x^\top W^* \bar{p} \right )^2 \right ].
\end{aligned}
\]

\textbf{Step 3: Compute Each Term}

\textbf{Term 1}
\[
T_1 = \operatorname{tr} \left( \Sigma_x \, \mathbb{E} \left[ \left( W^* X^\top X - I \right ) (\Sigma_{\beta_i} + \mu_i \mu_i^\top) \left( W^* X^\top X - I \right )^\top \right ] \right ).
\]

\textbf{Term 2}
\[
T_2 = 2 \operatorname{tr} \left( \Sigma_x W^{* \top} \bar{p} \mu_i^\top \left( n \Sigma_x W^{* \top} - I \right ) \right ).
\]

\textbf{Term 3}
\[
T_3 = \operatorname{tr} \left( \Sigma_x W^* \bar{p} \bar{p}^\top W^{* \top} \right ).
\]

\textbf{Step 4: Combine Terms}

\[
\mathcal{L}(W^*, \bar{p}) = T_1 + T_2 + T_3 + \sigma^2.
\]

\textbf{Step 5: Final Expression}

\[
\begin{aligned}
\mathcal{L}(W^*, \bar{p}) &= n(n+1) \operatorname{tr} \left( \Sigma_x W^{* \top} \Sigma_x W^* \Sigma_x M_i \right ) + n \operatorname{tr} \left( W^{* \top} \Sigma_x W^* \Sigma_x \right ) \operatorname{tr} \left( \Sigma_x M_i \right ) \\
&\quad - 2 n \operatorname{tr} \left( \Sigma_x W^* \Sigma_x M_i \right ) + \operatorname{tr} \left( \Sigma_x M_i \right ) + \sigma^2 \\
&\quad + 2 n \operatorname{tr} \left( \Sigma_x W^{* \top} \bar{p} \mu_i^\top \Sigma_x W^{* \top} \right ) - 2 \operatorname{tr} \left( \Sigma_x W^{* \top} \bar{p} \mu_i^\top \right ) + \operatorname{tr} \left( \Sigma_x W^* \bar{p} \bar{p}^\top W^{* \top} \right ).
\end{aligned}
\]

Here, we have defined:
\begin{itemize}
    \item \( M_i = \Sigma_{\beta_i} + \mu_i \mu_i^\top \).
\end{itemize}

This is the simplified expression for \( \mathcal{L}(W^*, \bar{p}) \) after substituting \( W^* \).

\textbf{Step 1: Simplify \( \mathcal{L}(W^*, \bar{p}) \)}

\[
\mathcal{L}(W^*, \bar{p}) = C + T_2 + T_3 + \sigma^2,
\]
where:

\begin{center}{\boxed{
\begin{aligned}
C &= n(n+1) \operatorname{tr} \left( \Sigma_x W^{* \top} \Sigma_x W^* \Sigma_x M_i \right ) + n \operatorname{tr} \left( W^{* \top} \Sigma_x W^* \Sigma_x \right ) \operatorname{tr} \left( \Sigma_x M_i \right ) \\
&\quad - 2 n \operatorname{tr} \left( \Sigma_x W^* \Sigma_x M_i \right ) + \operatorname{tr} \left( \Sigma_x M_i \right ),
\end{aligned}
}}
\end{center}

and \( M_i = \Sigma_{\beta_i} + \mu_i \mu_i^\top \).

\textbf{Step 2: Compute Gradient with Respect to \( \bar{p} \)}

\[
\frac{\partial \mathcal{L}(W^*, \bar{p}) }{ \partial \bar{p} } = 2 \left( n W^{* \top} \Sigma_x - I \right ) \Sigma_x W^* \mu_i + 2 W^{* \top} \Sigma_x W^* \bar{p}.
\]

\textbf{Step 3: Find Optimal \( \bar{p}^* \)}

Set the gradient to zero:
\[
0 = \left( n W^{* \top} \Sigma_x - I \right ) \Sigma_x W^* \mu_i + W^{* \top} \Sigma_x W^* \bar{p}^*.
\]
Solve for \( \bar{p}^* \):
\[
\boxed{ \bar{p}^* = - \left( W^{* \top} \Sigma_x W^* \right )^{-1} \left( n W^{* \top} \Sigma_x - I \right ) \Sigma_x W^* \mu_i }
\]

\textbf{Step 4: Compute \( \mathcal{L}(W^*, \bar{p}^*) \)}

Substitute \( \bar{p}^* \) back into \( \mathcal{L}(W^*, \bar{p}) \):
\[
\mathcal{L}(W^*, \bar{p}^*) = C - \mu_i^\top D D^\top \mu_i + \sigma^2,
\]
where:
\[
D = \left( n \Sigma_x W^{* \top} - I \right ) \Sigma_x W^* \left( W^{* \top} \Sigma_x W^* \right )^{-1}.
\]
\[
W^* = M \left( (n+1) \Sigma_x M + \operatorname{tr} \left( \Sigma_x M \right ) I \right )^{-1} ,M = \sum_{k=1}^{K} \pi_k \left( \Sigma_{\beta_k} + \mu_k \mu_k^\top \right)
\]
Simplify:
\[
\boxed{ \mathcal{L}(W^*, \bar{p}^*) = C - \mu_i^\top D D^\top \mu_i + \sigma^2 }
\]




\newpage


\section{Prompt}
\begin{proof}
Consider task, feature and noise following distributions  $\bt\sim\Dc_\bt$, $\x\sim\Dc_{\x}$ and $\xi\sim\Dc_{\xi}$. The label is generated via $y=\x^\top\bt+\xi$. Suppose that 
\[
\E[\bt]=\bmu,\quad\E[\x]=0,\quad\text{and}\quad\E[\xi]=0.
\]
Then we can rewrite 
\[
y=\x^\top\bt+\xi=\x^\top\bt_0+\xi+\x^\top\bmu=y_0+\x^\top\bmu
\]
where we have $\E[\bt_0]=0$. Then consider ICL with single prompt and let prompt vector be
\[
\p=\begin{bmatrix}
    \p_1\\p
\end{bmatrix},
\]
where $\p_1\in\R^d$ and $p\in\R$. Then the input sequence and query token can be written by
\[
\Z=\begin{bmatrix}
    \p_1&\x_1&\dots&\x_n\\
    p&y_1&\dots&y_n
\end{bmatrix}^\top=\begin{bmatrix}
    \p_1&\X^\top\\
    p&\y^\top
\end{bmatrix}^\top\quad\text{and}\quad\z=\begin{bmatrix}
    \x\\0
\end{bmatrix}.
\]
Additionally, denote
\[
\WQ\WK^\top=\begin{bmatrix}
    \Wb&\w_1\\
    \w_2^\top&w
\end{bmatrix}\qquad\text{and}\qquad\WV\vb=\begin{bmatrix}
    \vb_1\\
    v
\end{bmatrix}.
\]
where $\Wb\in\R^{d\times d}$, $\w_1,\w_2,\vb_1\in\R^d$, and $w,v\in\R$. 
Then we have
\begin{align}
g_{\att}(\Z)&=(\z^\top\WQ\WK^\top\Z^\top)\Z\WV\vb\nn\\
&=[\x^\top~0]\begin{bmatrix}
    \Wb&\w_1\\
    \w_2^\top&w
\end{bmatrix}\begin{bmatrix}
    \p_1&\X^\top\\
    p&\y^\top
\end{bmatrix}\begin{bmatrix}
    \p_1^\top&p\\
    \X&\y
\end{bmatrix}\begin{bmatrix}
    \vb_1\\
    v
\end{bmatrix}\nn\\
&=\x^\top(\Wb\X^\top+\w_1\y^\top)(\X\vb_1+\y v)+\x^\top(\Wb\p_1+\w_1p)(\p_1^\top\vb_1+p v)\nn\\
&=\x^\top(v\Wb\X^\top\y+\w_1\y^\top\X\vb_1)+\x^\top\left(\Wb\X^\top\X\vb_1+v\tn{\y}^2\w_1\right)+\x^\top\tilde \p\nn\\
&=\x^\top(v\Wb+\w_1\vb_1^\top)\X^\top\y+\x^\top\left(\Wb\X^\top\X\vb_1+v\tn{\y}^2\w_1+\tilde\p\right)\nn\\
&=\x^\top\Wt\X^\top(\y_0+\X\bmu)+\x^\top\left(\Wb\X^\top\X\vb_1+v(\tn{\y_0}^2+\tn{\X\bmu}^2+2\y_0^\top\X\bmu)\w_1+\tilde\p\right)\nn\\
% &=\x^\top(\Wt+2\w_1\bmu^\top)\X^\top\y_0+\x^\top\left(\Wb\X^\top\X\vb_1+\Wt\X^\top\X\bmu+v(\tn{\y_0}^2+\tn{\X\bmu}^2)\w_1\right)\nn\\
&=\underset{\tilde g_{\att}(\Z)}{\underbrace{\x^\top(\Wt+2v\w_1\bmu^\top)\X^\top\y_0}}+\underset{\eps}{\underbrace{\x^\top\left(\Wb\X^\top\X\vb_1+(\Wt+v\w_1\bmu^\top)\X^\top\X\bmu+v\tn{\y_0}^2\w_1+\tilde\p\right)}},\label{gd=att eq 1}
\end{align}
where $\Wt:=v\Wb+\w_1\vb_1^\top$ and $\tilde \p=(\Wb\p_1+\w_1p)(\p_1^\top\vb_1+p v)$. Then 
\begin{align*}
    \E[(g_{\att}(\Z)-y)^2]&=\E[(\tilde g_{\att}(\Z)+\eps-y_0-\x^\top\bmu)^2]\\
    &=\E[(\tilde g_{\att}(\Z)-y_0)^2]+\E[(\eps-\x^\top\bmu)^2]+2\E[(\tilde g_{\att}(\Z)-y_0)(\eps-\x^\top\bmu)].
\end{align*}
Suppose odd order of cross-moment of $\X,\x$ and $\bt$ are zeros. Additionally, suppose noise is independent from $\X,\x$ and $\bt$ with zero mean. Then we obtain
\begin{align*}
    \E[(\tilde g_{\att}(\Z)-y_0)(\eps-\x^\top\bmu)]=0.
\end{align*}
Therefore,
\[
\E[(g_{\att}(\Z)-y)^2]=\E[(\tilde g_{\att}(\Z)-y_0)^2]+\E[(\eps-\x^\top\bmu)^2]\geq\E[(\tilde g_{\att}(\Z)-y_0)^2].
\]
Consider any full rank matrix $\W\in\R^{d\times d}$ and let
\[
\WK=\WV=\Iden,\quad\WQ=\begin{bmatrix}
    \W&\zerbb\\
    \zerbb^\top&0
\end{bmatrix},\quad\vb=\begin{bmatrix}
    -\bmu\\1
\end{bmatrix},\quad\text{and}\quad\p=\begin{bmatrix}
    \W^{-1}\bmu\\\bmu^\top(\Wb^{-\top})\bmu+1
\end{bmatrix}.
\]
Then 
\begin{align*}
    g_{\att}(\Z)=\x^\top\W\X^\top\y_0+\x^\top\bmu
\end{align*}
and 
\[
\E[(g_{\att}(\Z)-y)^2]=\E[(\tilde g_{\att}(\Z)-y_0)^2].
\]
Therefore, the problem can be reduced to an unbiased preconditioned gradient descent problem. 
\end{proof}

Consider the following linear data setting. Suppose all the features (for all the tasks) follow the same distribution $\x_i\sim\Nc(0,\bSi_{\x})$ and noise follows $\xi_i\sim\Nc(0,\sigma^2)$ for $i\in[n+1]$. Consider the MTL setting where we have $K$ tasks each with distribution $\bt_k\sim\Nc(\bmu_k,\bSi_k)$ and probability $\pi_k$ for all $k\in[K]$, and $\sum_{k=1}^K\pi_k=1$.  Then using the reduction result, we can conclude:

\noindent\textbf{MTL risk. } Consider it as a single-task learning problem. Then the task is distributed as 
\[
\bar\bt\sim\Nc(\bar\bmu,\bar\bSi_{\bt}):=\Nc\left(\sum_{k=1}^K\pi_k\bmu_k,\sum_{k=1}^K\pi_k^2\bSi_k\right).
\]
Directly applying the previous work [], we have that
\[
\Lc_\st=M-n\tr{((n+1)\Iden+M\bSi^{-1})^{-1}}
\]
where
\[
\bSi=\bSi_{\x}^{1/2}\bar\bSi_{\bt}\bSi_{\x}^{1/2}\quad \text{and}\quad M=\tr{\bSi}+\sigma^2.
\]

\noindent\textbf{Single-task risk. } 

\subsection{Prompt tuning}
\begin{proof}
    Similarly, we get
    \begin{align*}
        g_{\att}(\Z_k)=\underset{\tilde g_{\att}(\Z_k)}{\underbrace{\x^\top(\Wt+2v\w_1\bmu_k^\top)\X^\top\y_0}}+\underset{\eps}{\underbrace{\x^\top\left(\Wb\X^\top\X\vb_1+(\Wt+v\w_1\bmu_k^\top)\X^\top\X\bmu_k+v\tn{\y_0}^2\w_1+\tilde\p_k\right)}},
    \end{align*}
    where $\Wt:=v\Wb+\w_1\vb_1^\top$ and $\tilde \p_k=(\Wb\p_{1k}+\w_1p_k)(\p_{1k}^\top\vb_1+p_k v)$. 
\end{proof}






% \subsection{Without restriction}
% Denote the input sequence by
% \[
% \mathbf{Z} := \begin{pmatrix}
% \mathbf{X}^\top & \mathbf{x} \\
% \mathbf{y}^\top & 0
% \end{pmatrix} \in \mathbb{R}^{(d+1) \times (n+1)}.
% \]

% Denote the query, key, and value parameters by
% \[
% \WQ, \WK, \WV \in \mathbb{R}^{(d+1) \times (d+1)}.
% \]

% Then the single-layer attention with residue connection outputs
% \[
% (\WV\mathbf{Z}) (\WQ\mathbf{Z})^\top (\WK\mathbf{Z}) \in \mathbb{R}^{(d+1) \times (n+1)}.
% \]

% The prediction is the bottom right entry of the above matrix, that is ($\mathbf{e}_i$ is a one-hot vector with $1$ on the $i-$th entry)
% \[
% \hat{y} = \left[ (\WV\mathbf{Z})(\WQ\mathbf{Z})^\top (\WK\mathbf{Z}) \right]_{d+1, n+1}
% \]
% \[
% \color{red}{= \mathbf{e}_{d+1}^\top \left( \WV\mathbf{ZZ}^\top \WQ \WK\mathbf{Z} \right) \mathbf{e}_{n+1}}
% \]
% \[
% =  \mathbf{e}_{d+1}^\top \WV\mathbf{ZZ}^\top \WQ \WK\mathbf{Z} \mathbf{e}_{n+1}
% \]
% \[
% =   \left( \mathbf{e}_{d+1}^\top \WV \right) 
% \begin{pmatrix} 
% \mathbf{X}^\top \mathbf{X} + \mathbf{x} \mathbf{x}^\top & \mathbf{X}^\top \mathbf{y} \\ 
% \mathbf{y}^\top \mathbf{X} & \mathbf{y}^\top \mathbf{y} 
% \end{pmatrix} 
% \WQ^\top \WK 
% \begin{pmatrix} 
% \mathbf{x} \\ 
% 0 
% \end{pmatrix},
% \]

% Our key assumption is that the bottom left \( 1 \times d \) block in \( \WV \) is fixed to be zero and the bottom left \( 1 \times d \) block in \( \WQ^\top \WK \) is fixed to be zero, that is, we assume that
% \[
% \WV = \begin{pmatrix}
% * & * \\
% 0 & v
% \end{pmatrix}, \quad \WQ^\top \WK = \begin{pmatrix}
% \mathbf{W} & * \\
% 0 & *
% \end{pmatrix},
% \]

% where \( v \in \mathbb{R} \) and \( \mathbf{W} \in \mathbb{R}^{d \times d} \) are relevant free parameters. Then we have
% \[
% \hat{y} = \begin{pmatrix} 0, v \end{pmatrix} \left( \begin{pmatrix} \mathbf{X}^\top \mathbf{X} + \mathbf{x} \mathbf{x}^\top & \mathbf{X}^\top \mathbf{y} \\ \mathbf{y}^\top \mathbf{X} & \mathbf{y}^\top \mathbf{y} \end{pmatrix} \begin{pmatrix} \mathbf{W} \mathbf{x} \\ 0 \end{pmatrix} \right)
% \]
% \[
% = v \mathbf{y}^\top \mathbf{X} \mathbf{W} \mathbf{x}
% \]
% \[
% = \left\langle \left( v \mathbf{W}^\top \right) \mathbf{X}^\top \mathbf{y}, \mathbf{x} \right\rangle,
% \]

% which recovers one-step GD when we replace \( v \mathbf{W}^\top \) by \( \mathbf{W} \).

% In our current setup (with restriction), the output is obtained by using a \color{red}{trainable head $\mathbf{v}$}, i.e.
% \[
% \hat{y}=\left( \mathbf{z}^\top\WQ \WK^\top \mathbf{Z}^\top \right) \mathbf{Z} \WV \mathbf{v},
% \]



==> app/simplified.tex <==
\section{Equivalence among Gradient Descent, Attention, and State-Space Models}
In this section, we present the proofs related to Section~\ref{sec:setup}. 
Recap that given data
\begin{align*}
&\X=[\x_1~\cdots~\x_n]^\top\in\R^{n\times d},\\
&\bxi=[\xi_1~\cdots~\xi_n]^\top\in\R^n,\\
&\y=[y_1~\cdots~y_n]^\top=\X\bt+\bxi\in\R^n,\\
&
\Z_0=[\z_1~\dots~\z_n~\zerbb_{d+1}]^\top=\begin{bmatrix}
    \x_1&\dots&\x_n&\zerbb_d\\
    y_1&\dots&y_n&0
\end{bmatrix}^\top \in \R^{(n+1) \times (d+1)},
\end{align*}
and corresponding prediction functions
\begin{subequations}\label{pred all app}
\begin{align}
&g_{\gd}(\Z)=\x^\top\W\X^\top\y,\label{pred gd app}\\
&g_{\wpgd}(\Z)=\x^\top\W\X^\top(\bom\odot\y),\label{pred wpgd app}\\
&g_{\att}(\Z)=(\z^\top\WQ\WK^\top\Zm^\top)\Zm\WV\vb,\label{pred att app}\\
&g_{\ssm}(\Z)=\left((\z^\top\WQ)^\top\odot((\Zm\WK\odot\Zm\WV) \ast\fb)_{n+1}\right)\vb,\label{pred ssm app}
\end{align}
\end{subequations}
we have objectives 
\begin{subequations}\label{obj all app}
\begin{align}
\min_{\W}\Lc_{\gd}(\Wc)\quad&\text{where}\quad\Lc_{\gd}(\Wc)=
\E\left[(y-g_{\gd}(\Z))^2\right]\label{obj gd app},\\
\min_{\W,\bom}\Lc_{\wpgd}(\Wc)\quad&\text{where}\quad\Lc_{\wpgd}(\Wc)=
\E\left[(y-g_{\wpgd}(\Z))^2\right]\label{obj wpgd app},\\
\min_{\WK,\WQ,\WV,\vb}\Lc_{\att}(\Wc)\quad&\text{where}\quad\Lc_{\att}(\Wc)=
\E\left[(y-g_{\att}(\Z))^2\right]\label{obj att app},\\
\min_{\WK,\WQ,\WV,\vb,\fb}\Lc_{\ssm}(\Wc)\quad&\text{where}\quad\Lc_{\ssm}(\Wc)=
\E\left[(y-g_{\ssm}(\Z))^2\right].\label{obj ssm app}
\end{align}
\end{subequations}
Here, the expectation is over the randomness in $(\x_i,\xi_i)_{i=1}^{n}$ and $\bt$, and the search space for $\W$ is $\R^{d\times d}$, for $\bom$ is $\R^{n}$, for $\WK,\WQ,\WV$ is $\R^{(d+1)\times(d+1)}$, for $\vb$ is $\R^{d+1}$, and for $\fb$ is $\R^{n+1}$. 


\subsection{Proof of Proposition~\ref{lemma:eqv}}\label{app:proof eqv}
Consider the problem setting as discussed in Section~\ref{sec:setup}, 
% and let $g:=g_{\gd}$ and $\Lc:=\Lc_{\gd}$. 
Proposition~\ref{lemma:eqv} can be proven by the following two lemmas.
\begin{lemma}\label{lemma gd=att}
Suppose Assumptions~\ref{assum:odd x beta} and \ref{assume:noise} hold. Then, given the objectives \eqref{obj gd app} and \eqref{obj att app}, we have
\[
\min_{\WQ,\WK,\WV,\vb}\Lc_{\att}(\Wc)=\min_{\W}\Lc_{\gd}(\Wc).
\]

\end{lemma}

\begin{proof}
Recap the linear attention estimator from \eqref{pred att app} and denote 
\[
\WQ\WK^\top=\begin{bmatrix}
    \Wb&\w_1\\
    \w_2^\top&w
\end{bmatrix}\qquad\text{and}\qquad\WV\vb=\begin{bmatrix}
    \vb_1\\
    v
\end{bmatrix},
\]
where $\Wb\in\R^{d\times d}$, $\w_1,\w_2,\vb_1\in\R^d$, and $w,v\in\R$. 
Then we have 
\begin{align}
g_{\att}(\Z)&=(\z^\top\WQ\WK^\top\Z_0^\top)\Z_0\WV\vb\nn\\
&=[\x^\top~0]\begin{bmatrix}
    \Wb&\w_1\\
    \w_2^\top&w
\end{bmatrix}\begin{bmatrix}
    \X^\top&\zerbb_d\\
    \y^\top&0
\end{bmatrix}\begin{bmatrix}
    \X&\y\\
    \zerbb_d^\top&0
\end{bmatrix}\begin{bmatrix}
    \vb_1\\
    v
\end{bmatrix}\nn\\
&=(\x^\top\Wb\X^\top+\x^\top\w_1\y^\top)(\X\vb_1+\y v)\nn\\
&=\x^\top(v\Wb)\X^\top\y+\x^\top\w_1\y^\top\X\vb_1+\x^\top\left(\Wb\X^\top\X\vb_1+v\tn{\y}^2\w_1\right)\nn\\
&=\x^\top(v\Wb+\w_1\vb_1^\top)\X^\top\y+\x^\top\left(\Wb\X^\top\X\vb_1+v\tn{\y}^2\w_1\right)\nn\\
&=\underset{\tilde{g}_{\att}(\Z)}{\underbrace{\x^\top\Wt\X^\top\y}}+\underset{\eps}{\underbrace{\x^\top\left(\Wb\X^\top\X\vb_1+v\tn{\y}^2\w_1\right)}},\label{gd=att eq 1}
\end{align}
where $\Wt:=v\Wb+\w_1\vb_1^\top$. 

We first show that for any given parameters $\WK,\WQ,\WV,\vb$,  
\begin{align}
\E\left[(g_{\att}(\Z)-y)^2\right]\geq\E\left[(\tilde g_{\att}(\Z)-y)^2\right].\label{lower bound}
\end{align}
To this goal, we have
\begin{align}
    \E\left[(g_{\att}(\Z)-y)^2\right]-\E\left[(\tilde g_{\att}(\Z)-y)^2\right]
    &=\E\left[(\tilde g_{\att}(\Z)+\eps-y)^2\right]-\E\left[(\tilde g_{\att}(\Z)-y)^2\right]\nn\\
    &=\E[\eps^2]+2\E[(\tilde g_{\att}(\Z)-y)\eps]\label{risk gap}
\end{align}
where we have decomposition
\begin{align*}
    (\tilde g_{\att}(\Z)-y)\eps&=(\x^\top\Wt\X^\top\y-y)\x^\top\left(\Wb\X^\top\X\vb_1+v\tn{\y}^2\w_1\right)\\
    &=\y^\top\X\Wt^\top\x\x^\top\left(\Wb\X^\top\X\vb_1+v\tn{\y}^2\w_1\right)-y\x^\top\left(\Wb\X^\top\X\vb_1+v\tn{\y}^2\w_1\right)\\
    &=\underset{(a)}{\underbrace{\y^\top\X\Wt^\top\x\x^\top\Wb\X^\top\X\vb_1}}+\underset{(b)}{\underbrace{v\tn{\y}^2\y^\top\X\Wt^\top\x\x^\top\w_1}}-\underset{(c)}{\underbrace{y\x^\top\Wb\X^\top\X\vb_1}}-\underset{(d)}{\underbrace{ vy\tn{\y}^2\x^\top\w_1}}.
\end{align*}
In the following, we consider the expectations of $(a),(b),(c),(d)$ sequentially, which return zeros under Assumptions~\ref{assum:odd x beta} and \ref{assume:noise}. Note that since Assumption~\ref{assum:odd x beta} holds, expectation of any odd \emph{order} of monomial of the entries of $\X,\x,\bt$ returns zero, i.e., 
order of $\x^\top\bt\x$ is 3 and therefore  $\E[\x^\top\bt\x]=\zerbb_d$. 
\begin{align*}
    (a):\quad&\E\left[\y^\top\X\Wt^\top\x\x^\top\Wb\X^\top\X\vb_1\right]\hspace*{300pt}\\
    &=\E\left[(\X\bt+\bxi)^\top\X\Wt^\top\x\x^\top\Wb\X^\top\X\vb_1\right]\\
    &=\E\left[\bt^\top\X^\top\X\Wt^\top\x\x^\top\Wb\X^\top\X\vb_1\right]+\E\left[\bxi^\top\X\Wt^\top\x\x^\top\Wb\X^\top\X\vb_1\right]\\
    &=0.
\end{align*}
\begin{align*}
    (b):\quad&\E\left[v\tn{\y}^2\y^\top\X\Wt^\top\x\x^\top\w_1\right]\hspace*{300pt}\\
    &=\E\left[v(\X\bt+\bxi)^\top(\X\bt+\bxi)(\X\bt+\bxi)^\top\X\Wt^\top\x\x^\top\w_1\right]\\
    &=\E\left[v\tn{\bxi}^2\bxi^\top\X\Wt^\top\x\x^\top\w_1\right]\\
    &=0.
\end{align*}
\begin{align*}
    (c):\quad&\E\left[y\x^\top\Wb\X^\top\X\vb_1\right]\hspace*{300pt}\\
    &=\E\left[(\x^\top\bt+\xi)\x^\top\Wb\X^\top\X\vb_1\right]\\
    &=\E\left[\bt^\top\x\x^\top\Wb\X^\top\X\vb_1\right]+\E\left[\xi\x^\top\Wb\X^\top\X\vb_1\right]\\
    &=0.
\end{align*}
\begin{align*}
    (d):\quad&\E\left[vy\tn{\y}^2\x^\top\w_1\right]\hspace*{300pt}\\
    &=v\E\left[(\bt^\top\x+\xi)(\X\bt+\bxi)^\top(\X\bt+\bxi)\x^\top\w_1\right]\\
    &=v\E\left[\xi\tn{\bxi}^2\x^\top\w_1\right]\\
    &=0.
\end{align*}
Combining the results with \eqref{risk gap} returns that 
\begin{align}
\E\left[(g_{\att}(\Z)-y)^2\right]-\E\left[(\tilde g_{\att}(\Z)-y)^2\right]=\E[\eps^2]\geq0\label{gd=att eq 2}
\end{align}
which completes the proof of \eqref{lower bound}. Therefore, we obtain
\[
\min_{\WQ,\WK,\WV,\vb}\E\left[(g_{\att}(\Z)-y)^2\right]\geq\min_{\tilde\W}\E\left[(\tilde g_{\att}(\Z)-y)^2\right]=\min_{\W}\E\left[(g_{\gd}(\Z)-y)^2\right].
\]
We conclude the proof of this lemma by showing that for any $\W\in\R^{d\times d}$ in $g_{\gd}$, there exist $\WK,\WQ,\WV,\vb$ such that $g_\att(\Z)=g_{\gd}(\Z)$. Let 
\[
\WK=\WV=\Iden_{d+1},\qquad\WQ=\begin{bmatrix}
    \W&\zerbb_d\\
    \zerbb_d^\top&0
\end{bmatrix},\quad\text{and}\quad\vb=\begin{bmatrix}
    \zerbb_d\\1
\end{bmatrix}.
\]
Then we obtain
\begin{align}
g_{\att}(\Z)=\x^\top\W\X^\top\y=g_{\gd}(\Z), \label{gd=att eq 3}
\end{align}
which completes the proof.
\end{proof}

\begin{lemma}Suppose Assumptions~\ref{assum:odd x beta} and \ref{assume:noise} hold. Then, given the objectives in \eqref{obj all app}, we have
\begin{align}
\min_{\WQ,\WK,\WV,\vb,\fb}\Lc_{\ssm}(\Wc)=\min_{\W,\bom}\Lc_{\wpgd}(\Wc).\label{lemma ssm=wpgd eq1}
\end{align}
{Additionally, if the examples $(\x_i,y_i)_{i=1}^n$ follow the same distribution and are conditionally independent given $\x$ and $\bt$, then SSM/H3 can achieve the optimal loss using the all-ones filter and
% $\Lc^\st_{\gd}=\Lc_{\ssm}^\st$.
\begin{align}
\min_{\W,\bom}\Lc_{\wpgd}(\Wc)=\min_{\W}\Lc_{\gd}(\Wc).\label{lemma ssm=wpgd eq2}
\end{align}}
\end{lemma}
\begin{proof}
Recap the SSM estimator from \eqref{pred ssm app} and let 
\begin{align*}
    &\WQ=\begin{bmatrix}
        \w_{q1}&
        \w_{q2}&
        \cdots&
        \w_{q,{d+1}}
    \end{bmatrix},\\
    &\WK=\begin{bmatrix}
        \w_{k1}&
        \w_{k2}&
        \cdots&
        \w_{k,{d+1}}
    \end{bmatrix},\\
    &\WV=\begin{bmatrix}
        \w_{v1}&
        \w_{v2}&
        \cdots&
        \w_{v,{d+1}}
    \end{bmatrix},
\end{align*}
where $\w_{qj},\w_{kj},\w_{vj}\in\R^{d+1}$ for $j\leq d+1$, and let
\[
\vb=\begin{bmatrix}
    v_1\\
    v_2\\
    \cdots\\
    v_{d+1}
\end{bmatrix},\quad\text{and}\quad\fb=\begin{bmatrix}
    f_{0}\\
    f_{1}\\
    \cdots\\
    f_{n}
\end{bmatrix}.
\]
Then we have
\begin{align*}
    g_\ssm(\Z)&=\left((\z^\top\WQ)^\top\odot((\Zm\WK\odot\Zm\WV) \ast\fb)_{n+1}\right)\vb\\
    &=\sum_{i=1}^nf_{n+1-i}\cdot\vb^\top\left(\begin{bmatrix}
        \w_{q1}^\top\z\\
        \cdots\\
        \w_{q,{d+1}}^\top\z
    \end{bmatrix}\odot\begin{bmatrix}
        \w_{k1}^\top\z_i\w_{v1}^\top\z_i\\
        \cdots\\
        \w_{k,{d+1}}^\top\z_i\w_{v,{d+1}}^\top\z_i
    \end{bmatrix}\right)\\
    &=\sum_{i=1}^nf_{n+1-i}\cdot\vb^\top\begin{bmatrix}
        \w_{q1}^\top\z\w_{k1}^\top\z_i\w_{v1}^\top\z_i\\
        \cdots\\
        \w_{q,{d+1}}^\top\z\w_{k,{d+1}}^\top\z_i\w_{v,{d+1}}^\top\z_i
    \end{bmatrix}.
\end{align*}
Next for all $j\leq d+1$, let 
\[
\w_{qj}=\begin{bmatrix}
    \wb_{qj}\\
    w_{qj}
\end{bmatrix},\quad\w_{kj}=\begin{bmatrix}
    \wb_{kj}\\
    w_{kj}
\end{bmatrix},\quad\w_{vj}=\begin{bmatrix}
    \wb_{vj}\\
    w_{vj}
\end{bmatrix}
\]
where $\wb_{qj},\wb_{kj},\wb_{vj}\in\R^d$ and $w_{qj},w_{kj},w_{vj}\in\R$. 
Then we have
\begin{align*}
    \w_{qj}^\top\z\w_{kj}^\top\z_i\w_{vj}^\top\z_i&=\left(\wb_{qj}^\top\x\right)\left(\wb_{kj}^\top\x_i+w_{kj}y_i\right)\left(\wb_{vj}^\top\x_i+w_{vj}y_i\right)\\
    &=\x^\top\wb_{qj}\left(w_{vj}\wb_{kj}^\top+w_{kj}\wb_{vj}^\top\right)\x_iy_i+\left(\wb_{qj}^\top\x\right)\left(\wb_{kj}^\top\x_i\right)\left(\wb_{vj}^\top\x_i\right)+\left(w_{kj}w_{vj}\wb_{qj}^\top\x y_i^2\right)\\
    &=\x^\top\W'_j\x_i y_i+\delta_j(\x,\x_i,\x_i)+{\w_j'}^\top \x y_i^2
\end{align*}
where 
\begin{align*}
&\W'_j:=\wb_{qj}\left(w_{vj}\wb_{kj}^\top+w_{kj}\wb_{vj}^\top\right)\in\R^{d\times d},\\
&\w_j':=w_{kj}w_{vj}\wb_{qj}\in\R^d,\\
&\delta_j(\x,\x_i,\x_i):=\left(\wb_{qj}^\top\x\right)\left(\wb_{kj}^\top\x_i\right)\left(\wb_{vj}^\top\x_i\right)\in\R.
\end{align*}
Then
\begin{align*}
    g_{\ssm}(\Z)&=\sum_{i=1}^nf_{n+1-i}\cdot\sum_{j=1}^{d+1}v_j\left(\x^\top\W'_j\x_i y_i+\delta_j(\x,\x_i,\x_i)+{\w_j'}^\top \x y_i^2\right)\\
    &=\x^\top\left(\sum_{j=1}^{d+1}v_j\W'_j\right)\X(\y\odot\tilde\fb)+\sum_{i=1}^nf_{n+1-i}\cdot\sum_{j=1}^{d+1}v_j\cdot\delta_j(\x,\x_i,\x_i)+\left(\sum_{j=1}^{d+1}v_j{\w_j'}^\top\right)\x \y^\top(\y\odot\tilde\fb)\\
    &=\underset{\tilde g_{\ssm}(\Z)}{\underbrace{\x^\top\tilde\W\X\tilde\y}}+\underset{\eps_1}{\underbrace{\tilde\delta(\x,\X,\X)}}+\underset{\eps_2}{\underbrace{\tilde\w^\top\x \y^\top\tilde\y}}.
\end{align*}
where
\begin{align*}
&\tilde\fb:=[f_n~\cdots~f_1]^\top\in\R^n,\\
&\tilde\y:=\y\odot\tilde\fb\in\R^n,\\
&\tilde\W:=\sum_{j=1}^{d+1}v_j\W'_j\in\R^{d\times d},\\
&\tilde\w:=\sum_{j=1}^{d+1}v_j{\w_j'}\in\R^d,\\
&\tilde\delta(\x,\X,\X):=\sum_{i=1}^nf_{n+1-i}\cdot\sum_{j=1}^{d+1}v_j\cdot\delta_j(\x,\x_i,\x_i)\in\R.
\end{align*}
Next we will show that for any $\WK,\WQ,\WV,\vb$, 
\[
\E\left[(g_{\ssm}(\Z)-y)^2\right]\geq\E\left[(\tilde g_{\ssm}(\Z)-y)^2\right].
\]
To start with, we obtain
\begin{align}
    \E\left[(g_\ssm(\Z)-y)^2\right]&=\E\left[(\tilde g_{\ssm}(\Z)+\eps_1+\eps_2-y)^2\right]\nn\\
    &=\E\left[(\tilde g_{\ssm}(\Z)-y)^2\right]+\E\left[(\eps_1+\eps_2)^2\right]+2\E\left[(\tilde g_{\ssm}(\Z)-y)(\eps_1+\eps_2)\right]\label{risk gap ssm}
\end{align}
where there is decomposition
\begin{align*}
    (\tilde g_{\ssm}(\Z)-y)(\eps_1+\eps_2)=\underset{(a)}{\underbrace{\tilde\delta(\x,\X,\X)\cdot\x^\top\tilde\W\X\tilde\y}}-\underset{(b)}{\underbrace{\tilde\delta(\x,\X,\X)y}}+\underset{(c)}{\underbrace{\tilde\w^\top\x \y^\top\tilde\y\cdot\x^\top\tilde\W\X\tilde\y}}-\underset{(d)}{\underbrace{y\cdot\tilde\w^\top\x \y^\top\tilde\y}}.
\end{align*}
In the following, similar to the proof of Lemma~\ref{lemma gd=att}, we consider the expectations of $(a),(b),(c),(d)$ sequentially, which return zeros under Assumptions~\ref{assum:odd x beta} and \ref{assume:noise}. Note that $\delta_j(\x,\x_i,\x_i)$'s and $\tilde\delta(\x,\X,\X)$ are summation of monomials of entries of $(\x,\X,\bt)$ with order 3, and entries of $\y$ and $y$ are summation of monomials of entries of $(\x,\X,\bt)$ with even orders: e.g., $y=\x^\top\bt+\xi$ where $\xi$ is of oder 0 and  $\x^\top\bt$ is of order 2.


\begin{align*}
    (a):\quad&\E\left[\tilde\delta(\x,\X,\X)\cdot\x^\top\tilde\W\X\tilde\y\right]\hspace*{300pt}\\
    &=\E\left[\tilde\delta(\x,\X,\X)\cdot\x^\top\tilde\W\X(\X\bt\odot\tilde\fb)\right]+\E\left[\tilde\delta(\x,\X,\X)\cdot\x^\top\tilde\W\X(\bxi\odot\tilde\fb)\right]\\
    &=\E\left[\tilde\delta(\x,\X,\X)\cdot\x^\top\tilde\W\X\right]\E\left[\bxi\odot\tilde\fb\right]\\
    &=0.
\end{align*}
\begin{align*}
    (b):\quad&\E\left[\tilde\delta(\x,\X,\X)y\right]\hspace*{400pt}\\
    &=\E\left[\tilde\delta(\x,\X,\X)(\x^\top\bt+\xi)\right]\\
    &=\E\left[\tilde\delta(\x,\X,\X)\x^\top\bt\right]+\E\left[\tilde\delta(\x,\X,\X)\xi\right]\\
    &=0.
\end{align*}
\begin{align*}
    (c):\quad&\E\left[\tilde\w^\top\x \y^\top\tilde\y\cdot\x^\top\tilde\W\X\tilde\y\right]\hspace*{400pt}\\
    &=\E\left[\tilde\w^\top\x (\X\bt+\bxi)^\top(\X\bt\odot\tilde\fb+\bxi\odot\tilde\fb)\cdot\x^\top\tilde\W\X(\X\bt\odot\tilde\fb+\bxi\odot\tilde\fb)\right]\\
    &=0.
\end{align*}
\begin{align*}
    (d):\quad&\E\left[y\cdot\tilde\w^\top\x \y^\top\tilde\y\right]\hspace*{400pt}\\
    &=\E\left[(\x^\top\bt+\xi)\cdot\tilde\w^\top\x (\X\bt+\bxi)^\top(\X\bt\odot\tilde\fb+\bxi\odot\tilde\fb)\right]\\
    &=0.
\end{align*}
Combining the results with \eqref{risk gap ssm} results that
\begin{align*}
    \E\left[(g_\ssm(\Z)-y)^2\right]-\E\left[(\tilde g_\ssm(\Z)-y)^2\right]=\E\left[(\eps_1+\eps_2)^2\right]\geq0.
\end{align*}
Therefore we obtain,
\[
\min_{\WQ,\WK,\WV,\vb,\fb}\E\left[(g_{\ssm}(\Z)-y)^2\right]\geq\min_{\tilde\W,\tilde\fb}\E\left[(\tilde g_{\ssm}(\Z)-y)^2\right]=\min_{\W,\bom}\E\left[( g_{\wpgd}(\Z)-y)^2\right].
\]
Next we show that for any choices of $\W$ and $\bom$ in $g_{\wpgd}$, there are $\W_{q,k,v},\vb,\fb$ such that $g_{\ssm}\equiv g_{\wpgd}$. To this end, given $\bom=[\omega_1~\dots~\omega_n]^\top$, let 
\[
\WQ=\Iden_{d+1},\quad\WK=\begin{bmatrix}
    \W^\top&\zerbb_d\\
    \zerbb_d^\top&0
\end{bmatrix},\quad\WV=\begin{bmatrix}
    \zerbb_{d\times d}&\zerbb_d\\
    \onebb_d^\top&0
\end{bmatrix},\quad\vb=\begin{bmatrix}
    \onebb_d\\
    0
\end{bmatrix}\quad\text{and}\quad\fb=\begin{bmatrix}
    0\\
    \omega_n\\
    \cdots\\
    \omega_1
\end{bmatrix}.
\]
Then we get
\begin{align*}
((\Z_0\WK\odot\Z_0\WV)\ast\fb)_{n+1}&=\left(\left(\begin{bmatrix}
    \X\W^\top&\zerbb_n\\
    \zerbb_d&0
\end{bmatrix}\odot\begin{bmatrix}
    \y\onebb_d^\top&\zerbb_n\\
    \zerbb_d&0
\end{bmatrix}\right)\ast\fb\right)_{n+1}\\
&=\begin{bmatrix}\sum_{i=1}^n\omega_i\cdot y_i\W\x_i\\
0\end{bmatrix}\\
&=\begin{bmatrix}\W\X^\top(\y\odot\bom)\\0\end{bmatrix},
\end{align*}
and therefore
\[
g_\ssm(\Z)=\x^\top\W\X^\top(\y\odot\bom)=g_{\wpgd}(\Z),
\]
which completes the proof of \eqref{lemma ssm=wpgd eq1}.

Next, to show \eqref{lemma ssm=wpgd eq2}, for any $\W\in\R^{d\times d}$, let $\Lc(\bom)=\E\left[\left(\x^\top\W\X^\top(\y\odot\bom)-y\right)^2\right]$.
Then we have
\begin{align*}
\frac{\partial\Lc(\bom)}{\partial \omega_i}&=\E\left[2\left(\x^\top\W \sum_{j=1}^n\omega_jy_j\x_j-y\right)\left(\x^\top\W y_i\x_i\right)\right]\\
&=2\sum_{j=1}^n\omega_j\E\left[(\x^\top\W y_j\x_j)(\x^\top\W y_i\x_i)\right]-2\E\left[y\x^\top\W y_i\x_i\right].
\end{align*}
Here since $(\x_i,y_i)_{i=1}^n$ follow the same distribution and are conditionally independent given $\x$ and $\bt$, for any $i\neq j\neq j'$, $\E\left[(\x^\top\W y_i\x_i)^2\right]=\E\left[(\x^\top\W y_{j}\x_{j})^2\right]$ and $\E\left[(\x^\top\W y_j\x_j)(\x^\top\W y_i\x_i)\right]=\E\left[(\x^\top\W y_{j'}\x_{j'})(\x^\top\W y_i\x_i)\right]$. Then let
\[
\E\left[(\x^\top\W y_j\x_j)(\x^\top\W y_i\x_i)\right]=\begin{cases}
    c_1,& i\neq j\\
    c_2,& i=j
\end{cases}\quad\text{and}\quad\E\left[y\x^\top\W y_i\x_i\right]=c_3,
\]
where $(c_1,c_2,c_3):=(c_1(\W),c_2(\W),c_3(\W))$. 
We get
\[
\frac{\partial\Lc(\bom)}{\partial \omega_i}
=2c_1\bom^\top\onebb_n+2(c_2-c_1)\omega_i-2c_3.
\]
If $c_2-c_1=0$, then $\frac{\partial\Lc(\bom)}{\partial \omega_i}\equiv2c_1\bom^\top\onebb_n-2c_3$ for all $i\leq n$ and any $\bom\in\R^n$ achieves the same performance.

If $c_2-c_1\neq0$, setting $\frac{\partial\Lc(\bom)}{\partial \omega_i}=0$ returns 
\[
\omega_i=\frac{c_3-c_1\sum_{j=1}^n\omega_j}{c_2-c_1}:=C\quad\text{for all }i\leq n.
\]
Therefore the optimal loss is achieved via setting $\bom=C\onebb_n$. Without loss of generality, we can update $\W\to C\W$. Then $\bom=\onebb_n$, and we obtain 
\[
\min_{\W,\bom}\E\left[\left(\x^\top\W\X^\top(\y\odot\bom)-y\right)^2\right]=\min_{\W}\E\left[(\x^\top\W\X^\top\y-y)^2\right]
\]
which completes the proof of \eqref{lemma ssm=wpgd eq2}.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma cvx 1}}


\begin{proof}
    Recap the loss $\Lc_{\gd}(\Wc)$ in \eqref{obj gd app} and prediction $g_{\gd}(\Z)$ in \eqref{pred gd app}, we have
    \begin{align}
        \Lc_{\gd}(\Wc)&=\E[(y-g_{\gd}(\Z))^2]\nn\\
        &=\E\left[\left(\x^\top\bt+\xi-\x^\top\W\X^\top(\X\bt+\bxi)\right)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2+2(\x^\top\bt-\x^\top\W\X^\top\X\bt)(\xi-\x^\top\W\X^\top\bxi)+(\xi-\x^\top\W\X^\top\bxi)^2\right]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2+(\xi-\x^\top\W\X^\top\bxi)^2\right]+2\E[(\x^\top\bt-\x^\top\W\X^\top\X\bt)(\xi-\x^\top\W\X^\top\bxi)]\nn\\
    &=\E\left[(\x^\top\bt-\x^\top\W\X^\top\X\bt)^2+(\xi-\x^\top\W\X^\top\bxi)^2\right]\label{cvx eq 1}\\
    &=\underset{f_1(\W)}{\underbrace{\E\left[(\x^\top\W\X^\top\X\bt)^2+(\x^\top\W\X^\top\bxi)^2\right]}}\underset{f_2(\W)}{\underbrace{-2\E[\bt^\top\x\x^\top\W\X^\top\X\bt+\xi\x^\top\W\X^\top\bxi]}}+\underset{\text{constant}}{\underbrace{\E[(\x^\top\bt)^2+\xi^2]}}\nn
    \end{align}
    where \eqref{cvx eq 1} follows Assumption \ref{assume:noise}. Since $f_2(\W)$ is convex, $\Lc_{\gd}(\Wc)$ is strongly-convex if and only if $f_1(\W)$ is strongly-convex, which completes the proof of strong convexity.

    Next, \eqref{gd=att eq 2} and \eqref{gd=att eq 3} in the proof of Lemma~\ref{lemma gd=att} demonstrate that the optimal loss is achievable and is achieved at $\eps=0$. Subsequently, \eqref{gd=att eq 1} indicates that $g^\st_{\att}$ has the same form as $g^\st_{\gd}$. Under the strong convexity assumption, $g^\st_{\gd}$ is unique, which leads to the conclusion that $g^\st_{\gd} = g^\st_{\att}$.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma cvx 2}}

\begin{proof} 
According to Lemma~\ref{lemma cvx 1}, $\Lc_{\gd}(\Wc)$ is strongly-convex as long as either $\E[(\x^\top\W\X^\top\X\bt)^2]$ or $\E[(\x^\top\W\X^\top\bxi)^2]$ is strongly-convex. Therefore, in this lemma, the two claims correspond to the strong convexity of $\E[(\x^\top\W\X^\top\bxi)^2]$ and $\E[(\x^\top\W\X^\top\X\bt)^2]$ terms, respectively. 

Suppose the decomposition claim holds. Without losing generality, we may assume $(\x_1,\bt_1,\X_1)$ are zero-mean because we can allocate the mean component to $(\x_2,\bt_2,\X_2)$ without changing the covariance. 

\noindent $\bullet$ \textbf{Claim 1:} Let $\bSb_{\x}=\E[\x_1\x_1^\top]$, $\bSb_{\bt}=\E[\bt_1\bt_1^\top]$, and $\bSb_{\X}=\E[\X_1^\top\X_1]$. If the first claim holds, using independence, observe that we can write
\begin{align}
\E[(\x^\top\W\X^\top\bxi)^2]&=\E[(\x_1^\top\W\X_1^\top\bxi)^2]+\E[(\x_1^\top\W\X_2^\top\bxi)^2]+\E[(\x_2^\top\W\X_1^\top\bxi)^2]+\E[(\x_2^\top\W\X_2^\top\bxi)^2],\nn
\end{align}
where the last three terms of the right hand side are convex and the first term obeys
\begin{align*}
\E[(\x_1^\top\W\X_1^\top\bxi)^2]&=\sigma^2\E[\x_1^\top\W\X_1^\top\X_1\W^\top \x_1]\\
&=\sigma^2\tr{\E[\x_1\x_1^\top\W\X_1^\top\X_1\W^\top]}\\
&=\sigma^2\tr{\bSb_{\x}\W\bSb_{\X}\W^\top}\\
&=\sigma^2\tf{\sqrt{\bSb_{\x}}\W\sqrt{\bSb_{\X}}}^2.
\end{align*}
Since noise level $\sigma>0$, using the full-rankness of covariance matrices $\bSb_{\x}$ and $\bSb_{\X}$, we conclude with strong convexity of $\E[(\x^\top\W\X^\top\bxi)^2]$. 

\noindent $\bullet$ \textbf{Claim 2:} Now recall that $\bSb_{\X}=\E[\X_1^\top\X_1]$ and set $\A=\X_1^\top\X_1-\bSb_{\X}$ and $\B=\X_2^\top\X_2+\bSb_{\X}$. Observe that $\E[\A]=0$. If the second claim holds, $\E[\X^\top\X]=\E[\A+\B]$. Note that $(\A,\bt_1,\x_1)$ are independent of each other and $(\B,\bt_2,\x_2)$. Using independence and $\E[\A]=0$, similarly write
\begin{align*}
\E[(\x^\top\W\X^\top\X\bt)^2]&=\E[(\x^\top\W\A\bt)^2]+\E[(\x^\top\W\B\bt)^2].
\end{align*}
Now using $\E[\bt_1]=\E[\x_1]=0$ and their independence from rest, these terms obeys 
\begin{align*}
&\E[(\x^\top\W\A\bt)^2]=\E[(\x_1^\top\W\A\bt_1)^2]+\E[(\x_1^\top\W\A\bt_2)^2]+\E[(\x_2^\top\W\A\bt_1)^2]+\E[(\x_2^\top\W\A\bt_2)^2]\\
&\E[(\x^\top\W\B\bt)^2]=\E[(\x_1^\top\W\B\bt_1)^2]+\E[(\x_1^\top\W\B\bt_2)^2]+\E[(\x_2^\top\W\B\bt_1)^2]+\E[(\x_2^\top\W\B\bt_2)^2].
\end{align*}
In both equations, the last three terms of the right hand side are convex. To proceed, we focus on the first terms. Using independence and setting $\bSi_{\X
}=\E[\X^\top\X]\succeq \bSb_{\X}\succ 0$, we note that
\begin{align*}
\E[(\x_1^\top\W\A\bt_1)^2]+\E[(\x_1^\top\W\B\bt_1)^2]=\E[(\x_1^\top\W\X^\top\X\bt_1)^2]
\end{align*}
where $\x_1,\bt_1,\X$ are independent and full-rank covariance. To proceed, note that 
\begin{align*}
\E[(\x_1^\top\W\X^\top\X\bt_1)^2]=\E[(\x_1^\top\W\bSi_{\X}\bt_1)^2]+\E[(\x_1^\top\W(\X^\top\X-\bSi_{\X})\bt_1)^2].
\end{align*}
Observing the convexity of the right hand side and focusing on the first term, we get
\begin{align*}
\E[(\x_1^\top\W\bSi_{\X}\bt_1)^2]=\tr{\bSb_{\x}\W\bSi_{\X}\bSb_{\bt}\bSi_{\X}\W^\top}=\tf{\sqrt{\bSb_x}\W\bSi_{\X}\sqrt{\bSb_\bt}}^2.
\end{align*}
Using the fact that covariance matrices, $\bSb_{\x},\bSi_{\X},\bSb_{\bt}$,  are full rank concludes the strong convexity proof of $\E[(\x^\top\W\X^\top\X\bt)^2]$.
\end{proof}


==> app/thm_restate.tex <==
\begin{theorem} [Pretraining followed by fine-tuning] For the model defined in (\ref{eqn:LinearAttn}), we consider independent linear data as defined in Section~\ref{sec:assumptions} and loss function as defined in (\ref{eqn:loss}), and suppose covariance matrices $\bSi_{\x},\{\bSi_{\bt_k}\}_{k=1}^K$ are full rank. Let 
\begin{align}
\W^\star_{\textnormal{pretr}} &:= \arg\min_{\W}\mathcal{L}(\W, \bar\p=0), \notag\\
\bar\p^\star_k &:= \arg\min_{\bar\p_k}\mathcal{L}(\W^\star_{\textnormal{pretr}}, \bar\p_k), k\in[K],\notag\\
\mathcal{L}^\star_{\textnormal{pretr}} &:= \mathcal{L}(\W^\star_{\textnormal{pretr}}, \bar\p=0), \notag\\
\mathcal{L}^\star_\textnormal{fine-tune} &:= \mathcal{L}(\W^\star_{\textnormal{pretr}}, \bar\p^\star). \notag
\end{align}
Additionally, let $\M:=\sum_{k=1}^K\pi_k(\bSi_{\beta_k}+\bmu_k\bmu_k^\top)$, and $ \bSibt:=\bar\M:=\sum_{k=1}^K\pi_k\bSi_{\beta_k}$, $\bSimu=\sum_{k=1}^K\pi_k\bmu_k\bmu_k^\top$ then $\W^\star_{\textnormal{pretr}}$,$\bar\p^\star_k$, $\mathcal{L}^\star_{\textnormal{pretr}}$ and $\mathcal{L}^\star_\textnormal{fine-tune}$ satisfy
\[
\boxed{
\begin{aligned}
\W^\star_{\pt}&=(\bSibt+\bSimu)\left(\tr{\bSi_{\x}(\bSibt+\bSimu)}\Iden+(n+1)\bSi_{\x}(\bSibt+\bSimu)\right)^{-1}\notag\\
\bar{\p}_k^\star &= \left((\W^\star_{\pt})^{-1} - n\bSi_{\x}\right)\bmu_k, k\in[K],\\
\mathcal{L}^\star_{\pt} &= \tr{(\bSibt+\bSimu)\bSi_{\x}}
-2n\tr{\W^\star_{\pt}\bSi_{\x}(\bSibt+\bSimu)\bSi_{\x}}+n\tr{\W^\star_{\pt}\Big(\tr{(\bSibt+\bSimu)\bSi_{\x}}\bSi_{\x}+(n+1)\bSi_{\x}(\bSibt+\bSimu)\bSi_{\x}\Big)\W^{\star\top}_{\pt}\bSi_{\x}}.\\
&=\tr{(\bSibt+\bSimu)\bSi_{\x}}
-n\tr{\W^\star_{\pt}\bSi_{\x}(\bSibt+\bSimu)\bSi_{\x}}
\\\\
\mathcal{L}^\star_\ft(\W) = &\tr{\bSibt\bSi_{\x}}-2n\tr{\W\bSi_{\x}\bSibt\bSi_{\x}}+n\tr{\W\Big(\tr{\bSibt\bSi_{\x}}\bSi_{\x}+\bSi_{\x}\Big((n+1)\bSibt+ \bSimu \Big)\bSi_{\x}\Big)\W^{\top}\bSi_{\x}}
\end{aligned}
}
\]
\[
\bSbbt=\bSi_{\x}\bSibt,\quad\bSbmu=\bSi_{\x}\bSimu,\quad\Wb=\bSi_{\x}\W~\text{for any }\W\in\R^{d\times d}
\]
\[
\boxed{
\begin{aligned}
\Wb^\star_{\pt}&=(\bSbbt+\bSbmu)\left(\tr{\bSbbt+\bSbmu}\Iden+(n+1)(\bSbbt+\bSbmu)\right)^{-1}\notag\\
\bar{\p}_k^\star &= \left((\W^\star_{\pt})^{-1} - n\bSi_{\x}\right)\bmu_k, k\in[K],\\
\mathcal{L}^\star_{\pt} &= \tr{\bSbbt+\bSbmu}
-2n\tr{\Wb^\star_{\pt}(\bSbbt+\bSbmu)}+n\tr{\W^\star_{\pt}\Big(\tr{\bSbbt+\bSbmu}+(n+1)(\bSbbt+\bSbmu)\Big)\Wb^{\star\top}_{\pt}}.\\
&=\tr{\bSbbt+\bSbmu}
-n\tr{\Wb^\star_{\pt}(\bSbbt+\bSbmu)}
\\\\
\mathcal{L}^\star_\ft(\W) &= \tr{\bSbbt}-2n\tr{\Wb\bSbbt}+n\tr{\Wb\Big(\tr{\bSbbt+\bSbmu}+\Big((n+1)\bSbbt+ \bSbmu \Big)\Big)\Wb^{\top}}\\
\\
\mathcal{L}^\star_\ft(\W_\pt^\st) &= \mathcal{L}^\star_{\pt}-\tr{\bSbmu}
+2n\tr{\Wb^\star_{\pt}\bSbmu}-n^2\tr{\W^\star_{\pt}\bSbmu\Wb^{\star\top}_{\pt}}\\
&=\mathcal{L}^\star_{\pt}-\tr{\bSbmu(\Wb^{\star}_{\pt}-\Iden)^\top(\Wb^{\star\top}_{\pt}-\Iden)}
\end{aligned}
}
\]
\end{theorem}

\begin{theorem}[Joint training] For the model defined in (\ref{eqn:LinearAttn}), we consider independent linear data as defined in \ref{sec:assumptions} and loss function as defined in \ref{eqn:loss}, and suppose covariance matrices $\bSi_{\x},\{\bSi_{\bt_k}\}_{k=1}^K$ are full rank. Let $\W^\star, \{\bar\p_k^\star\}_{k=1}^K:=\arg\min_{\W, \{\bar\p_k\}_{k=1}^K}\mathcal{L}(\W, \{\bar\p_k\}_{k=1}^K)$, and $\mathcal{L}^\star=\mathcal{L}(\W^\star, \{\bar\p_k^\star\}_{k=1}^K)$. 
Additionally, let $\M:=\sum_{k=1}^K\pi_k(\bSi_{\beta_k}+\bmu_k\bmu_k^\top)$, and $ \bar\M:=\sum_{k=1}^K\pi_k\bSi_{\beta_k}$, then $\W^\star_{\textnormal{joint}},\bar\p^\star_k$ and $\mathcal{L}^\star_{\textnormal{joint}}$ satisfy
\[
\boxed{
\begin{aligned}
\W^\star_{\jt} &= \bSibt
\Bigg( \tr{\bSi_{\x}(\bSibt+\bSimu)} \Iden + \bSi_{\x}\red{\Big((n+1)\bSibt + \bSimu\Big)}\Bigg)^{-1}\\
\bar{\p}_k^\star &= \left((\W^\star_{\jt})^{-1} - n\bSi_{\x}\right)\bmu_k, k\in[K],\\
\mathcal{L}^\star_{\jt} &= \tr{\bSibt\bSi_{\x}}
-2n\tr{\W^\star_{\jt}\bSi_{\x}\bSibt\bSi_{\x}}
+n\tr{\W^\star_{\jt}\Big(\tr{\bSibt\bSi_{\x}}\bSi_{\x}+\bSi_{\x}\Big((n+1)\bSibt+ \bSimu \Big)\bSi_{\x}\Big)\W^{\star\top}_{\jt}\bSi_{\x}}
\end{aligned}
}
\]
\[
\bSbbt=\bSi_{\x}\bSibt,\quad\bSbmu=\bSi_{\x}\bSimu,\quad\Wb^\star_{\jt}=\bSi_{\x}\W^\star_{\jt}
\]
\[
\boxed{
\begin{aligned}
\Wb^\star_{\jt} &= \bSbbt
\Bigg( \tr{\bSbbt+\bSbmu} \Iden + \red{\Big((n+1)\bSbbt + \bSbmu\Big)}\Bigg)^{-1}\\
\bar{\p}_k^\star &= \left((\W^\star_{\jt})^{-1} - n\bSi_{\x}\right)\bmu_k, k\in[K],\\
\mathcal{L}^\star_{\jt} &= \tr{\bSbbt}
-2n\tr{\Wb^\star_{\jt}\bSbbt}
+n\tr{\Wb^\star_{\jt}\Big(\tr{\bSbbt+\bSbmu}\Iden+\Big((n+1)\bSbbt+ \bSbmu \Big)\Big)\Wb^{\star\top}_{\jt}}\\
&=\tr{\bSbbt}
-n\tr{\Wb^\star_{\jt}\bSbbt}
\end{aligned}
}
\]
\end{theorem}

==> backup/AISTATS_chklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

\textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}
% %%% END INSTRUCTIONS %%%


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes/No/Not Applicable]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes/No/Not Applicable]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes/No/Not Applicable]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes/No/Not Applicable]
   \item Complete proofs of all theoretical results. [Yes/No/Not Applicable]
   \item Clear explanations of any assumptions. [Yes/No/Not Applicable]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes/No/Not Applicable]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes/No/Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes/No/Not Applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes/No/Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes/No/Not Applicable]
   \item The license information of the assets, if applicable. [Yes/No/Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Yes/No/Not Applicable]
   \item Information about consent from data providers/curators. [Yes/No/Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Yes/No/Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Yes/No/Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Yes/No/Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Yes/No/Not Applicable]
 \end{enumerate}

 \end{enumerate}


==> sec/derivation.tex <==
\section{Derivations}
\subsection{Model Description}

Consider the model:
\[
y = \mathbf{x}^\top \boldsymbol{\beta} + \xi
\]
where:
\begin{itemize}
    \item \( \mathbf{x} \) is a \( d \)-dimensional Gaussian vector: \( \mathbf{x} \sim \mathcal{N}(0, \Sigma_x) \).
    \item \( \boldsymbol{\beta} \) follows a Gaussian Mixture Model (GMM):
    \[
    \boldsymbol{\beta} \sim \sum_{k=1}^K \pi_k \mathcal{N}(\mathbf{u}_k, \Sigma_{\beta_k})
    \]
    where \( \sum_{k=1}^K \pi_k = 1 \), \( \mathbf{u}_k \) is the mean vector, and \( \Sigma_{\beta_k} \) is the covariance matrix of the \( k \)-th component.
    \item \( \xi \) is a one-dimensional Gaussian noise: \( \xi \sim \mathcal{N}(0, \sigma^2) \).
\end{itemize}

\textbf{Objective}: Compute \( \mathbb{E}[y^2] \).

\subsection{Calculation Steps}

\subsubsection{1. Expand \( y^2 \) and Its Expectation}

First, express \( y^2 \) in terms of \( \mathbf{x} \), \( \boldsymbol{\beta} \), and \( \xi \):
\[
y = \mathbf{x}^\top \boldsymbol{\beta} + \xi \quad \Rightarrow \quad y^2 = (\mathbf{x}^\top \boldsymbol{\beta} + \xi)^2
\]
Expanding the square:
\[
y^2 = (\mathbf{x}^\top \boldsymbol{\beta})^2 + 2 (\mathbf{x}^\top \boldsymbol{\beta}) \xi + \xi^2
\]
Taking the expectation:
\[
\mathbb{E}[y^2] = \mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta})^2 \right] + 2 \mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta}) \xi \right] + \mathbb{E}\left[ \xi^2 \right]
\]

\subsubsection{Simplify Using Independence}

Assuming \( \mathbf{x} \), \( \boldsymbol{\beta} \), and \( \xi \) are mutually independent:
\[
\mathbb{E}[\xi] = 0 \quad \text{and} \quad \mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta}) \xi \right] = \mathbb{E}[\mathbf{x}^\top \boldsymbol{\beta}] \mathbb{E}[\xi] = 0
\]
Thus, the expression simplifies to:
\[
\mathbb{E}[y^2] = \mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta})^2 \right] + \mathbb{E}\left[ \xi^2 \right] = \mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta})^2 \right] + \sigma^2
\]

\subsubsection{Compute }

Notice that:
\[
(\mathbf{x}^\top \boldsymbol{\beta})^2 = \mathbf{x}^\top \boldsymbol{\beta} \boldsymbol{\beta}^\top \mathbf{x}
\]
Therefore:
\[
\mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta})^2 \right] = \mathbb{E}\left[ \mathbf{x}^\top \boldsymbol{\beta} \boldsymbol{\beta}^\top \mathbf{x} \right] = \mathbb{E}\left[ \text{Tr}\left( \boldsymbol{\beta} \boldsymbol{\beta}^\top \mathbf{x} \mathbf{x}^\top \right) \right] = \text{Tr}\left( \mathbb{E}\left[ \boldsymbol{\beta} \boldsymbol{\beta}^\top \right] \mathbb{E}\left[ \mathbf{x} \mathbf{x}^\top \right] \right)
\]
where we used the linearity of trace and the independence of \( \mathbf{x} \) and \( \boldsymbol{\beta} \).

Given \( \mathbf{x} \sim \mathcal{N}(0, \Sigma_x) \):
\[
\mathbb{E}\left[ \mathbf{x} \mathbf{x}^\top \right] = \Sigma_x
\]
Thus:
\[
\mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta})^2 \right] = \text{Tr}\left( \mathbb{E}\left[ \boldsymbol{\beta} \boldsymbol{\beta}^\top \right] \Sigma_x \right)
\]

\subsubsubsection{Compute \( \mathbb{E}\left[ \boldsymbol{\beta} \boldsymbol{\beta}^\top \right] \)}

Since \( \boldsymbol{\beta} \) follows a GMM:
\[
\mathbb{E}\left[ \boldsymbol{\beta} \boldsymbol{\beta}^\top \right] = \sum_{k=1}^K \pi_k \mathbb{E}\left[ \boldsymbol{\beta} \boldsymbol{\beta}^\top \mid k \right]
\]
For each Gaussian component \( k \):
\[
\mathbb{E}\left[ \boldsymbol{\beta} \boldsymbol{\beta}^\top \mid k \right] = \Sigma_{\beta_k} + \mathbf{u}_k \mathbf{u}_k^\top
\]
Therefore:
\[
\mathbb{E}\left[ \boldsymbol{\beta} \boldsymbol{\beta}^\top \right] = \sum_{k=1}^K \pi_k \left( \Sigma_{\beta_k} + \mathbf{u}_k \mathbf{u}_k^\top \right)
\]

\subsubsubsection{Substitute Back into \( \mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta})^2 \right] \)}

\[
\mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta})^2 \right] = \text{Tr}\left( \sum_{k=1}^K \pi_k \left( \Sigma_{\beta_k} + \mathbf{u}_k \mathbf{u}_k^\top \right) \Sigma_x \right)
\]
Using the linearity of trace:
\[
\mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta})^2 \right] = \sum_{k=1}^K \pi_k \text{Tr}\left( \Sigma_{\beta_k} \Sigma_x \right) + \sum_{k=1}^K \pi_k \text{Tr}\left( \mathbf{u}_k \mathbf{u}_k^\top \Sigma_x \right)
\]
Simplifying further:
\[
\text{Tr}\left( \mathbf{u}_k \mathbf{u}_k^\top \Sigma_x \right) = \mathbf{u}_k^\top \Sigma_x \mathbf{u}_k
\]
Thus:
\[
\mathbb{E}\left[ (\mathbf{x}^\top \boldsymbol{\beta})^2 \right] = \sum_{k=1}^K \pi_k \text{Tr}\left( \Sigma_{\beta_k} \Sigma_x \right) + \sum_{k=1}^K \pi_k \mathbf{u}_k^\top \Sigma_x \mathbf{u}_k
\]

\subsubsection{Combine All Components to Find \( \mathbb{E}[y^2] \)}

Substituting back into the expression for \( \mathbb{E}[y^2] \):
\[
\mathbb{E}[y^2] = \sum_{k=1}^K \pi_k \left( \text{Tr}\left( \Sigma_{\beta_k} \Sigma_x \right) + \mathbf{u}_k^\top \Sigma_x \mathbf{u}_k \right) + \sigma^2
\]

\subsection{Final Formula}

The expectation \( \mathbb{E}[y^2] \) is given by:
\[
\mathbb{E}[y^2] = \sum_{k=1}^K \pi_k \left( \text{Tr}\left( \Sigma_{\beta_k} \Sigma_x \right) + \mathbf{u}_k^\top \Sigma_x \mathbf{u}_k \right) + \sigma^2
\]
Alternatively, it can be expressed as:
\[
\boxed{
\mathbb{E}[y^2] = \text{Tr}\left(\M\Sigma_x  \right) + \sigma^2}
\]

\subsubsection{Explanation of Terms}

\begin{itemize}
    \item \( \sum_{k=1}^K \pi_k \text{Tr}\left( \Sigma_{\beta_k} \Sigma_x \right) \): This term accounts for the contribution of the covariance matrices of each mixture component and the covariance of \( \mathbf{x} \).
    \item \( \sum_{k=1}^K \pi_k \mathbf{u}_k^\top \Sigma_x \mathbf{u}_k \): This term captures the contribution of the mean vectors of each mixture component projected through \( \Sigma_x \).
    \item \( \sigma^2 \): This is the variance of the noise term \( \xi \).
\end{itemize}


==> sec/discuss.tex <==
\section{Discussion}
In this work, we revisited the loss landscape of in-context learning with 1-layer sequence models. We have established a general connection between ICL and gradient methods that accounts for correlated data, non-attention architectures (specifically SSMs), and the impact of low-rank parameterization including LoRA adaptation.

\noindent\textbf{Limitations.} The results of this work fall short of being a comprehensive theory for ICL in LLMs and can be augmented in multiple directions. First, while the exact equivalence between H3 and linear attention is remarkable, we should examine whether it extends to other SSMs. Secondly, while empirically predictive, our RAG and LoRA analyses are not precise and fully formal. Thirdly, it is desirable to develop a deeper understanding of multilayer architectures and connect to iterative GD methods as in \citep{ahn2024transformers,von2023transformers}. Finally, we have studied the population risk of ICL training whereas one can also explore the sample complexity of pretraining \citep{wu2023many,yuelu}. Moving beyond the theoretically tractable setup of this work, our simplified models are trained on in-context prompts from random initialization. Therefore, this theoretical study doesn't address more challenging in-context learning tasks, such as question answering, where both in-context demonstration and general knowledge from pretraining are required.  Future work in this area could also shed light on how certain contexts might elicit undesirable behaviors acquired by an LLM during pretraining, an aspect not covered in our current analysis. This work also studies a theoretical model for retrieval augmentation-based ICL. In a real-life retrieval augmentation-based ICL, one needs to account for the quality of the collection of the retrievable demonstrations and its (negative) impacts on the final predictions.
\begin{comment}
\begin{itemize}
    \item RAG and LoRA analysis is not exact
    \item focus on the single layer analysis only
    \item future work: analysis the 1-layer formula for minimizing averaged loss
\end{itemize}
\end{comment}

==> sec/fig_add_exp.tex <==
\begin{figure}[!t]
% \vspace{-10pt}
\centering
\begin{subfigure}{0.244\linewidth}
    \includegraphics[height=0.75\linewidth]{figs/avg_att.pdf}
\caption{Linear attention}\label{fig:avg att}
\end{subfigure}
\begin{subfigure}{0.244\linewidth}    
    \includegraphics[height=.75\columnwidth]{figs/avg_h3.pdf}
\caption{H3}\label{fig:avg h3}
\end{subfigure}
\begin{subfigure}{0.244\linewidth}    
    \includegraphics[height=.75\columnwidth]{figs/avg_test_risk.pdf}
\caption{Averaged risk}\label{fig:avg risk}
\end{subfigure}
\begin{subfigure}{0.244\linewidth}    
    \includegraphics[height=.75\columnwidth]{figs/distribution_shift_v3.pdf}
\caption{Evolving $\bt$}\label{fig:evolve}
\end{subfigure}

\caption{Comparison for linear attention and H3. Experimental details are discussed in Section~\ref{sec exp}.}
\label{fig:add exp}
% \vspace{-7pt}
\end{figure}

==> sec/fig_low_rank.tex <==
\begin{figure}[!t]
\centering
\begin{subfigure}{0.325\linewidth}
    \includegraphics[height=0.75\linewidth]{figs/rank_d5.pdf}
\caption{Low-rank ($d=5$)}\label{fig:low rank d5}
\end{subfigure}
\begin{subfigure}{0.325\linewidth}    
    \includegraphics[height=.75\columnwidth]{figs/rank_d20.pdf}
\caption{Low-rank ($d=20$)}\label{fig:low rank d20}
\end{subfigure}
\begin{subfigure}{0.325\linewidth}    
    \includegraphics[height=.75\columnwidth]{figs/lora_d20.pdf}
\caption{LoRA ($d=20$)}\label{fig:lora}
\end{subfigure}
\caption{Low-rank and LoRA experiments. In Figs.~\ref{fig:low rank d5} and \ref{fig:low rank d20}, we train low-rank linear attention by setting $\WK,\WQ\in\R^{(d+1)\times r}$ where $r$ is the rank restriction and $\W:=\WK\WQ^\top$. In Fig.~\ref{fig:lora}, we first pretrain the model using isotropic linear data. Then train additional $r$-rank LoRA weights to adapt the model to solve new distributed data using low rank matrices. }
\label{fig:low rank}
\end{figure}

==> sec/fig_overview.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=1\linewidth]{figs/overview_fig2.pdf}
% \caption{We investigate the optimization landscape of in-context learning from the lens of architecture choice, the role of distributional alignment, and low-rank parameterization.}
% of feature or task vectors
\label{fig:main}
%\vspace{-7pt}
\end{figure}

==> sec/fig_std_rag.tex <==
% \begin{figure}[!t]
% \centering
% \centering
% \begin{subfigure}{0.244\linewidth}
%     \includegraphics[height=0.75\linewidth]{figs/test_eqv_noise.pdf}
% \caption{Noisy label}\label{fig:noise}
% \end{subfigure}
% \begin{subfigure}{0.244\linewidth}
%     \includegraphics[height=0.75\linewidth]{figs/test_eqv_cov.pdf}
% \caption{Non-isotropic task}\label{fig:cov}
% \end{subfigure}
% \centering
% \centering
% \begin{subfigure}{0.244\linewidth}    
% \centering
%     \includegraphics[height=.75\columnwidth]{figs/test_rag_loss_v2.pdf}
% \caption{$\Lc^\st$}\label{fig:rag loss}
% \end{subfigure}
% \begin{subfigure}{0.244\linewidth}    

% \includegraphics[height=.75\columnwidth]{figs/test_rag_Ws_v2.pdf}
% \caption{$\Lc(\W^\st)$}\label{fig:rag Ws}
% \end{subfigure}
% \caption{Independent data and RAG experiments. Figs.~\ref{fig:noise} and \ref{fig:cov} show the ICL results using data generated via \eqref{data ind}. While Figs.~\ref{fig:rag loss} and \ref{fig:rag Ws} focus on the RAG setting where data obeys \eqref{data rag}. Solid and dashed curves correspond to the linear attention and H3 prediction results. Dotted curves present the theoretical results drawn from \eqref{formula ind} in Theorem~\ref{thm:independent} and \eqref{formula rag}. More details are discussed in Section~\ref{sec exp}.}
% \label{fig:add exp}

% \end{figure}

\begin{figure}[!t]
% \vspace{-10pt}
\centering
\centering
% \begin{subfigure}{0.325\linewidth}
\begin{subfigure}{0.244\linewidth}
    \includegraphics[height=0.75\linewidth]{figs/test_eqv_noise.pdf}
\caption{Noisy label}\label{fig:noise}
\end{subfigure}
\begin{subfigure}{0.244\linewidth}
    \includegraphics[height=0.75\linewidth]{figs/test_eqv_cov.pdf}
\caption{Non-isotropic task}\label{fig:cov}
\end{subfigure}
\begin{subfigure}{0.244\linewidth}
    \includegraphics[height=0.75\linewidth]{figs/test_ctf_fixed_2.pdf}
\caption{Task-feature alignment}\label{fig:corr feature}
\end{subfigure}
\centering
\centering
\begin{subfigure}{0.244\linewidth}    
\centering
    \includegraphics[height=.75\columnwidth]{figs/rank_d20.pdf}
\caption{Low-rank attention}\label{fig:low rank d20}
\end{subfigure}
\caption{Independent data, task-feature alignment and LoRA experiments. 
% Figs.~\ref{fig:noise} and \ref{fig:cov} show the ICL results using data generated via \eqref{data ind}. While Figs.~\ref{fig:rag loss} and \ref{fig:rag Ws} focus on the RAG setting where data obeys \eqref{data rag}. Solid and dashed curves correspond to the linear attention and H3 prediction results. Dotted curves present the theoretical results drawn from \eqref{formula ind} in Theorem~\ref{thm:independent} and \eqref{formula rag}. 
Experimental details are discussed in Section~\ref{sec exp}.}
% \vspace{-7pt}
\end{figure}





==> sec/idea.tex <==


\section{Problem Setup}

\noindent\textbf{In-context linear estimation.} Let prompt be $\Z=[\z_1^\top~\dots~\z_n^\top]^\top \in \R^{n \times (d+1)}$ where we set $\z_i=[\x_i^\top~y_i]^\top \in \R^{d+1}$ and $\z_{n+1}=[\x_{n+1}~0] \in \R^{d+1}$. When clear from context, we drop the subscript $n+1$ and set $\z=\z_{n+1},\x=\x_{n+1}$. The linear attention layer estimates the label $y$ associated to $\x$ via $F(\Z)=\z^\top\W\Z^\top\Z\vb$. Here $\hat\bt=\W\Z^\top\Z\vb$ provides an estimate of the true task vector $\bt$. Given a distribution $\Z\sim\Dc$, we optimize the linear attention layer as follows:
\[ 
\vbs,\Ws=\arg\min_{\vb,\W}\E[(y-F(\Z))^2].
\]
Suppose $\W=\begin{bmatrix}\W&\boldsymbol{0}\\?&?\end{bmatrix}\in\R^{(d+1)\times (d+1)}$ and $\vb=\begin{bmatrix}\boldsymbol{0}\\v\end{bmatrix}\in\R^{d+1}$. Then $\Z\vb=v\y$ and 
\[ 
F(\Z)=\z^\top \W\Z^\top \Z\vb=v \x^\top \W \X^\top \y.
\]
$\W\gets v\W$, $F(\Z)= \x^\top \W \X^\top \y$.
\begin{align} 
\E[(y-F(\Z))^2]&=\E[(\x^\top\bt-\x^\top \W \X^\top \y)^2]\\
&=\E[\x^\top (\bt- \W \X^\top \y)^2]=\E[ (\bt- \W \X^\top \y)\bSi(\bt- \W \X^\top \y)^\top]\\
&=\E[ \tn{\bSb(\bt- \W \X^\top \y)}]
\end{align}
\begin{definition}[Independent Data Model] We assume $\y_i=\x_i^\top\bt+w_i$ where $(\x_i)_{i=1}^{n+1}\sim\Nn(0,\bSi),\bt\sim\Nn(0,\B),(w_i)_{i=1}^{n+1}\sim\Nn(0,\sigma^2)$ are all independent. 
\end{definition}
\red{For vanilla analysis that prove optimal estimator is 1-step GD, we might not need Gaussian distribution.}

The papers \url{https://arxiv.org/pdf/2307.03576} and \url{https://arxiv.org/pdf/2306.00297} are providing a fairly detailed analysis of the standard data model above (under some assumptions on $\bSi,\B$). 

\noindent\textbf{Simplified Attention Model.} Assume $\w_{12}=0$ (top right of key-query) and $\vb_1=0$ (top $d$ entries of value). Justification: For independent data model, these cross-terms results in odd moments of the entries of the task $\bt$ and features $\x_i$ (e.g.~$\x^\top\W\x_i\x_i^\top\vb$ which is third order) whereas the target label $\x^\top\bt$ requires even moment terms. The fourth order term $\x^\top\w_{12}y_i\x_i^\top\vb$ can only explain 1 out of $d$ degrees of freedom of $\bt$, thus not useful for prediction as $d$ grows. Specifically, the fourth order term can only estimate $\bt$ using the fixed $\w_{12}$ direction via $\hat\bt=\w_{12}y_i\x_i^\top\vb$, thus can only reduce the error by a factor of $1/d$ (whenever distribution of $\bt$ sweeps all directions like $\Nn(0,\Iden)$).

%For our settings (RAG, Task-Feature alignment), these results in asymptotically inconsistent estimation i.e.~they provide noisy estimates as $n\rightarrow\infty$ hurting the eventual accuracy. Dedicate a section (potentially in appendix) to discuss why this assumption is warranted.

\subsection{How to analyze this model?} 
For simplicity, suppose covariances are isotropic and no noise. After some algebra, the analysis essentially boils down to the following expectation $\E[\tn{\bt-\W\X^\top\y}^2]$ where $\y=\X\bt$. Thus, we wish to study $\min_{\W}\E[\tn{(\Iden-\W\X^\top\X)\bt}^2]$. This can be approached in more than one ways. An important trick is orthogonal decomposition: Namely, let us set $\btb=\bt/\tn{\bt}$, $\g=\X\btb\sim\Nn(0,1)$, $\Xb=\X-\X\btb\btb^\top$, and observe that $\g,\Xb$ are independent and $\X=\Xb+\g\btb^\top$. We can then write
\begin{align}
\X^\top\X\btb=(\Xb^\top+\btb\g^\top)\g=\tn{\g}^2\btb+\Xb^\top\g.
\end{align}
Since $\g,\Xb$ are independent and $\Xb$ is effectively a $n\times (d-1)$ standard normal, the right hand side is approximately distributed as $\Nn(n\btb,n\Iden_d)$. In other words, using $\tn{\bt}\approx\sqrt{d}$, for $\hb\sim\Nn(0,\Iden_d)$,
\[ 
\frac{1}{n}\X^\top\y\approx \bt+\sqrt{\frac{d}{n}}\hb
\] 
Thus, 
\begin{align}
\E[\tn{\bt-\frac{1}{n}\W\X^\top\y}^2]&\approx \E[\tn{(\Iden-\W)\bt}^2]+\E[\tn{\W\hb}^2]/n\\
&=\text{trace}((\Iden-\W)(\Iden-\W^\top)+\frac{d}{n}\W\W^\top)\\
&=\text{trace}(\Iden-\W-\W^\top+(1+\frac{d}{n})\W\W^\top).
\end{align}
Differentiating, the optimal $\W$ is given by $\Ws\approx\frac{n}{n+d}\Iden$.

\vspace{-5pt}
\subsubsection{Analysis outline for general covariance}
We can use the above strategy but we should whiten the covariances. \red{I believe the analysis below already generalizes the results of \url{https://arxiv.org/pdf/2307.03576} which assumes $\bSi=\B^{-1}$.} For instance, set $\X=\Xa\bSb$ where $\bSb=\sqrt{\bSi}$ and $\Xa$ is now $\Nn(0,1)$. Now set $\bta=\bSb\bt$ and $\btb=\bta/\tn{\bta}$. We have $\X\bt=\Xa\bSb\bt=\Xa\bta$ and set $\g=\Xa\btb\sim\Nn(0,\tn{\btb}^2\Iden)$. We similarly decompose 
\[ 
\Xa=\Xb+\g\btb^\top
\] 
where $\Xb,\g$ are independent. Set $\Sb=\bSb\B\bSb$. Noting $\E[\tn{\bt_0}^2]=\tr{\Sb}:=M$, we can then write
\[
\frac{1}{n}\X^\top\y=\frac{1}{n}\bSb\Xa^\top\Xa\bta\approx \bSb(\bt_0+\sqrt{\frac{M}{n}}\hb).
\]
The MSE error is given by (after accounting for $\x$'s covariance)
\[ 
\E[\tn{\bt_0-\frac{1}{n}\bSb\W\X^\top\y}^2]=\E[\tn{\bt_0-\bSb\W\bSb(\bt_0+\sqrt{\frac{M}{n}}\hb)}^2]
\] 
Now define the change-of-variable $\Wz=\bSb\W\bSb$. Recalling $M=\tr{\Sb}$, we can then write
\begin{align}
\E[\tn{\bt_0-\Wz(\bt_0+\sqrt{\frac{M}{n}}\hb)}^2]&=\E[\tn{(\Iden-\Wz)\bt_0}^2]+\frac{M}{n}\tr{\Wz\Wz^\top}\\
&=M-2\tr{\Wz\Sb}+\tr{\Wz\Sb\Wz}+\frac{M}{n}\tr{\Wz\Wz^\top}.\label{loss function}
\end{align}

Differentiating, we basically obtain % and setting $\Sb=\sqrt{\Sb}$
\[ 
\Sb=\Sb\Wz+\frac{M}{n}\Wz\implies \Iden=(\Iden+\frac{M}{n}\Sb^{-1})\Wz\implies \Wz=(\Iden+\frac{M}{n}\Sb^{-1})^{-1}.
\] 
This then yields $\Ws=(\bSi+\frac{M}{n}\B^{-1})^{-1}$. This solution strictly generalizes and recovers the Identity covariance model. Crucially, through this, we can likely figure out what LoRa does. This is because performance is controlled by the combined covariance matrix $\Sb=\bSb\B\bSb$.

\begin{lemma}[Optimizing Low-rank Attention Weights]\label{low rank attn} Suppose we use attention parameterization $\W_q,\W_k\in\R^{d\times r}$ which enforces $\text{rank}(\W)\leq r$. Consider the population objective \eqref{loss function} given by
\[ 
\Lc(\Wz)=\tr{\Sb}-2\tr{\Wz\Sb}+\tr{\Wz\Sb\Wz}+\frac{M}{n}\tr{\Wz\Wz^\top}.
\]
Denoting $\la_i$ to be the $i$'th largest eiganvalue of $\Sb$, we have that 
\[
\min_{\text{rank}(\Wz)\leq r}\Lc(\Wz)=\tr{\Sb}-\sum_{i=1}^r\frac{\la_i^2}{\la_i+M/n}.
\]
Noting $\tr{\Sb}=\sum_{i=1}^n\la_i$ and removing the rank constraint, this reduces to the standard optimal risk
\[ 
\min_{\Wz}\Lc(\Wz)=\sum_{i=1}^d\frac{1}{n/M+1/\la_i}.
\]
\end{lemma}
\begin{proof} 
Let us parameterize $\Wz=\Ub\La\Ub^\top$ where $\Ub\in\R^{d\times r}$ is the eigenvectors of $\Wz$. We will first treat $\Ub$ as fixed and optimize $\La\in\R^{r\times r}$. We will then optimize $\Ub$. Fixing $\Ub$ and setting $\Sbb=\Ub^\top\Sb\Ub$ and setting $\Lc'(\La)=\Lc(\Wz)-\tr{\Sb}$, we have that 
\begin{align}
\Lc'(\La)&=\tr{\Sbb\La^2}+\frac{M}{n}\tr{\La^2}-2\tr{\La\Sbb}.
\end{align}
Differentiating, we obtain $\La^*=(\Iden+\frac{M}{n}\Sbb^{-1})^{-1}$. Let $\s_i$ denote the eigenvalues of $\Sbb$. Plugging in this value, we obtain the optimal risk given by
\[ 
\Lc^*:=\Lc^*(\Ub)=-\sum_{i=1}^r s_i (1+\frac{M}{ns_i})^{-1}=-\sum_{i=1}^r\frac{ns_i}{M/s_i+n}.
\]
Now observe that, the right hand side is strictly decreasing function of the eigenvalues $s_i$ of $\Ub^\top\Sb\Ub$. Thus, to minimize $\Lc^*(\Ub)$, we need to maximize $\sum_{i=1}^r\frac{ns_i}{M/s_i+n}$. It follows from Cauchy's interlace theorem that $s_i\leq \la_i$ where $\la_i$ is the $i$th largest eigenvalue of $\Sb$ since $\Sbb$ is an orthogonal projection of $\Sb$ on $\Ub$. Consequently, we find the desired bound.
\end{proof}


\noindent\textbf{Impact of LoRA:} Based on the above Lemma \ref{low rank attn}, under jointly-diagonalizable new and old eigenvalues of $\Sb,\Sb^{old}$ $(\la_i)_{i=1}^d,(\la_i^{old})_{i=1}^d$; LoRA obtains top $r$ eigenvalue indices $\Ic$ maximizing the function $\texttt{gain}_i=\frac{1}{n/M+1/\la^{old}_i}-\frac{1}{n/M+1/\la_i}$. That means, LoRA's risk is given by
\[ 
\Lc(\W_{lora})=\min_{|\Ic|\leq r,\Ic\subset[d]}\sum_{i\in\Ic}\frac{1}{n/M+1/\la_i}+\sum_{i\not\in\Ic}\frac{1}{n/M+1/\la^{old}_i}
\]
Note that, this only provides a lower bound as we have to prove that the optimal LoRA-updated model $\W_{lora}$ is also jointly diagonalizable with covariances $\Sb,\Sb^{old}$, and $\W^{old}$.


\begin{comment}
and letting $s_i=\Sbb_{ii}$, we have that
\begin{align}
\Lc'(\La)&=\tr{\Sbb\La^2}+\frac{M}{n}\tr{\La^2}-2\tr{\La\Sbb}\\
&=\sum_{i=1}^r \la_i^2(\frac{M}{n}+s_i)-2\la_is_i.
\end{align}
Differentiating, we obtain $\la^*_i=(1+\frac{M}{ns_i})^{-1}=s_i(s_i+\frac{M}{n})^{-1}$. Next, let us study the risk which is given by plugging the optimal $\La^*$
\[ 
\Lc^*=-\sum_{i=1}^d s_i (1+\frac{M}{ns_i})^{-1}=-\sum_{i=1}^d\frac{ns_i}{M/s_i+n}.%-\sum_{i=1}^d\frac{ns_i^2}{M+ns_i}=
\]
\noindent\red{\textbf{Basic LoRa analysis:}} Assume that new and old covariances are jointly diagonalizable (e.g.~$\bSi_{old},\bSi_{new}$). Write the loss function \eqref{loss function} in terms of a sum over eigenvalues. Then determine which $r$ eigenvalues of the old distribution's $\W_{\text{old}}$ should be updated and matched to new optimal $\W_{new}$ by LoRa.

Exact LoRa objective is: Suppose $\Wz$ is fixed
\begin{align}
\Lc(\Lb)=M-2\tr{(\Wz+\Lb)\Sb}+\tr{(\Wz+\Lb)\Sb(\Wz+\Lb)}+\frac{M}{n}\tr{(\Wz+\Lb)(\Wz+\Lb)^\top}.\label{loss function}
\end{align}
If $\Lb$ was full rank, solution is $\Lb_\st=(\Iden+\frac{M}{n}\Sb^{-1})^{-1}-\Wz$.
\end{comment}


\subsubsection{Simplifying assumptions} 
Initially, we can benefit from following assumptions:
\begin{itemize}
\item For standard data model, the optimal attention model has the form $\W=\begin{bmatrix}\W'&0\\0&0\end{bmatrix}$ where $\W'\in\R^{d\times d}$. The choice of bottom row has no impact beacuse we set $\z=[\x~0]$ which zeroes it out. Setting top-right column to 0 suppresses the label-feature term of the form $y_i\x$. For standard data model, it can be shown that, these label-feature terms increase the test error and are undesirable, thus, optimal solution zeroes them out.
\item Similarly, optimal value matrix has the form $\vb=\begin{bmatrix}\vb'\\v\end{bmatrix}$ where $\vb'=0$. $\vb'\in\R^d$ picks up second-order features $\x_i\x_i^\top$ which are not useful for prediction. Thus, optimal solution zeroes them out and only $v$ remains.
\item We can assume $\W'$ is a symmetric matrix. Again this should be proven for all optimal solutions, but it may simplify notation/analysis.
\end{itemize}
\begin{comment}
\begin{proposition}[Optimal Linear Attention]
\end{proposition}
\begin{proof} Without losing generality, denote $\W'\gets \begin{bmatrix}\W~\w\\0~0\end{bmatrix}$ since $\z=[\x~0]$ and final row of $\W$ gets hit by zero. Also set $\vb'\gets \begin{bmatrix}\vb\\v\end{bmatrix}$. Observe that 
\begin{align}
\W'\Z^\top\Z\vb&=\W\X^\top\X\vb+v\W\X^\top\y +\w\y^\top \X\vb+v\w\y^\top\y.
%&=\W\X^\top\X\vb+v\W\X^\top\X\bt +\w\bt^\top\X^\top \X\vb+v\w\bt^\top\X^\top\X\bt\\
\end{align}
The prediction error (w.r.t.~noiseless label $y$ i.e.~$\sigma^2$ subtracted for noisy label) is given by 
\[ 
\Lc(\vb,\W,\w)=\E[(\x^\top(\bt-\W'\Z^\top\Z\vb'))^2]=\E[\tn{\bt-\W'\Z^\top\Z\vb'}^2],
\]
assuming $\bSi=\Iden$. We observe that optimal error is given by fitting the $v\W\X^\top\y $ term. Setting $\W\gets v\W$, we aim to control
%Let $\bth$ be the estimate of $\bt$. We have that 
\begin{align}
\Lc(\vb,\W,\w)&=\E[\tn{\bt-\W\X^\top\y}^2]=\E[\tn{(\Iden-\W\X^\top\X)\bt-\sigma\W\X^\top\z}^2]\\
&=\E[(\Iden-\W\X^\top\X)\B(\Iden-\W\X^\top\X)]+\sigma^2\E[\tn{\W\X^\top\z}^2].
\end{align} 
\end{proof}
\end{comment}
\subsection{Non-standard Data Models}

\noindent\textbf{Scenario 1: Retrieval-Augmented Generation.} In this model, we draw the query vector $\x$ and task vector $\bt$. We then draw data $(\x_i)_{i=1}^n$ to be used in-context according to the rule $\text{corr\_coef}(\x,\x_i)\geq \alpha>0$. An alternative simpler model is assuming $\x_i\sim\Nn(\alpha\x,(1-\alpha^2)\Iden)$ with $\x\sim\Nn(0,\Iden)$. All labels obey $\y_i=\x_i^\top \bt+w_i$. The \textbf{key takeaway} is leveraging aligned ICL data for better prediction along query.

\noindent\textbf{Proof strategy.} Start by decomposing $\X^\top\X=(\rho\X'+\alpha \onebb\x^T)^T(\rho\X'+\alpha \onebb\x^T)$ where $\rho=\sqrt{1-\alpha^2}$ and $\X'$ has i.i.d.~$\Nn(0,1)$ entries. Proceed by writing $\X^\top\X\bt$ which will provide terms in the form $\x\x^\top\bt$. Hitting this with $\x^\top$ from left will provide a useful $\x^\top\bt$ term which will help estimate $y$.

\vspace{10pt}
\noindent\textbf{Scenario 2: Task-Feature Alignment.} In this model, we first draw $\bt$ and then draw $\x_i\sim\Nn(\alpha\bt,\bSi)$. The \textbf{key takeaway} is leveraging the task-feature alignment for stronger estimation of the task vector.

\noindent\textbf{Proof strategy.} Start by decomposing $\X^\top\X=(\rho\X'+\alpha \onebb\bt^T)^T(\rho\X'+\alpha \onebb\bt^T)$ where $\rho=\sqrt{1-\alpha^2}$ and $\X'$ has i.i.d.~$\Nn(0,1)$ entries. Proceed by writing $\X^\top\X\bt$ which will provide useful terms along $\bt$ direction.

\vspace{10pt}
\noindent\textbf{Scenario 3: Distribution Shift with LoRa.} We train the model on $\Dc_1=(\bSi_1,\B_1)$ distribution to obtain $\W_1$. We are then given a new distribution $\Dc_2=(\bSi_2,\B_2)$. We adapt to $\Dc_2$ using LoRa on $\W_1$, that is, we ask for $\W_2$ such that $\text{rank}(\W_2-\W_1)\leq r$. The \textbf{key takeaway} is understanding how LoRa enables adaptation (e.g. we expect LoRa to update along the principal eigendirections of the difference between the two task distributions/covariances).

\vspace{10pt}
\noindent\textbf{Scenario 4: State-Space Models.} We consider the H3-like convolutional model. In its seq2seq form, the model is given by
\[ 
\text{SSM}(\Z) = ((\Z\W_1 \odot \Z\W_2) \ast \fb) \odot (\Z\W_3),
\] 
where $\fb\in\R^n$ is a 1-D convolution filter and $\W_{1,2,3}$ are weight matrices that correspond to K/V/Q of the attention layer, respectively. $\fb$ facilitates the aggregation of the key-value products. As explained in Section \ref{ssm blueprint}, this model can be used to perform one gradient step similar to linear attention. The \textbf{key takeaways} are
\begin{itemize}
\item Establishing the first result on the loss landscape of SSM-based ICL. Does the optimal SSM take gradient step?
\item Can SSM solve a distribution beyond linear attention?
\end{itemize}
To address the second question, our hypothesis is that SSM can leverage the convolutional filter $\fb$ to capture positional priors. Specifically, rather than vanilla gradient step $\bth=\frac{1}{n}\W\X^\top\y$, SSM can make the position-weighted update $\bth=\frac{1}{n}\W\X^\top(\fb\odot\y)=\frac{1}{n}\sum_{i=1}^n\W \fb_i\x_i y_i$. Here through $\fb$, we can weight the samples, in practice, we can do a recency weighting based on SSM e.g. setting $\fb_i=\rho^i$ for $i\geq 1$ corresponds to applying exponential smoothing along the context window during ICL.

\noindent\textbf{Dataset Model for SSM (temporal task shift).} Consider the following dataset where task distribution is shifting over time. Specifically draw $\bt\sim\Nn(0,\Iden)$ and draw $\bt_i$ IID such that $\bt_i\sim\Nn(\alpha_i\bt,(1-\alpha_i^2)\Iden)$. This way, at time $i$, task vector is $\alpha_i$-correlated to the task vector at time $n+1$. Set data $y_i=\x_i^\top\bt_i+w_i$. We wish to show that these correlations can be captured by the optimal convolution filter $\fb$ to obtain better estimation.

\subsection{In-context Linear Estimation with SSM}\label{ssm blueprint}
To implement 1 gradient step in-context, let us consider the following 1 layer SSM block \footnote{\noindent\emph{Remark:} This model is similar to H3 \url{https://arxiv.org/pdf/2212.14052.pdf}.}
\[
\text{SSM}(Z) = ((ZW_1 \odot ZW_2) \ast F) \odot (ZW_3).
\]
Blueprint for in-context learning:
\begin{enumerate} 
\item Get $X=[x_1 \dots x_L]^\top$ via $X=ZW_1$
\item Get labels $Y$ via $Y=ZW_2$.
\begin{itemize}
\item Here we can set $W_2$ to be a vector so that $Y\in\R^L$ is enforced to be a vector (to help the model grab labels).
\end{itemize}
\item Elementwise product $E=X \odot Y\in\R^{L\times d}$
\item Convolve $E \ast F$ where causal filter $F=[0~\texttt{all\_ones}]\in\R^L$ to obtain $\hat{\beta} = X^TY$.
\begin{itemize}
\item Note that, filter is shifted by 1 to ensure we use first $i-1$ samples to predict $y_i$.
\item I bet we can use a state-space model and population minima will still be the all\_ones filter. 
\end{itemize}
\item Elementwise $\hat{\beta} \odot x_{L+1}$ and then collapse with $\texttt{all\_ones}\in\R^d$ to get prediction $\hat y$. Here, we simply set $W_3=W_1$.
\end{enumerate}




==> sec/main.tex <==
\section{Main Results}\label{sec:main}
  In this section, we train and optimize the single-layer linear attention model in a multi-task linear regression ICL setting with dataset described in Definition~\ref{definition:multi-task}, and characterize the loss landscape $\Lc^\st_\pt$, $\Lc^\st_\ft$ and $\Lc^\st_\jt$ in Section~\ref{sec:PGD} under different settings. 
\subsection{Loss landscape optimization }
\label{sec:landscape}
Recap the multi-task ICL dataset from Definition \ref{definition:multi-task} where $\bSi_{\x}$ is the shared covariance matrix of the input features and $\{(\bmu_k,\bSi_{\bt_k})\}_{k=1}^K$ are the task mean vectors and covariance matrices. In the main paper, we consider noiseless data setting where $\sigma=0$. We defer the exact analysis considering noisy labels to \chang{ Appendix}.

% We first consider the following independent linear data distribution. Let $\bSi_{\x}, \{\bSi_{\bt_k}\}_{k=1}^K$ be the covariance matrices of the input features and task parameters and $\sigma\ge 0$ be the noise level \YL{Are we assuming $\sigma=0$?}. From the multi-task definition.~\ref{definition:multi-task} we have:
% \begin{align}
% &\bt\sim\sum_{k=1}^K \pi_k\Nn(\bmu_k,\bSi_{\beta_k}),\bt_k\sim\Nn(\bmu_k,\bSi_{\beta_k}),k\in[K],\notag\\&\x_i\sim\Nn(0,\bSi_{\x}),\xi_i\sim\Nn(0,\sigma^2), i\in[n+1]
% \label{eqn:assumption}
% \end{align}
% and the label is obtained via $y=\x^\top\bt+\xi$. 
% \red{According to Assumption~\ref{assumption:PGD}, our following results characterize the optimal solution of the settings in Section~\ref{sec:icl}. Then the ICL objective becomes:}
% \begin{align}
%     &\Lc(\W,\Pb)=\sum_{k=1}^K \pi_k \Lc_k(\W,\p_k) \label{eqn:loss}\\
%     &\text{where }\Lc_k(\W,\p_k)=\E_{(\Z,y)\sim\Dc_k}\left[( f_\att(\Z^{(k)})-y )^2\right].\nn
% \end{align}
% \begin{align}
%     &\Lc(\W,\{\bar\p_k\}_{k=1}^K)=\sum_{k=1}^K \pi_k \E\left[\left( f(\X, \y, \x; \W,\bar\p_k)-y \right)^2\right] \notag\\
%     &=\sum_{k=1}^K\pi_k \E\left[\left( \x^\top \A_k \right)^2\right]\notag   \\
%     &\text{where }\A_k=(\W\X^\top\X-\Iden_d)\bt_k+\W\bar\p_k. 
%     \label{eqn:loss}
% \end{align}



% \YL{We can write pretraining results in a separate theorem and finetuning results can be more general for any $\W$}

We first analyze the plain training setting where no additional task-specific parameters are introduced, and all $K$ tasks are mixed together. 
\begin{theorem} [Plain training]\label{thm:pretrain} Consider training a single-layer linear attention model in solving multi-task ICL problem with dataset defined in Definition~\ref{definition:multi-task} and model construction as described in Assumption~\ref{assumption:PGD}. Let the optimal solution $\W_{\pt}^\st$ (c.f.~\eqref{eqn:obj pt}) and the minimal plain training loss $\Lc_\pt^\st$ as defined in Section~\ref{sec:PGD}. 
Additionally, let 
\begin{align*}
&\bSbbt=\bSi_{\x}\left(\sum_{k=1}^K\pi_k\bSi_{\bt_k}\right),\\
&\bSbmu=\bSi_{\x}\left(\sum_{k=1}^K\pi_k\bmu_k\bmu_k^\top\right),\\
&\text{and}\quad\Wb^\st_\pt=\bSi_{\x}\W^\st_\pt.
\end{align*}
Then the solution $\Wb^\star_{\pt}$ and optimal loss $\Lc^\st_\pt$ satisfy
\begin{tcolorbox}[colback=white!5!white,colframe=black!5!black,colback=white!5!white,
                  %%enhanced,
                  %%frame hidden,
                  interior hidden,
                  arc=0pt,
                  boxrule=1pt,
                  boxsep=0pt,
                  left=5pt,
                  right=5pt,
                  top=-5pt,]
\[
\scalemath{0.83}{\Wb^\star_{\pt}=(\bSbbt+\bSbmu)\left((n+1)(\bSbbt+\bSbmu)+\tr{\bSbbt+\bSbmu}\Iden\right)^{-1},}
\]
\[
\scalemath{0.95}{\Lc^\star_{\pt} 
=\tr{\bSbbt+\bSbmu}
-n\tr{\Wb^\star_{\pt}(\bSbbt+\bSbmu)}.}
\]
% \begin{align*}
% &\scalemath{0.95}{\Wb^\star_{\pt}=\left((n+1)\Iden+\tr{\bSbbt+\bSbmu}(\bSbbt+\bSbmu)^{-1}\right)^{-1},}\\
% &\scalemath{0.95}{\Lc^\star_{\pt} 
% =\tr{\bSbbt+\bSbmu}
% -n\tr{\Wb^\star_{\pt}(\bSbbt+\bSbmu)}.}
% \end{align*}
\end{tcolorbox}
\end{theorem}
Note that the above solution and optimal loss are identical to those in previous work \chang{cite} when considering a single-task ICL problem with zero task mean and isotropic task covariance $\bSibt$. 

% Here, due to the bias in the dataset, i.e., 
% $\E[\bt_k]=\bmu_k\neq\zerbb$, the penalty term 
% $\tr{\bSbmu}$ appears in 
% $\Lc^\st_\pt$. Next, we investigate whether this penalty introduced by the mean can be eliminated and consider the fine-tuning setting (c.f.~\eqref{eqn:obj ft}) where task-specific prompts are applied.


\begin{theorem} [Fine-tuning]\label{thm:pretrain-finetune} Suppose a pretrained model as described in Theorem~\ref{thm:pretrain} is given with $\W^\st_\pt$ being its optimal solution. Consider fine-tuning this model with task-specific prompts as defined in Definition~\ref{def:task-specific param}, and let the optimal prompt matrix $\Pb^\st_\ft$ (c.f.~\eqref{eqn:obj ft}) and the minimal fine-tuning loss $\Lc^\st_\ft$ be defined in Section~\ref{sec:PGD}. Additionally, let $\bSbbt,\bSbmu,\Wb^\st_\pt$ follow the same definitions as in Theorem~\ref{thm:pretrain} and define the mean matrix
\[
\M_\mu=[\bmu_1~\cdots~\bmu_K]^\top\in\R^{K\times d}.
\]
Then the solution $\Pb^\st_\ft$ and optimal loss $\Lc^\st_\ft$ satisfy 
\begin{tcolorbox}[colback=white!5!white,colframe=black!5!black,colback=white!5!white,
                  %%enhanced,
                  %%frame hidden,
                  interior hidden,
                  arc=0pt,
                  boxrule=1pt,
                  boxsep=0pt,
                  left=5pt,
                  right=5pt,
                  top=3pt,]
\[
\scalemath{0.95}{\Pb^\st_\ft = \M_\mu\left((\W^\star_{\pt})^{-1} - n\bSi_{\x}\right),}
\]
\[
\scalemath{0.95}{\Lc^\star_\ft
=\Lc^\star_{\pt}-\tr{\bSbmu(n\Wb^{\star}_{\pt}-\Iden)^2}.}
\]
% \begin{align*}
% % &\scalemath{0.95}{\bar{\p}_k^\star = \left((\W^\star_{\pt})^{-1} - n\bSi_{\x}\right)\bmu_k, k\in[K],}\\
% &\scalemath{0.95}{\Pb^\st_\ft = \M\left((\W^\star_{\pt})^{-1} - n\bSi_{\x}\right),}\\
% &\scalemath{0.95}{\Lc^\star_\ft
% =\Lc^\star_{\pt}-\tr{\bSbmu(\Wb^{\star}_{\pt}-\Iden)^\top(\Wb^{\star}_{\pt}-\Iden)}.}
% \end{align*}
\end{tcolorbox}
\end{theorem}
Results in Theorem~\ref{thm:pretrain-finetune} show that, fine-tuning achieves better loss than plain training, $\Lc^\st_\ft\leq\Lc^\st_\pt$, and our results provably quantize the loss difference.



\begin{theorem}[Joint training]\label{thm:joint-training} Consider training a single-layer linear attention model in solving multi-task ICL problem with dataset defined in Definition~\ref{definition:multi-task} and model construction as described in Assumption~\ref{assumption:PGD}. Let $\W_{\jt}^\st,\Pb^\st_\jt$ (c.f.~\eqref{eqn:obj jt}) be the optimal solutions and $\Lc_\jt^\st$ is the optimal joint training loss defined in Section~\ref{sec:PGD}. 
Additionally, let $\bSbbt,\bSbmu,\M_\mu$ follow the same definitions as in Theorem~\ref{thm:pretrain-finetune} and define $\Wb^\st_\jt=\bSi_{\x}\W^\st_\jt$. Then the solution $(\W_{\jt}^\st,\Pb^\st_\jt)$ and optimal loss $\Lc^\st_\jt$ satisfy 
\begin{tcolorbox}[colback=white!5!white,colframe=black!5!black,colback=white!5!white,
                  %%enhanced,
                  %%frame hidden,
                  interior hidden,
                  arc=0pt,
                  boxrule=1pt,
                  boxsep=0pt,
                  left=5pt,
                  right=5pt,
                  top=-5pt,]
% \[
% \scalemath{0.93}{\Wb^\star_{\jt} = 
% \left( (n+1)\Iden + \tr{\bSbbt}\bSbbt^{-1}+(\tr{\bSbmu} + \bSbmu)\bSbbt^{-1}\right)^{-1},}
% \]
% \[
% \scalemath{0.93}{\Wb^\star_{\jt} = 
% \left( (n+1)\Iden + \tr{\bSbbt+\bSbmu} \bSbbt^{-1} + \bSbmu\bSbbt^{-1}\right)^{-1},}
% \]
\[
\scalemath{0.9}{\Wb^\star_{\jt} = \bSbbt
\Big(\Big((n+1)\bSbbt + \bSbmu\Big)+ \tr{\bSbbt+\bSbmu} \Iden\Big)^{-1},}
\]\[
\scalemath{0.95}{\Pb_\jt^\star = \M_\mu\left((\W^\star_{\jt})^{-1} - n\bSi_{\x}\right),}
\]
\[
\scalemath{0.95}{\Lc^\star_{\jt} =\tr{\bSbbt}-n\tr{\Wb^\star_{\jt}\bSbbt}.}
\]
\end{tcolorbox}
\end{theorem}


 The results of Theorem~\ref{thm:pretrain-finetune} and Theorem~\ref{thm:joint-training} highlight an important commonality of the optimal prompt:
the optimal prompts $\pbb_k$ capture the mean of corresponding tasks based on the attention weight $\W^\st_\pt$ and $\W^\st_\jt$ . For a large context length $n$, $(\pbb_k)^\st_\ft$ and $(\pbb_k)^\st_\jt$ will be approximately $-n\bSi_{\x}\bmu_k$.

\YL{Discuss that when $n$ is large enough, all solutions are the same. Therefore the benefits of joint/finetune is more visible for finite $n$.}

Additionally, regardless of the training setting, the optimal prompts $\Pb^\star$ consistently maintain the same functional relationship with the optimal $\W^\st$, which implies:
\begin{corollary}
Let $\Lc^\st_\pt$ and $\Lc^\st_\ft$ be the optimal plain training and fine-tuning loss given in Theorem~\ref{thm:pretrain} and Theorem~\ref{thm:pretrain-finetune}, there exists a shared single-variable functional relationship $\Lc(\W, \Pb^\st(\W))$ for $\W^\st_\pt,\W^\st_\jt$:
 $$\Lc^\st_\ft= \Lc(\W^\st_\pt,\Pb^\st(\W^\st_\pt)),  \Lc^\st_\jt= \Lc(\W^\st_\jt, \Pb^\st(\W^\st_\jt)),$$
 which implies an alternative but shared form of $\Lc^\st_\ft$ and $\Lc^\st_\jt$ in Theorem~\ref{thm:pretrain-finetune} and Theorem~\ref{thm:joint-training}.
 \label{corollary:shared form}
\end{corollary}
Due to the space limit and the complexity of the explicit form of $\Lc(\W, \Pb^\st(\W))$, we defer the details to the \chang{Appendix}. It can also be shown that $\W^\st_\jt$ is the unique minimizer of $\Lc(\W, \Pb^\st(\W))$, leading to the inequality 
$\Lc^\star_\jt \leq \Lc^\star_\ft$, and thus:

\begin{corollary}
\label{corollary:ordering}
Let $\Lc^\st_\pt$, $\Lc^\st_\ft$, and $\Lc^\st_\jt$ denote the optimal loss values for plain training, fine-tuning, and joint training, as described in Theorem~\ref{thm:pretrain}, Theorem~\ref{thm:pretrain-finetune}, and Theorem~\ref{thm:joint-training}, respectively. These losses satisfy the following relationship:
\[
\Lc^\st_\jt \leq \Lc^\st_\ft \leq \Lc^\st_\pt.
\]
Equality holds if and only if $\bSimu = \zerbb_{d \times d}$.
\end{corollary}



\subsection{Covariance-mean decoupling}\label{thm:vector head}
It is worth noting that in Section~\ref{sec:landscape}:

\YL{Explain what does covariance-mean decoupling mean}
\begin{itemize}
    \item For a single-layer linear attention model following the constructions in Assumption~\ref{assumption:PGD}, where $\W \in \R^{d \times d}$ captures all the statistics, the plain training loss $\Lc^\star_\pt$ is determined by the second-order moments of the task parameters $\bt_k$, specifically:
    $$
    \E[\bt_k \bt_k^\top] = \bSi_{\bt_k} + \bmu_k \bmu_k^\top,
    $$
    which represents a coupled variable of the task covariance and the task mean. As a result, $\Lc^\star_\pt$ can be seen as a function of this \textbf{covariance-mean coupled} variable, denoted as $\bSbbt + \bSbmu$ (see Theorem~\ref{thm:pretrain}), which appears both in the expression for $\W^\st_\pt$ and in $\Lc^\st_\pt$:
    $$
    \Lc^\star_\pt = \Lc^\star_\pt\left(\W^\st_\pt(\{\bSbbt + \bSbmu\}_i), \{\bSbbt + \bSbmu\}_j\right).
    $$
    Here, the index $i$ refers to the $i$-th instance of the coupled variable $\bSbbt + \bSbmu$ within $\W^\st_\pt$, while $j$ refers to its $j$-th instance as it appears directly in $\Lc^\star_\pt$, outside of $\W^\st_\pt$.


    \item When all tasks have zero mean, i.e., $\E[\bt_k] = \bmu_k = \mtx{0}$ for all $t \in [K]$, which leads to $\bSbmu=\zerbb_{d\times d}$, the optimal losses for pretraining, fine-tuning, and joint training are identical. As a result, prompt fine-tuning during any stage does not improve the pretrained model (see Theorem~\ref{thm:pretrain-finetune},~\ref{thm:joint-training}):
    \begin{align}
        \bmu_k = \mtx{0}, k\in[K] \Rightarrow \Lc^\star_\pt = \Lc^\star_\ft = \Lc^\star_\jt.
        \label{eqn:zero_mean_loss}
    \end{align}
    In this case, the fine-tuned prompts are all zero vectors and have learnt nothing during the fine-tuning phase, which follows as a corollary from Theorem~\ref{thm:pretrain-finetune} and Theorem~\ref{thm:joint-training}. Additionally, this observation implies: it is the coupling between $\bSbbt$ and $\bSbmu$ that leads to the loss difference, since setting task means to zero will eliminate the loss difference. 
    \chang{Experimentally, Eqn.~\ref{eqn:zero_mean_loss} can be verified.}
\item The degree of covariance-mean decoupling can be regarded as a perturbation $\lambda\bSbmu (0\le\lambda\le 1)$ that  poses on $\bSbbt$: $\lambda=1$ (i.e., $\bSbbt + \bSbmu$) is fully coupled, while $\lambda=0$ (i.e., $\bSbbt$) is fully decoupled. Theorem~\ref{thm:pretrain-finetune},~\ref{thm:joint-training} imply that optimizing trainable prompts can lead to decoupling, i.e., for a $j$-indexed coupled variable:
$$\{\bSbbt+\bSbmu\}_j\xrightarrow[\text{optimize}]{}\{\bSbbt+\lambda_j\bSbmu\}_j, 0\le\lambda_j<1. $$
Take the explicit form of $\bar\W^\st$ in Theorem~\ref{thm:pretrain},~\ref{thm:joint-training} for example, $\Wb^\star_{\pt}$ is fully coupled since all $\lambda_i=1$: $$\scalemath{0.75}{\Wb^\star_{\pt}=\underbrace{(\bSbbt+\bSbmu)}_{i=1}\Big((n+1)\underbrace{(\bSbbt+\bSbmu)}_{i=2}+\texttt{tr}(\underbrace{\bSbbt+\bSbmu}_{i=3})\Iden\Big)^{-1}},$$
and $\Wb^\star_{\jt}$ is partially decoupled with $\lambda_1=0, \lambda_2=\frac{1}{n+1},\lambda_3=1$:
$$\scalemath{0.75}{\Wb^\star_{\jt} = \underbrace{\bSbbt}_{i=1}
\Big((n+1)\Big(\underbrace{\bSbbt +\frac{1}{n+1} \bSbmu}_{i=2}\Big) + \texttt{tr}(\underbrace{\bSbbt+\bSbmu}_{i=3}) \Iden \Big)^{-1},}$$



\item When the task means $\E[\bt_k]=\bmu_k$ are non-zero, the decoupling effect of trainable prompt differs across settings, and can be analyzed with the alternative form of Theorem~\ref{thm:pretrain-finetune} and Theorem~\ref{thm:joint-training} with Corollary~\ref{corollary:shared form} (see Appendix for the explicit form of $\lambda_i,\lambda_j$):

  
     \textbf{Fine-tuning}: In the pretraining-finetuning setting, despite the coupled statistics captured by the fixed $\W^\st_\pt$, 
    the prompts $\Pb^\st_\pt$ help decouple the terms in the loss $\Lc^\star_\ft$:
    \begin{align}
    &\Lc_\pt^\st(\W^\star_\pt(\bSbbt + \bSbmu),\bSbbt + \bSbmu)\notag\\\xrightarrow[\ft]{\Pb}&\Lc_\ft^\st\Big(\W^\star_\pt(\bSbbt + \bSbmu),\{\bSbbt+\lambda_j\bSbmu\}_j\Big).
    \notag
    \end{align}
    
    
     \textbf{Joint Training}: In the joint training setting, $\W,\Pb$ are optimized simultaneously. This allows $\Pb$ to decouple the covariance and mean components in both $\W^\st_\jt$ and $\Lc^\st_\jt(\W^*)$:
    \begin{align}
    &\Lc_\pt^\st(\W^\star_\pt(\bSbbt + \bSbmu),\bSbbt + \bSbmu)\notag\\\xrightarrow[\jt]{\W,\Pb}&\Lc^\st_\jt\Big(\W^\star_\jt(\{\bSbbt+\lambda_i\bSbmu\}_i),\{\bSbbt+\lambda_j\bSbmu\}_j\Big).
    \notag
    \end{align}
 

\end{itemize}
 It can be seen that joint training decouples 
 
 This observation suggests that incorporating additional task-specific trainable parameters into the single-layer linear attention model can help decouple the task covariance and task mean.



==> sec/meeting.tex <==
\section{Main Results}


\SO{Please state the main results \textbf{as clearly as possible}. I don't have bandwidth to read everything, however I can understand the importance of what we have so far and discuss next steps.}
\begin{assumption} ($n-$size dataset). For a fixed number of contexts $n \geq 0$, a dataset\textsuperscript{1} of size $n+1$, denoted by $(\mathbf{X}, \mathbf{y}, \mathbf{x}, y) \in \mathbb{R}^{n \times d} \times \mathbb{R}^n \times \mathbb{R}^d \times \mathbb{R}$, is generated as follows:

\begin{itemize}
    \item A task parameter is generated from a Gaussian prior, $\boldsymbol{\beta} \sim \mathcal{N}(\mu, \mathbf{I}_d)$.
    
    \item Conditioned on $\boldsymbol{\beta}$, $(\mathbf{x}, y)$ is generated by $\mathbf{x} \sim \mathcal{N}(0, \mathbf{\Sigma_x})$ and $y \sim \mathcal{N}(\boldsymbol{\beta}^{\top} \mathbf{x}, \sigma^2)$.
    
    \item Conditioned on $\boldsymbol{\beta}$, each row of $(\mathbf{X}, \mathbf{y}) \in \mathbb{R}^{n \times (d+1)}$ is an independent copy of $(\mathbf{x}^{\top}, y) \in \mathbb{R}^{d+1}$.
\end{itemize}
\end{assumption}


\begin{assumption} \textbf{ICL risk.} For model  with a fixed parameter $\mathbf{W}$, we measure its ICL risk by its \textit{average regression risk on an independent dataset}. Specifically, for $n \geq 0$, the ICL risk evaluated on a dataset of size $n$ is defined by
\[
\mathcal{R}_n(\mathbf{W}) := \mathbb{E} \left( f(\mathbf{X}, \mathbf{y}, \mathbf{x}; \mathbf{W}) - y \right)^2,
\]
where the expectation is taken with respect to the dataset $(\mathbf{X}, \mathbf{y}, \mathbf{x}, y)$ generated according to Assumption 1 with $n$ contexts.
\end{assumption}

\text{We also denote the prompt by}
\[
\mathbf{Z} := \begin{pmatrix}
\mathbf{X}^{\top} & \mathbf{x} \\
\mathbf{y}^{\top} & 0
\end{pmatrix} \in \mathbb{R}^{(d+1) \times (n+1)}.
\]


\begin{corollary} (Simplified ICL model). We consider an ICL model parameterized as a one-step GD with matrix steps:
$f(\mathbf{X}, \mathbf{y}, \mathbf{x}; \mathbf{W}) := \left\langle \mathbf{W} \mathbf{X}^{\top} \mathbf{y}, \mathbf{x} \right\rangle, \quad \mathbf{W} \in \mathbb{R}^{d \times d}$
\end{corollary} 

\begin{corollary}  (Simplified ICL-prompt model). We still consider the above ICL model with trainable prompts, then the input sequence and query token can be written by
\[
\Z=\begin{bmatrix}
    \p_1&\x_1&\dots&\x_n\\
    p&y_1&\dots&y_n
\end{bmatrix}^\top=\begin{bmatrix}
    \p_1&\X^\top\\
    p&\y^\top
\end{bmatrix}^\top\quad\text{and}\quad\z=\begin{bmatrix}
    \x\\0
\end{bmatrix}.
\]
Then the simplified model is $f(\mathbf{X}, \mathbf{y}, \mathbf{x}; \mathbf{W}) := \left\langle \mathbf{W} \mathbf{X}^{\top} \mathbf{y}+\mu, \mathbf{x} \right\rangle, \quad \mathbf{W} \in \mathbb{R}^{d \times d}$\\
The learnt prompt can be expressed with $\mathbf{W}:$ $\p=\begin{bmatrix}
    \W^{-1}\bmu\\\bmu^\top(\Wb^{-\top})\bmu+1
\end{bmatrix}$
\end{corollary} 


\begin{theorem}[Main Result on Joint Pretraining] 
\textit{(ICL risk). Fix $N \geq 0$ as the number of contexts for generating a dataset according to Assumption 1. The following holds for the ICL risk $\mathcal{R}_N(\cdot)$ defined in (2):}

\begin{enumerate}
    \item The minimizer of $\mathcal{R}_N(\cdot)$ is unique and given by
    \[
    \mathbf{W}_N^* := \left( \left(\text{tr}(\mathbf{\Sigma_x}) + \sigma^2\right) \mathbf{I} + (N + 1) \mathbf{\Sigma_x} \right)^{-1}.
    \]
    
    \item The minimum ICL risk is given by
    \[
    \min_{\mathbf{W}} \mathcal{R}_N(\mathbf{W}) = \mathcal{R}_N(\mathbf{W}_N^*) = \sigma^2 + \text{tr} \left( \mathbf{W}_N^* \mathbf{\Sigma_x} \left( \left(\text{tr}(\mathbf{\Sigma_x}) + \sigma^2\right) \mathbf{I} +  \mathbf{\Sigma_x} \right) \right).
    \]
    
    \item The excess ICL risk, denoted by $\Delta_N(\mathbf{W})$, is given by
    \[
    \Delta_N(\mathbf{W}) := \mathcal{R}_N(\mathbf{W}) - \min_{\mathbf{W}} \mathcal{R}_N(\mathbf{W}) = \left\langle \mathbf{\Sigma_x}, \left( \mathbf{W} - \mathbf{W}_N^* \right) \mathbf{\tilde{\Sigma}}_N \left( \mathbf{W} - \mathbf{W}_N^* \right)^{\top} \right\rangle,
    \]
    where
    \[
    \mathbf{\tilde{\Sigma}}_N := \mathbb{E} \left(  \mathbf{X}^{\top} \mathbf{y} \right) \left(  \mathbf{X}^{\top} \mathbf{y} \right)^{\top} = \Sigma_x \left(\left( \text{tr}(\mathbf{\Sigma_x}) + \sigma^2 \right) \mathbf{I} + (N + 1) \mathbf{\Sigma_x}\right).
    \]
\end{enumerate}
\end{theorem}

\begin{theorem}[Main Result on Pretrain$\rightarrow$Finetune] 
\end{theorem}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs//exp_figs/singletask_zero_joint}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs//exp_figs/singletask_zero_ft}
\end{figure}

\clearpage
\newpage

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs//exp_figs/multitask_zero_joint.png}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs//exp_figs/multitask_zero_ft.png}
\end{figure}
\clearpage
\newpage
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{/multitask_nonzero_joint.png}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{multitask_nonzero_ft.png}
\end{figure}
\clearpage
\newpage
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{singletask_nonzero_joint.png}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{singletask_nonzero_ft.png}
\end{figure}
\clearpage
\newpage

p -> mean, W-> Cov but not enough, h->scalling W in order to help capture the cov



\SO{If there is no main result proven so far, then clearly write exactly what the technical challenges are to prove so that we can discuss.}

\so{Precise theoretical claim to prove goes here. (This claim will help prove the main results.)}
\begin{challenge} Modeling of multi-task setting
\end{challenge}
\begin{challenge} The Vanilla ICL risk, joint training risk, finetuning risk seemingly to be consistent with large $N$
\end{challenge}
\begin{challenge} Formulation of pretrain-finetune
\end{challenge}

==> sec/non-iid.tex <==
r

==> sec/table_main.tex <==
\begin{table}
  \caption{\ankit{Add caption...}}
  \label{table:main}
  \centering
  \begin{tabular}{lcc}
    \toprule
    % &\multicolumn{}{c}{$\min_{\W}\Lc(\W):=$}                   \\
    % \cmidrule(r){1-3}
    % Linear model& i.i.d. & RAG\\
    % Task 
    % \midrule
    % \multirow{3}{*}{Linear model}
    & i.i.d.&RAG\\
    &$\Nc(0,\Iden),\Nc(0,\Iden)$&$\Nc(0,\Iden),\Nc(\alpha\x_{n+1},(1-\alpha^2)\Iden)$\\
    % &$\Nc(0,\Iden)$& $\Nc(\alpha\x_{n+1},(1-\alpha^2)\Iden)$ \\
    \midrule
    $\W^\st$ & $\frac{1}{n+d+1}\Iden$  & $\frac{1}{(\alpha^2d+1)n+d}\Iden$     \\
    % \midrule
    $\Lcs/d$     & $1-\frac{n}{n+d+1}$ & $1-\frac{(\alpha^2d+1-\alpha^2)n}{(\alpha^2d+1)n+d}$      \\
    \bottomrule
  \end{tabular}
\end{table}
